Brownian Noise Reduction: Maximizing Privacy Subject to Accuracy Constraints

There is a disconnect between how researchers and practitioners handle privacy-utility tradeoffs. Researchers primarily operate from a privacy first perspective, setting strict privacy requirements and minimizing risk subject to these constraints. Practitioners often desire an accuracy first perspective, possibly satisfied with the greatest privacy they can get subject to obtaining sufficiently small error. Ligett et al. have introduced a "noise reduction" algorithm to address the latter perspective. The authors show that by adding correlated Laplace noise and progressively reducing it on demand, it is possible to produce a sequence of increasingly accurate estimates of a private parameter while only paying a privacy cost for the least noisy iterate released. In this work, we generalize noise reduction to the setting of Gaussian noise, introducing the Brownian mechanism. The Brownian mechanism works by first adding Gaussian noise of high variance corresponding to the final point of a simulated Brownian motion. Then, at the practitioner's discretion, noise is gradually decreased by tracing back along the Brownian path to an earlier time. Our mechanism is more naturally applicable to the common setting of bounded $\ell_2$-sensitivity, empirically outperforms existing work on common statistical tasks, and provides customizable control of privacy loss over the entire interaction with the practitioner. We complement our Brownian mechanism with ReducedAboveThreshold, a generalization of the classical AboveThreshold algorithm that provides adaptive privacy guarantees. Overall, our results demonstrate that one can meet utility constraints while still maintaining strong levels of privacy.

==> OldFiles/Adaptive_Stopping.tex <==
\section{Data-dependent stopping via Augmented Mechanisms}
\label{sec:aug}

Noise reduction mechanisms, such as the Brownian mechanism presented in Section~\ref{sec:bm}, provide a general framework under which data analysts can heuristically optimize a utility function while still maintaining privacy guarantees. While it is true that the privacy loss of an $((\epsilon_n), \delta)$-noise reduction mechanism is bounded by $\epsilon_N$ under an arbitrary stopping condition $N$, in certain cases, the privacy loss process doesn't truly capture how much information is being leaked about the underlying database. It may be the case that we want to determine our stopping condition not just based on the noisy parameters we view, but also on the results of private queries we make to the trusted curator holding the data. For instance, in Example~\ref{ex:holdout}, we considered the case where we halted based on the accuracy of the parameter on some held-out dataset. In many cases, it may be more desirable to check accuracy on the private dataset. Repeatedly querying the curator, even in a private manner, may eventually leak information about the underlying dataset.

To address the above concerns, in this section, we present the framework of \textit{mechanism augmentation}. In short, instead of just releasing noisy estimates of the underlying parameter, we also release additional random variables which may privately reflect the underlying dataset $x \in \calX$. We then redefine privacy loss in terms of the joint distributions of these processes. By looking at the privacy loss at random times $N$ which are stopping times under the natural filtration generated by the iterates of the noise reduction mechanism and the additional random process, we can provide meaningful privacy loss bounds along with rigorous utility guarantees.

In addition to devising a general framework for mechanism augmentation, we also provide several concrete examples of augmenting processes. First, we look at how to augment noise reduction mechanisms with the classic differentially private algorithm AboveThreshold~\cite{dwork2014algorithmic}. Second, we extend the AboveThreshold procedure to itself take advantage of the noise reduction framework. With our new procedure, which we call ReducedAboveThreshold (RAT), we construct an augmenting process which adaptively changes its privacy levels over time to match those of the underlying noise reduction mechanism. This ultimately allows for increased utility while paying negligibly more in terms of privacy loss. Overall, our methods provide an adaptive means of privately optimizing utility functions on sensitive databases.

\subsection{Mechanism Augmentation}

We now present the general framework of \textit{mechanism augmentation}. The idea is that the data analyst not only receives a sequence of noisy parameter estimates $(\beta_n(x))_{n \in \N}$, but also a sequence of additional, arbitrary random variables $(\alpha_n)_{n \in \N} := (\alpha_n(x))_{n \in \N}$ taking values in some space $\calZ$. The distribution of these variables can be arbitrary, but will typically depend in some way on the private dataset $x \in \calX$. For instance, $\alpha_n$ could be a noisy estimate of the utility of parameter $\beta_n$ on the dataset $x \in \calX$. The process $(\alpha_n)_{n \in \N}$ is said to be an \textit{augmenting process} for the underlying noise-reduction mechanism, and jointly the two processes are called an \textit{augmented reduction mechanism}, or ARM for conciseness. The joint distribution of these two processes ultimately gives us a clean way of classifying privacy loss for data-dependent stopping conditions. We formally present the definition of augmented augmented reduction mechanisms below. %\rrcomment{Is it worth trying to generalize the augementing process to take an arbitrary number of augmenting processes, not just $(\alpha_n)$?  Why stop at just one additional process?}
%\jwcomment{The augmenting process as listed could be vector-valued, and thus without loss of generality we only need one process}



\begin{definition}[\textbf{Augmented Reduction Mechanisms (ARMs)}]
\label{def:aug_nrm}
Let $\calR$ be a noise reduction mechanism associated with a function $f : \calX \rightarrow \R^d$. Assume $(\beta_n)_{n \in \N} := (\beta_n(x))_{n \in \N}$ is the sequence of iterates produced by $\calR$, as defined in Definition~\ref{def:nrm}. Additionally, assume there is some additional \textit{augmenting process} $(\alpha_n)_{n \in \N} := (\alpha_n(x))_{n \in \N}$; $\alpha_n(x)$ taking values in some measurable space $(\calZ, \calH)$. may also depend on $\beta_1(x),\dots,\beta_n(x)$ but we leave this dependence implicit via $x$. Let $(\calF_n(x))_{n \in \N}$ be the filtration generated by both processes, i.e. $\calF_n(x) := \sigma(\alpha_m(x), \beta_m(x) : m \leq n)$. The \textbf{Augmented Reduction Mechanism} associated with $\calR$ and the augmenting process $(\alpha_n(x))_{n \in \N}$ is the function $\calA : \calX \times \calT \rightarrow (\R^d\times\calZ)^\ast$, which, when given a dataset $x \in \calX$ and a stopping rule $N \in \calT$, outputs the vectors:
$$
\beta_{1:N}(x) = (\beta_1(x),  \beta_2(x),  \dots, \beta_N(x)) \text{~ and ~}  \alpha_{1:N}(x) = (\alpha_1(x), \dots, \alpha_N(x)),
% = (\beta_1(x), \dots, \beta_{N((\beta_n(x), \alpha_n(x))_{n \in \N})})
$$
where $N \equiv N((\beta_n(x), \alpha_n(x))_{n=1}^N)$ is allowed to depend on all observed data up to stopping.

For any $n \in \N$ and $y \in \calX$, let $q^y_n$ be the joint density of $\beta_{1:n}(y)$ and $\alpha_{1:n}(y)$ on the product space $(\calY^n \times \calZ^n, \calG^{\otimes n} \otimes \calH^{\otimes n})$ with respect to some reference measure $\kappa$ \footnote{We always assume there are $\sigma$-finite reference measures $\nu$ and $\rho$ respectively on the measurable spaces $(\calY, \calG)$ and $(\calZ, \calH)$. With these measures in mind, we assume for any $y \in \calX$ that the joint law $\mu_n^y$ of $(\beta_{1:n}(y), \alpha_{1:n}(y))$ is absolutely continuous with respect to the product measure $\kappa := \nu^{\otimes n} \otimes \rho^{\otimes n}$ on the product space $(\calY^n \times \calZ^n, \calG^{\otimes n} \otimes \calH^{\otimes n})$, and thus admits a density with respect to $\kappa$, which we refer to as $q^y$. Typically, we will have $(\calY, \calG) = (\R^d, \calB(\R^d))$ and $(\calZ, \calH) = (\{0, 1\}, 2^{\{0, 1\}})$, so we can respectively take $\nu$ to be the Lebesgue measure and $\rho$ to be the counting measure.}. Then, if $x'$ is a neighbor of the input dataset $x$ on which $\calA$ is being run, the \textit{privacy loss process} for an augmented reduction mechanism is the discrete-time stochastic process $(\calL_{n}(x, x'))_{n \in \N}$ given by
$$
\calL_{n}(x, x') = \log\left(\frac{q^{x}_n(\beta_{1:n}, \alpha_{1:n})}{q^{x'}_n(\beta_{1:n}, \alpha_{1:n})}\right).
$$


\end{definition}

Now, we take time to notice the differences between the privacy loss processes presented in Definition~\ref{def:nrm} and Definition~\ref{def:aug_nrm} respectively. In Definition~\ref{def:nrm}, we were able to show that the privacy loss of any noise reduction mechanism \textit{only} depended on the privacy loss of the least noisy iterate. Here, this is generally not the case, as there may be complicated distributional dependencies between the iterates of the noise reduction mechanism $(\beta_n)_{n \in \N}$ and the augmenting process $(\alpha_n)_{n \in \N}$. Nonetheless, we are able to prove a simple decomposition result which will give us similar bounds on privacy loss.
%\rrcomment{With $k$ other augmenting processes, will you end up with something like $\calL_n^{Red}(x, x') + \calL_n^{Aug_1}(x, x')+ \calL_n^{Aug_2}(x,x') + \cdots \calL_n^{Aug_k}(x,x')$}

\begin{lemma}[\textbf{Privacy Loss Decomposition for Augmented Reduction Mechanisms}]
\label{lem:ploss_decomp}
Let $\calA : \calX \times \calT$ be an augmented reduction mechanism associated with some function $f$. Given a true underlying dataset $x \in \calX$ and a neighboring dataset $x'$, let $(\calL_n(x, x'))_{n \in \N}$ be the privacy loss process for $\calA$ as defined in Definition~\ref{def:aug_nrm}. Then, the privacy loss for any fixed $n \in \N$ decomposes as
$$
\calL_n(x, x') = \log\left(\frac{p^{x}_{n}(\beta_{n})}{p^{x'}_{n}(\beta_{n})}\right) + \log\left(\frac{q^{x}(\alpha_{1:n}\mid\beta_{1:n})}{q^{x'}(\alpha_{1:n}\mid\beta_{1:n})}\right)
$$
$$
=: \calL_n^{Red}(x, x') + \calL_n^{Aug}(x, x'),
$$
where $(\calL_n^{Red}(x, x'))_{n \in \N}$ is the privacy loss process for the underlying noise reduction mechanism, as defined in Lemma~\ref{lem:markov}.

\end{lemma}

Lemma~\ref{lem:ploss_decomp} directly follows from applying Bayes rule to the joint $q^x$ of the Brownian mechanism and the augmenting process. 
In words, the above lemma tells us that the privacy loss of an augmented reduction mechanism decomposes as the sum of the privacy loss of the underlying noise reduction mechanism, denoted $\calL^{Red}_n(x, x')$, and the conditional privacy loss of the process $(\alpha_n)_{n \in \N}$ given the points we have seen of the noise reduction mechanism, denoted $\calL^{Aug}_n(x, x')$. Consequently, we just need to control this latter quantity to get bounds of the overall privacy loss, since we already have tight high-probability control over the former.

This can be difficult for general augmenting processes $(\alpha_n)_{n \in \N}$. However, we are ultimately concerned with optimizing some utility function which depends both on the underlying dataset $x \in \calX$ and the current model parameter iterate, $\beta_n$. The goal of the analyst is just to want to view parameters until they are convinced the current parameter attains a certain target accuracy or utility. Our goal is thus twofold: provide tight control over $\calL^{Aug}_n(x, x')$ while simultaneously providing high-probability utility guarantees.

Luckily for us, there exists a mechanism which allows us to exactly accomplish this goal: AboveThreshold. We now discuss how to leverage AboveThreshold to create the first example of an augmented reduction mechanism.

\subsection{Augmenting with Above Threshold}

The AboveThreshold algorithm \cite{dwork2014algorithmic} is a classical example of a purely differentially private mechanism. AboveThreshold takes in a target privacy level $\epsilon$, a threshold $T$, and an adaptively chosen sequence of $\Delta$-sensitive functions, $(f_n)_{n = 1}^K$. The algorithm outputs a sequence of 0's and 1's, such that one can infer the first index of a parameter which has utility exceeding the threshold (in a noisy sense). Despite the algorithm's simplicity, due to its strong privacy and accuracy guarantees, it has seen use in a wide range of contexts \cite{ligett2017accuracy} \cite{}\rrcoment{Fix citation}. We outline AboveThreshold in Algorithm~\ref{alg:at} below. Lemma~\ref{lem:at}, which follows the algorithm, outlines the various theoretical guarantees AboveThreshold provides.

\begin{algorithm}[h]
\caption{AboveThreshold}\label{alg:at}
\begin{algorithmic}
\Require $\epsilon > 0$, input database $x \in \calX$, sequence $(f_n)_{n \in [K]}$ of $\Delta$ sensitive functions, threshold $T \in \R$.
\State $\zeta \sim \Lap\left(\frac{2\Delta}{\epsilon}\right)$
\State $\hat{T} := T + \zeta$
\For{$n \leq K$}
    \State $\xi_n \sim \Lap\left(\frac{4\Delta}{\epsilon}\right)$ 
    \If{$f_n(x) + \xi_n \geq \hat{T}$}
        \State Print $1$
        \State HALT
    \Else
        \State Print $0$
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{lemma}[\textbf{Guarantees of AboveThreshold}]
\label{lem:at}
Let $\epsilon > 0$ be an arbitrary privacy parameter, $(f_n)_{n \in [K]}$ an adaptively chosen sequence of $\Delta$-sensitive functions $f_n : \calX \rightarrow \R$, and $T \in \R$ an arbitrary threshold. Then, Algorithm~\ref{alg:at} is $\epsilon$-differentially private. Moreover, if the algorithm halts in round $N \in [K]$, then, with probability $\geq 1 - \gamma$, we have
$$
 f_N(x) \geq T - \frac{4\Delta\left(\log\left(\frac{2}{\gamma}\right) + \log(K)\right)}{\epsilon}.
$$

\end{lemma}

The proof of Lemma~\ref{alg:at} can be found in a standard textbook on Differential Privacy, such as \cite{dwork2014algorithmic}\rrcomment{\jwcomment{Yeah but I don't know if anyone ever refers to them}Are there other text books on DP?}. We now explain how to use Algorithm~\ref{alg:at} to construct an augmenting process for general noise reduction mechanisms. To do this, we recall the context in which we motivated noise reduction mechanisms. Recall, for a fixed underlying database $x \in \calX$, we thought of $f(x) \in \R^d$ as an optimal set of parameters for maximizing some utility function. The sequence of parameters $(\beta_n)_{n \in \N}$ being revealed by the noise reduction mechanism were all just noisy approximations to $f(x)$.

Formalizing this notion of utility maximizing parameters, we assume there is some utility function $u :\calX \times \R^d \rightarrow \R$. In words, $u(x, \beta)$ gives a measure of the utility of parameter $\beta$ on an input point $x$. We assume there is some $\Delta > 0$ such that, for all $\beta \in \R^d$, the function $u(\cdot, \beta) : \calX \rightarrow \R$ is at most $\Delta$-sensitive.

With this formalization in mind, the goal of the data analyst is to iteratively view parameters $\beta_1, \dots, \beta_n, \dots$ until one achieves sufficiently high utility, i.e. the utility is greater than or equal to some threshold $T$. In the context of AboveThreshold, the threshold input is $T$, the target privacy level is some $\epsilon$, and we adaptively select the $n$th function $f_n$ to be $f_n(x) = u(x, \beta_n)$. Example~\ref{eg:aug_at} below formalizes this by rephrasing AboveThreshold as an augmenting process, in the context outlined above.

\begin{example}[\textbf{Augmenting via AboveThreshold}]
\label{eg:aug_at}
Suppose $\calR : \calX \times \calT$ is an $((\epsilon_n)_{n \in [K]}, \delta)$-noise reduction mechanism for a function $f : \calX \rightarrow \R^d$. Suppose $u : \calX \times \R^d \rightarrow \R$ is a measure of the joint utility of datasets and parameters which is $\Delta$-sensitive for any $\beta \in \R^d$. Let the random variables $\hat{T} := T + \Lap(\frac{2\Delta}{\epsilon})$ and $\xi_n \sim \Lap(\frac{4\Delta}{\epsilon})$ all be jointly independent. Consider the augmenting process $(\alpha_n(x))_{n \in [K]}$ given by 
$$
\alpha_n(x) := \one_{\left\{u(x, \beta_n) + \xi_n \geq \hat{T}\right\}}.
$$
Then, at the stopping time $N := \inf\{n \in \N : \alpha_n(x)= 1\}$, for any neighboring $x' \sim x \in \calX$, we have, with probability at least $1 - \delta$,
$$
\calL_n(x, x') \leq \epsilon_N + \epsilon.
$$
This follows immediately from the differential privacy guarantees of Lemma~\ref{alg:at} and from Theorem~\ref{thm:up_conf}.
Moreover, for any $\gamma \in (0, 1)$,  with probability $\geq 1- \gamma$, we have that $f_n(x) \geq T- \eta$, where
$$
\eta := \frac{4\Delta\left(\log\left(\frac{2}{\gamma}\right) + \log(K)\right)}{\epsilon}.
$$
This follows from the utility guarantees in Lemma~\ref{lem:at}. Consequently, by taking a simple union bound, we obtain both the privacy and utility guarantees with probability at least $1 - \delta - \gamma$.


\end{example}

Example~\ref{eg:aug_at} provides perhaps the simplest example of a useful augmented reduction mechanism. Even in this simple example, we obtain high probability bounds on both privacy loss and accuracy. We take our inspiration for using AboveThreshold to ``augment" noise reduction methods from \cite{ligett2017accuracy}, who take a similar approach in their paper. Nonetheless, we are the first to formalize the combination of such methods through the framework of augmenting processes. While the benefit of this approach may not be as tangible in this example, it will be more tangible in the next example, in which we construct a new variant of AboveThreshold which more naturally aligns with the noise reduction framework.



\subsection{Combining Laplace Noise Reduction with AboveThreshold}

In the above Section, we demonstrated how to augment noise reduction mechanisms with AboveThreshold to obtain both strong privacy loss bounds and utility guarantees. However, AboveThreshold as presented above is still not a great fit for the noise reduction framework. Recall the goal of noise reduction was to iteratively strip noise from an estimate of an optimal private parameter, obtaining greater accuracy at the cost of privacy as noise is successively removed. With AboveThreshold, the privacy level $\epsilon > 0$ is fixed in advance. An ideal augmenting process should ultimately have its privacy degrade in tandem with the Brownian mechanism, allowing for overall increased utility.


To address this shortcoming of AboveThreshold, we construct a novel mechanism called ReducedAboveThreshold, or RAT for short. RAT, much like AboveThreshold, aims to halt the first time a query is approximately above a target threshold. However, whereas AboveThreshold took a single privacy parameter $\epsilon$, RAT takes an increasing sequence of privacy parameters $(\epsilon_n)_{n \in \N}$. If $N$ is the (random) first time a query is noisily above some threshold, RAT provides the ex-post guarantee that privacy loss is bounded by the random variable $\epsilon_N$. While this, quite naturally, does not provide differential privacy guarantees, it is a perfect fit for our accuracy-first mindset.

\begin{comment}
\subsubsection{ReducedAboveThreshold}

Before constructing ReducedAboveThreshold, we examine a method for the gradual release of sensitive data, first constructed in \cite{}. The authors in \cite{} construct a novel stochastic process for gradually removing noise from a hidden point, much like our Brownian mechanism. The main difference is that the Brownian mechanism has \textit{Gaussian} marginal distributions, fitting the framework of approximate differential privacy. The mechanism of [] et al., which we will refer to as \textit{Laplace Noise Reduction Mechanism}, or the \textit{LNR} mechanism for short, correspondingly has Laplace marginal distributions.

In Algorithm~\ref{alg:lnr} below, we state the gradual release mechanism presented in \cite{}. Then, in Lemma~\ref{}, we state its theoretical guarantees. The proofs of all mentioned guarantees can be found in the original paper.

\begin{algorithm}
\caption{LaplaceNoiseReduction}\label{alg:lnr}
\begin{algorithmic}
\Require $(\epsilon_n)_{n \in \N}$ increasing sequence of privacy parameters, input database $x\in \calX$, $\Delta$-sensitive function $f : \calX \rightarrow \R$.
\State $\beta_1 \gets f(x) + Lap\left(\frac{\Delta}{\epsilon_1}\right)$
\For{$n \in \N$}
    \State With probability $\left(\frac{\epsilon_n}{\epsilon_{n - 1}}\right)^2$, $\beta_n \gets \beta_{n -1}$
    \State Otherwise, $\beta_n \gets \beta_{n - 1} + Lap\left(\frac{\Delta}{\epsilon_n}\right)$
    \State Print $\beta_n$
\EndFor
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:lnr} enjoys the following theoretical guarantees.

\begin{lemma}[\textbf{Guarantees of the LNR mechanism}]\label{lem:lnr_guar}
Suppose $(\epsilon_n)_{n \in \N}$ is an increasing sequence of privacy parameters, $f : \calX \rightarrow \R$ is a function of sensitivity $\Delta$. The Laplace Noise Reduction Mechanism enjoys the following guarantees:
\begin{enumerate}
    \item The mechanism which release $\beta_{1:n}$, for any $n\in\N$, is $\epsilon_n$-differentially private.
    \item For any input $x \in \calX$ and number $n \in \N$, $\beta_n \sim Lap\left(\frac{\Delta}{\epsilon_n}\right) + f(x)$.
    \item $(\beta_n)_{n \in \N}$ is a Markov Process.
\end{enumerate}
\end{lemma}
\end{comment}
At a high level, RAT generalizes AboveThreshold by applying the Laplace Noise Reduction mechanism to the cutoff threshold $T$. In round $n$, instead of adding independent noise scaled inversely to $\epsilon$ to the queries, it instead adds independent noise scaled inversely to $\epsilon_n$. These combined alternations allow for stopping time-dependent accuracy guarantees, making RAT a strict generalization of the usual AboveThreshold procedure. Since ReducedAboveThreshold is not the focus of this work, we defer its presentation to Appendix~\ref{app:rat}. In particular, Algorithm~\ref{alg:rat} presents the algorithm itself, and Theorem~\ref{thm:rat} discusses the corresponding theoretical guarantees. 
%\rrcomment{Maybe don't reference things in the Appendix here}

Much like AboveThreshold, ReducedThreshold can be naturally applied as an augmenting process. This can be seen in the following example.

\begin{example}[\textbf{Augmenting with ReducedAboveThreshold}]
\label{ex:rat}
Suppose $\calB$ is a $((\epsilon_n)_{n \in \N}, \delta)$-Brownian mechanism associated with function $f$ and sequence of times $(t_n)_{n \in [K]}$. Furthermore, suppose $u : \calX \times \R^d \rightarrow \R$ is a measure of the joint utility of datasets and parameters which is $\Delta$-sensitive for any fixed $\beta \in \R^d$. Let $(\zeta_n)_{n \in [K]}$ and  $(\xi_n)_{n \in [K]}$ be obtained as in Algorithm~\ref{alg:rat} run with privacy parameters $(\epsilon_n')_{n \in [K]}$ and sensitivity parameter $\Delta$ (note that thresholds $(T_n)_{n \in [K]}$, adaptively chosen functions $(f_n)_{n \in [K]}$, and underlying database $x \in \calX$ are also inputs, but do not affect the generations of $(\zeta_n)_{n \in [K]}$ or $(\xi_n)_{n \in [K]}$). Consider the augmenting process $(\alpha_n)_{n \in \N}$ given by 
$$
\alpha_n := \one_{\left\{u(x, \beta_n) + \xi_n \geq T_n + \zeta_n\right\}}.
$$
Then, at the stopping time $N := \inf\{n \in \N : \alpha_n = 1\}$, for any neighboring $x' \sim x \in \calX$, with probability at least $1 - \delta$, we have the overall privacy loss bound \rrcomment{State this in terms of the ex-post privacy definition}
$$
\calL_N(x, x) = \calL^{Red}_N(x, x') + \calL^{Aug}_N(x, x') \leq \epsilon_N + \calL^{RAT}(x, x') \leq \epsilon_N + \epsilon_N',
$$
where $\calL^{RAT}(x, x')$ is the privacy loss for ReducedAboveThreshold, as outlined in Appendix~\ref{app:rat}.

Moreover, for any $\gamma \in (0, 1)$, we have that, with probability $\geq 1- \gamma$, $T - f_N(x) \leq \alpha_N$, where the $\alpha_n$ are given by
$$
\alpha_n \geq \frac{4\Delta\left(\log\left(\frac{2}{\gamma}\right) + \log(p_n)\right)}{\epsilon_n},
$$
where $(p_n)_{n \in [K]}$ is a sequence satisfying $\sum_{n \in [K]}p_n = 1$.
\end{example}

\rrcomment{What \jwcomment{I will think a bit on this}sort of experiment can you show that would highlight the improvement of RAT and traditional AboveThreshold?  Can we give an apples to apples comparison of privacy and then plot utility?}



==> OldFiles/Conclusion.tex <==
\section{Summary of Results and Related Work}
\subsection{Summary of Results}
In this work, we studied the general problem of releasing a sensitive, high-dimensional vector subject to utility constraints. Building off of the example of a Laplace noise-based noise reduction mechanism presented in \cite{koufogiannis2015gradual} and \cite{ligett2017accuracy}, we construct the Brownian mechanism -- a more natural noise reduction technique constructed from Gaussian noise. This mechanism more naturally aligns with common statistical techniques such as $\ell_2$-regularized logistic regression, principal component analysis, and ridge regression. 

We then demonstrated how noise reduction mechanism can be used to obtain data-dependent utility guarantees through the general framework of mechanism augmentation. This framework allows for one to combine an arbitrary noise reduction mechanism (such as the Brownian mechanism or aforementioned Laplace-based mechanism) with what we refer to as an augmenting process. When this augmenting process is strategically chosen to depend on the underlying sensitive database in a private manner, mechanism augmentation allows for provable, high-probability guarantees both in terms of privacy and utility.


\subsection{Related Work}

Our work mainly takes inspiration from \cite{ligett2017accuracy}. In this work, the authors provide a specific example of a mechanism for obtaining provable privacy and utility guarantees for gradually releasing a private vector. In particular, they do this by combining a Laplace noise-based noise reduction mechanism from \cite{koufogiannis2015gradual} with the classical AboveThreshold algorithm \cite{dwork2014algorithmic}. Our contributions serve as a strict generalization of these initial contributions. In particular, the results presented in \cite{ligett2017accuracy} can be recovered from our general framework of mechanism augmentation, which allows for general combinations of noise reduction mechanisms with data-dependent augmenting processes. Moreover, we construct the Brownian mechanism, a novel noise-reduction mechanism which leverages Gaussian noise instead of Laplace noise. 

Our Brownian mechanism directly parallels the Laplace noise reduction mechanism presented in \cite{koufogiannis2015gradual}. The main difference between the mechanisms just lies in the marginal distributions -- our mechanism has Gaussian marginal distributions whereas the latter has Laplace. As such, our mechanism serves as a better fit for settings such as $\ell_2$-regularized logistic regression, principal component analysis, or ridge regression -- all settings where $\ell_2$-sensitivity is a more natural measure of closeness. Our Brownian mechanism is also conceptually simpler than the Laplace noise based mechanism. The Laplace noise-based mechanism required the introduction of a novel, complicated stochastic process. The Brownian mechanism can just be stated in terms of a standard Brownian motion. Lastly, \cite{koufogiannis2015gradual} also mention the construction of a Brownian motion-based mechanism for the gradual release of a private vector. However, the mechanism and analysis presented in \cite{koufogiannis2015gradual} only provides privacy guarantees at times \textit{fixed in advance} -- not at random times as we do. This is a crucial deficit, as our motivation for noise-reduction mechanisms was to iteratively view parameters until we encountered an iterate satisfying utility constraints.


Our work is more tangentially related to various works in the statistical and probability-theoretic literature which aim to provide time-uniform, high-probability upper bounds on martingales. In \cite{howard2020line}, the authors construct a plethora of line-crossing inequalities for martingales. In particular, the results presented in this work can be seen as generalizations of Fact~\ref{fact:line_cross} to strictly more general classes of stochastic processes. Likewise, works such as \cite{howard2021unif} and \cite{kaufmann2018mixture} provide time-uniform curve crossing inequalities for martingales using the method of mixtures. These can be seen as generalizing the bounds in Fact~\ref{fact:mixture} more general classes of stochastic processes, and we take our inspiration for using mixture bounds from these works. Lastly, while not directly related, we use the above concentration inequalities in similar manner to \cite{whitehouse2021composition}. The main difference lies in the fact that \cite{whitehouse2021composition} uses these inequalities to study the fully-adaptive composition of differentially private algorithms, whereas we use the inequalities to construct privacy loss bounds for noise reduction mechanisms. 



\subsection{Future Directions}

In this work, we presented a general framework for combining noise reduction mechanisms with augmenting processes to obtain provable privacy and data-dependent utility guarantees. While we constructed the Brownian mechanism and \cite{koufogiannis2015gradual} constructed the Laplace noise reduction mechanism, there are currently no noise reduction mechanisms for categorical problems. In particular, it would be useful in many instances to have a noise-reduction equivalent of the exponential mechanism. It is not a priori clear how to go about constructing such a mechanism, so we leave this direction for future work. 

Another direction would be to come up with a more natural Laplace Noise Reduction mechanism. As aforementioned, the noise reduction mechanism presented in \cite{koufogiannis2015gradual} is complicated, unlike our Brownian mechanism which relies just on an underlying, easy-to-simulate continuous stochastic process. One would suspect that such a continuous process would exist while having Laplace marginal distributions as well. 



==> OldFiles/DP_and_Ploss.tex <==
\section{Mathematical Background}
In this section, we discuss the mathematical basics that are necessary to understand this paper. We start by briefly discussing notation and terminology which will be ubiquitously used throughout the paper. After this, we present the basics of differential privacy. In particular, we discuss in-depth the concept of \textit{privacy loss}, a random variable capturing how much information is leaked for any given outcome of a private algorithm, and \textit{ex-post privacy}, a form of privacy which provides a randomized, high-probability bound on privacy loss. Lastly, we discuss Brownian motion, a continuous-time stochastic process which will be used later to construct our Brownian mechanism. 

\subsection{Notation}

Throughout, we assume the space of databases is denoted as $\calX$. There is some arbitrary \textit{neighboring relation} $\sim$ defined on $\calX$, and we say databases $x, x' \in \calX$ are \textit{neighbors} if $x \sim x'$. As one example, if $\calX = \mathbb{X}^n$ for some data domain $\mathbb{X}$, vectors $x, x' \in \calX$ may be considered neighbors if $x$ and $x'$ differ in exactly one entry. Likewise, if $\calX = 2^\mathbb{X}$ (where $2^S$ denotes the power set of a set $S$), we may say subsets $x \sim x'$ if $x, x'$ are of finite size and $x$ can be obtained by deleting or adding one element of $\mathbb{X}$ from the set $x'$. Likewise, in this setting, we could say  $x \sim x'$ if the sets are of the same finite size and differ in one entry. The exact definition of neighboring datasets will not be important in what follows, so we choose to leave the notion as general as possible.

We will consider \textit{algorithms}, which are randomized mappings $A : \calX \rightarrow \calY$ taking inputs from $\calX$ to some output space $\calY$. We consider $\calY$ as a \textit{measurable space}, meaning $\calY$ is endowed with some $\sigma$-algebra $\calG$ denoting possible events. Recall that a $\sigma$-algebra $\calS$ for a set $S$ is simply a subset of $2^S$ containing the empty set and $S$ itself that is closed under countable union, countable intersection, and complements. To formalize the randomness used in algorithm $A$, for any $x \in \calX$, we can view $A(x)$ as a random variable $A(x) : \Omega \rightarrow \calY$ taking values from some probability space $(\Omega, \calF, \P)$ (where $\calF$ is a $\sigma$-algebra and $\P$ a probability measure) to outputs in the measurable space $(\calY, \calG)$. More often than not, for any input $x \in \calX$, we will need to consider a sequence of algorithm outputs/random variables $(A_n(x))_{n \in \N}$. We typically assume all random variables in the sequence are defined on a common probability space. If all algorithms $A_n$ take values in $(\calY, \calG)$, the sequence takes values in the infinite product space $(\calY^\infty, \calG^{\otimes \infty})$.

Given that we will be considering sequences of random outputs, it is sometimes necessary to discuss the measure-theoretic notion of a \textit{filtration}. Given some probability space $(\Omega, \calF, \P)$, a filtration $(\calF_n)_{n \in \N}$ for $\calF$ is a sequence of $\sigma$-algebras satisfying: (i) $\calF_n \subset \calF_{n + 1}$ for all $n \in \N$, and (ii) $\calF_n \subset \calF$ for all $n \in \N$. Given an arbitrary $\calY$-valued discrete-time stochastic process $(X_n)_{n \in \N}$, it is often useful to consider the filtration $(\calF_n)_{n \in \N}$ given by $\calF_n := \sigma(X_m : m\leq n)$. Such a filtration is called the \textit{natural filtration} of $\calF$ associated with $(X_n)_{n \in \N}$, as $\calF_n$ entails all possible events determined by the first $n$ iterates of the stochastic process $(X_n)_{n \in \N}$.

\begin{comment}
We ultimately want to privately release some high-dimensional parameter $\beta(x) \in \R^d$ which depends on the private input database $x \in \calX$. As such, we assume there is some function $f : \calX \rightarrow \R^d$ which takes $x \in \calX$ to corresponding parameters $f(x) \in \R^d$. Our goal is ultimately to find a good approximation for $f(x)$ without revealing too much information about the underlying dataset $x$. Our algorithms will always produceFor simplicity, we assume that $f$ has $\ell_2$-sensitivity 1, but this can be easily generalized to bounded sensitivity under any positive-definite matrix norm, $||\cdot||_A$. We will consider Many times, there is a \textit{utility function} $u :\calX \times \R^d \rightarrow \R$ which determines the utility of a parameter $\beta \in \R^d$ on an input database $x \in \calX$. For the sake of privacy, we always assume $u(\cdot, \beta)$ to be of bounded sensitivity $\Delta$ for any fixed $\beta \in \R^d$. When there is some utility function $u$ under consideration, we always assume $f$ takes an input database $x$ to a corresponding optimal parameter in $\R^d$, i.e.
$$
f(x) = \arg\min_{\beta \in \R^d} u(x, \beta).
$$
\end{comment}


Lastly, we model viewing a random number of iterates of a hidden parameter through what we call \textit{stopping rules}. A stopping rule can just be viewed as a measurable map from a measurable space $(\calY^\infty, \calG^\infty)$ of sequences of outputs to $(\N, 2^\N)$, the measurable space of times at which an adversary can stop. By $\calT$ we denote the space of all stopping rules.
Note that, for any $x \in \calX$, $N((A_n(x))_{n \in \N}) : \Omega \rightarrow \N$ is a random time, i.e. a stopping condition which depends potentially on past and future algorithm outputs. If $(\calF_n(x))_{n \in \N}$ is the natural filtration of $(A_n(x))_{n \in \N}$, depending on the input $x \in \calX$, we say $N((A_n(x))_{n \in \N})$ is a $(\calF_n(x))_{n \in \N}$ stopping time if the event $\{N((A_n(x))_{n \in \N}) \leq n\}$ is contained in the sigma algebra $\calF_n(x)$. In plain English, this means that whether or not we stop in round $n$ only depends on the outputs we have seen up to and including round $n$. When we design our noise reduction algorithms later, it will always take the form of a randomized mapping $\calR : \calX \times \calT \rightarrow \calY^\ast$ where $\calY^\ast$ consists of all possible finite sequences of algorithm outputs. In particular, for some sequence of algorithms $(A_n)_{n \in \N}$, $\calR(x, N)$ will output $A_{1:N}(x) := (A_1(x), \dots, A_N(x))$, where $N$ is used to represent $N((A_n(x))_{n \in \N})$ for conciseness. While our mechanisms will be able to take in any stopping rule, We then prove results about our mechanisms solely in the case where $N$ only depends on the data seen up to any point in time, i.e. $N((A_n(x))_{n \in \N})$ is a $(\calF_n(x))_{n \in N}$ stopping time for any $x \in \calX$. In a certain sense, there are no reasonable situations in which one would hope to use future iterates to determine when to stop interacting with a private dataset. 

\subsection{Differential Privacy and Privacy Loss}
In this section, we briefly cover several important concepts in the field of differential privacy. We begin with the definition of differential privacy.


\begin{definition}[\textbf{Differential Privacy}]
\label{def:dp}
A randomized algorithm $A$ having inputs in a space $\calX$ and outputs in a measurable space $(\calY, \calG)$ is said to be $(\epsilon, \delta)$-differentially private if, for any neighboring inputs $x \sim x' \in \calX$ and $G \in \calG$,
$$
\P\left(A(x) \in G\right) \leq e^\epsilon \P\left(A(x') \in G\right) + \delta.
$$

\end{definition}

In short, an algorithm is differentially private if similar inputs induce similar distributions over outputs. While differential privacy has proven itself a mainstay of private computation, the definition can be too rigid to allow data analysts to freely explore privacy-utility tradeoffs in many problems. In particular, to attain the strong probabilistic guarantees of differential privacy, many algorithms have inherently weak utility guarantees. This is because, in order to guarantee differential privacy, it is necessary to pre-specify a desired level of privacy (determined through $\epsilon$ and $\delta$). Correspondingly, the goal of a mechanism is to optimize utility guarantees to meet this fixed level of privacy. Often times, in industry settings where model accuracy/utility may have impacts in safety-critical regimes, the incentive structure is reversed.  In particular, \textit{some} level of privacy may be desired, but only subject to fixed, high-probability accuracy goals being met. 
%\rrcomment{It would be nice to have an example of an application that said utility first then privacy, otherwise people might not think this is a very privacy centric approach.  I will look around. [Update] I was not able to find an example that stated what accuracy they want first}.
As such, we need a more flexible framework in which to construct our mechanism. The authors of \cite{ligett2017accuracy} recognized that the study of the  information-theoretic notion of \textit{privacy loss} is a perfect fit, and as a consequence we adopt the same perspective here.


%\swcomment{I would suggest we rephrase the above two paragraphs differently: typically, we perform differentially private data analysis by committing to fixed privacy parameters $(\epsilon, \delta)$ ahead of time. In some cases, however, high accuracy or utility is the primary goal, so a more natural goal is to achieve a fixed level of accuracy while minimizing privacy loss. Here we define privacy loss...} 


\begin{definition}[\textbf{Privacy Loss}]
\label{def:ploss}
Suppose $A$ is a randomized algorithm mapping inputs in a space $\calX$ to outputs in a measurable space $(\calY, \calG)$. Fix two neighboring inputs $x \sim x' \in \calX$. The privacy loss between $A(x)$ and $A(x')$, denoted as $\calL(x, x')$, is the random variable given by
$$
\calL(x, x') = \log\left(\frac{p^x(A(x))}{p^{x'}(A(x))}\right),
$$
where $p^x$ and $p^{x'}$ are the respective densities for the laws of $A(x)$ and $A(x')$ with respect to an arbitrary common dominating measure on $(\calG, \calY)$.

\end{definition}

Privacy loss can essentially be seen as a log-likelihood ratio, giving the bias a data analyst would have toward whether the witnessed outputs were produced by an input $x$ or a similar input $x'$. When privacy loss is very negative, an analyst would believe $x'$ was the underlying dataset. Likewise, if privacy loss were high, the analyst would be biased toward to the input $x$. 
\begin{comment}
Often times, we will need to consider the slightly more abstract of \textit{conditional privacy loss}. Conditional privacy loss allows a data analyst to re-calibrate his beliefs about the underlying dataset based on auxiliary information he may observe. This is particularly useful in the case where the noise being added is correlated over rounds, as will be the case in the Brownian mechanism we introduce. Formally, we have the following.

\begin{definition}[\textbf{Conditional Privacy Loss}]
\label{def:cploss}
Suppose $A$ is a randomized algorithm mapping inputs in a space $\calX$ to outputs in a measurable space $(\calY, \calG)$. Let $Y$ be a random variable. Fix any neighboring inputs $x \sim x' \in \calX$. The privacy loss between $A(x)$ and $A(x')$ \textit{conditioned on} $Y$, denoted $L_{Y}(x, x')$, is the random variable given by 
$$
L_{Y}(x, x') := \log\left(\frac{p_{x|Y}(A(x))}{p_{x'|Y}(A(x'))}\right),
$$
where $p_{x|Y}$ and $p_{x'|Y}$ are the respective conditional densities for $A(x)$ and $A(x')$ given $Y$.

\end{definition}

Definition~\ref{def:cploss} gives us a straightforward way for decomposing the privacy loss of a sequential interaction. Suppose $\beta_{1:n} := (\beta_1, \dots, \beta_n)$ is the random vector representing the outputs of the first $n$ rounds of a sequential interaction, and suppose that a data analyst is speculating whether the data was being produced from an input $x$ or another input $x'$. From Bayes rule, it follows that the privacy loss for the first $n$ outputs (denoted $L_{1:n}(x, x')$ to indicate composition) can be decomposed as
$$
L_{1:n}(x, x') = \sum_{m \leq n}\log\left(\frac{p_{x|\beta_{1:m -1}}(\beta_m)}{p_{x'|\beta_{1:m-1}}(\beta_m)}\right) = \sum_{m \leq n}\log\left(\frac{p_{x|\beta_{m+1:n}}(\beta_m)}{p_{x'|\beta_{m + 1|n}}(\beta_m)}\right).
$$

Note that the above decomposition also holds if we replace the deterministic time $n$ with an arbitrary (random) stopping condition $\tau$. Typically, this random time $\tau$ will be taken to be the first time a target accuracy is hit, or the first time loss falls below some threshold. Thus, to provide privacy guarantees we will aim to control the composed privacy loss $L_{1:\tau}$.
\end{comment}

One may (incorrectly) think that differential privacy can be simply defined in terms of a probabilistic guarantee on the privacy loss random variable. Namely, an algorithm $A$ should be be $(\epsilon, \delta)$-differentially private if and only if $\P\left(\calL(x, x') \geq \epsilon\right) \leq \delta$ for all neighbors $x \sim x'$. Unfortunately, a simple deterministic post-processing of randomized response \cite{} shows that the supposed equivalence isn't true. %\rrcomment{Can you write down the example (I believe you are thinking of the randomized response example on 4 outcomes and then post-processing it to get 2 outcomes that then breaks the probability statement).  Without writing it out, it just feels like a missing detail or ``We leave this as an exercise to the reader..."}. 
However, there is a useful one-way implication. In the reverse direction, one has to pay a price according to the privacy parameters $\epsilon$ and $\delta$. The proof of Lemma~\ref{lem:priv_conv} can be found in \cite{kasiviswanathan2014semantics}.

\begin{lemma}
\label{lem:priv_conv}
Let $A : \calX \rightarrow \calY$ be a randomized algorithm, and suppose, for any $x \sim x' \in \calX$, $\P(\calL(x, x') \geq \epsilon) \leq \delta$, where the probability is over the randomness used in algorithm $A$. Then, the algorithm $A$ is $(\epsilon, \delta)$-differentially private.

Likewise, if $A$ is $(\epsilon, \delta)$-differentially private, then, for any $x, x' \in \calX$, we have that with probability at least $1 - \frac{2\delta}{e^\epsilon\epsilon}$
$$
\calL(x, x') \leq 2\epsilon.
$$
\end{lemma}

Thus, while controlling privacy loss with high probability cannot be equated with differential privacy, it does indeed imply it. This motivates a definition of privacy called \textit{ex-post privacy}. In simple terms, ex-post privacy gives a random, high-probability bound on the privacy loss of an algorithm. Importantly, the bound is computable, and depends \textit{only} on the viewed output of the algorithm. Ex-post privacy is formally defined as follows.

\begin{definition}[\textbf{Ex-post Privacy}]
\label{def:ex_post}
Suppose $A :\calX \rightarrow \calY$ is a randomized algorithm, $\Epsilon : \calY \rightarrow \R_{\geq 0}$ is a function, and $\delta \in (0,1)$. Then, we say $A$ is $(\Epsilon, \delta)$-ex-post private if, for all neighboring datasets $x \sim x' \in \calX$, we have
$$
\P(\calL(x, x') \geq \Epsilon(A(x)))\leq \delta.
$$
\end{definition}


%ADD CITATION, ONE MORE SENTENCE MOTIVATION. EXAMPLE OF WHY THIS IS NOT CAPTURED. ADD WHAT WAS DONE, WHAT IS DIFFERENT. CITE RYAN'S.
Clearly, since $\Epsilon(A(x))$ is itself random, ex-post privacy does not imply differential privacy. However, in settings such as \cite{} where privacy is a secondary concern, ex-post privacy has proven itself a valuable tool for measuring how much information was leaked by any given computation. In sum, the flexibility provided by allowing a randomized upper bound on privacy loss ultimately lets a data analyst to obtain stronger, provable utility guarantees. We will detail the applications of ex-post privacy to utility maximization in the sections to come.

\subsection{Background on Brownian Motion}
\label{sec:bm_background}

Brownian motion is perhaps the most famous example of a continuous time stochastic process. First introduced in the context of describing the dispersion of pollen on the surface of water, Brownian Motion has found applications throughout areas of mathematics from queueing theory \cite{reiman1984open} to quantitative finance \cite{shreve2004stochastic}. In this work, we will apply Brownian Motion to the study of data privacy, constructing what we call the \textit{Brownian Mechanism}.

Before we can describe our mechanism, we first convey both the definition and basic properties of standard Brownian Motion.

\begin{definition}[\textbf{Standard Brownian Motion}]
\label{def:bm}
A real-valued stochastic process $(B_t)_{t \geq 0}$ is a standard 1-dimensional Brownian motion if it satisfies the following criteria.
\begin{enumerate}
    \item $B_t$ has almost surely continuous sample paths.
    \item $B_0 = 0$ almost surely.
    \item $B_t$ has independent increments, i.e. $B_{t + s} - B_t$ is independent of $B_t$ for any $s, t \geq 0$.
    \item $B_t \sim N(0, t)$.
\end{enumerate}

Likewise, a process $B_t$ in $\mathbb{R}^d$ is a $d$-dimensional standard Brownian motion if $B_t^{(i)}$ is standard 1-dimensional Brownian motion for each $i \in [d]$, and the components of $B_t$ are independent.
\end{definition}

Throughout, for conciseness, we will simply refer to standard Brownian Motion as just Brownian motion. Sometimes, we will consider a Brownian motion $(B'_t)_{t \geq 0}$ started at a point other than the origin. We trivially have the decomposition  $B_t' = x + B_t$ for some standard Brownian Motion, $(B_t)_{t \geq 0}$, where $x$ represents the desired initial point of the process. 

Brownian Motion enjoys a number of properties which will be useful in the sequel. We simply state these properties without proof, as they can all be found in reference texts such as \cite{durrett2019probability} and \cite{le2016brownian}.

\begin{fact}
\label{fact:bm_prop}
\textbf{Properties of Brownian Motion}
\begin{enumerate}
    \item Brownian motion is a martingale with respect to its natural filtration $(\mathcal{F}_t)_{t \geq 0}$ given by $\calF_t := \sigma\left(B_s: s\leq t\right)$, i.e. for all $0 \leq s \leq t$, $\mathbb{E}\left(B_t|\calF_s\right) = B_s$ almost surely.
    \item If $v \in \mathbb{R}^d$ is a unit vector (under the $\ell_2$ norm), $(B_t)_{t \geq 0}$ a standard $d$-dimensional Brownian motion, then the process $W_t := \langle v, B_t \rangle$ is a standard 1-dimensional Brownian motion.
    \item For any $\lambda > 0$, the process $(X_t^\lambda)_{t \geq 0}$ given by $X^\lambda_t := \exp\left(\lambda B_t - \frac{\lambda^2}{2}t\right)$ is a nonnegative martingale. It is known as \textit{Geometric Brownian motion}.
    \item Brownian motion obeys the \textit{Markov property}. That is, for any measurable set $A \subset \R^d$, $\P(B_t \in A \mid \calF_s) = \P(B_t \in A\mid B_s)$.

\end{enumerate}
\end{fact}

As mentioned in Fact~\ref{fact:bm_prop}, one of the most useful properties of Brownian Motion is that it is a martingale. At a high-level, a martingale is a stochastic process where our best guess for where the process will be at a future time is where the process is now. Martingales are of both practical and theoretical interest due to the fact they support strong, time-uniform concentration inequalities. The following classical result is the backbone of vast swath of time-uniform concentration results~\cite{howard2020line}, of which we will state a few later.

\begin{fact}[\textbf{Ville's Inequality}~\cite{ville1939etude}]
\label{fact:ville}
Suppose $(X_t)_{t \geq 0}$ is a nonnegative martingale. Let $\delta \in (0, 1)$ be an arbitrary fixed parameter. Then,
$$
\P\left(\exists t \geq 0 : X_t \geq \frac{\E X_0}{\delta}\right) \leq \delta.
$$
\end{fact}

A self-contained proof can be found in~\cite{howard2020line}.
Note that a standard Brownian Motion $B_t$ itself is not a nonnegative martingale. As a result, we cannot apply Fact~\ref{fact:ville} directly. However, do note that $(X^\lambda_t)_{t \geq 0}$, geometric Brownian motion with parameter $\lambda \in \R$, is in fact a nonnegative martingale. As a result, some of the concentration results below will leverage this process instead of Brownian motion directly.

One classic result regarding Brownian motion is what is a known as a line-crossing inequality. 

\begin{fact}[\textbf{Line Crossing Inequality for Brownian Motion}]
\label{fact:line_cross}
Suppose $(B_t)_{t \geq 0}$ is a standard Brownian motion. Let $a, b \in \R_{>0}$ be arbitrary positive real numbers. Then,
$$
\P\left(\exists t \geq 0 : B_t \geq at + b\right) = e^{-2ab}.
$$

\end{fact}

For a proof, see a standard graduate text in probability theory such as Durrett \cite{durrett2019probability} or Le Gall \cite{le2016brownian}.

Another concentration result for Brownian motion, which we call a curve crossing inequality (as opposed to line crossing) comes from applying a technique called \textit{the method of mixtures}. The method of mixtures is a technique for martingale concentration that hinges on a simple observation. Suppose $\{(X_t^\lambda)_{t \geq 0}\}_{\lambda \in \R}$ is a family of nonnegative martingales (indexed by $\lambda \in \R$), and suppose $\pi(d\lambda)$ is a probability measure on $\R$. Using Fubini's theorem for conditional expectations, it is straightforward to show that the \textit{mixture process} defined as 
$$
Y_t := \int_{\R}X^\lambda_t\pi(d\lambda)
$$
is in fact a nonnegative martingale. One can then apply Fact~\ref{fact:ville} to the process $(Y_t)_{t \geq 0}$ to obtain interesting concentration results.

The above paragraph may sound a bit dense on a first pass, but we can illustrate the usefulness of the technique in the following fact. 

\begin{fact}[\textbf{Curve Crossing Inequality for Brownian Motion}]
\label{fact:mixture}
Let $(B_t)_{t \geq 0}$ be a standard Brownian Motion, and let $\rho >0$ be a fixed positive real number. Then, for any confidence parameter $\delta \in (0,1)$, we have
$$
\P\left(\exists t \geq 0 : |B_t| \geq \sqrt{(t + \rho)\log\left(\frac{t + \rho}{\delta^2\rho}\right)}\right) \leq \delta.
$$

\end{fact}

To see a proof of Fact~\ref{fact:mixture}, and to see similar examples of the method of mixtures, see a work such as \cite{howard2021unif} or \cite{kaufmann2018mixture}. 






==> OldFiles/Experiments.tex <==
\section{Experiments}

We compare BM to LNR in the two experimental setting analyzed in \cite{ligett2017accuracy}.
\begin{enumerate}
    \item First, we perform ridge regression on the Twitter dataset to predict log popularity of twitter posts. We train on a randomly selected set of size $N = 10000$ where each data point has $d = 77$ features.
    \item Second, we perform logistic regression on the KDD-99 cup dataset to distinguish normal and malicious network traffic. We train on a randomly selected set of size $N = 10000$ and each data point has $d = 38$ features.
\end{enumerate}

For each experimental setting, produce three types of plots.
\begin{enumerate}
    \item First, we plot the guaranteed (with high probability) privacy loss of the iterates of LNR and BM against empirical loss (in either terms of logisitic loss or ridge loss) for a single run of each mechanism. For each subplot, we plot a vertical line demonstrating the obtained privacy loss for each of the methods illustrated in Section~\ref{} for obtaining a target accuracy/loss. 
    \item Second, we plot the guaranteed (with high probability) privacy loss of the iterates of each mechanism against the empirical loss \textit{averaged} over $M = 20$ trials. In addition, we plot, for both mechanisms, a point-wise valid 95\% upper confidence bound on empirical loss.
    \item Lastly, we create boxplots to illustrate the (empirical) distribution of privacy loss over $M = 20$ trials subject to each of the methods presented in Section~\ref{} for obtaining a target loss/accuracy.
\end{enumerate}

\begin{figure}
    \centering
    \subfloat[Comparing privacy loss of LNR and BM in Logistic Regression (holdout)]{
        \includegraphics[width=0.45\textwidth]{figs/boxplot_BM_LR_NONE.png}
        \includegraphics[width=0.45\textwidth]{figs/boxplot_LNR_LR_NONE.png}
        \label{fig:boxplot:lr_none}
    }\\
    \subfloat[Comparing privacy loss of LNR and BM in Logistic Regression (AT)]{
        \includegraphics[width=0.45\textwidth]{figs/boxplot_BM_LR_AT.png}
        \includegraphics[width=0.45\textwidth]{figs/boxplot_LNR_LR_AT.png}
        \label{fig:boxplot:lr_AT}
    }\\
    \subfloat[Comparing privacy of LNR and BM in Logistic Regression (RAT)]{
        \includegraphics[width=0.45\textwidth]{figs/boxplot_BM_LR_RAT.png}
        \includegraphics[width=0.45\textwidth]{figs/boxplot_LNR_LR_RAT.png}
    
    }

        
    \caption{Say something smart here later}
    \label{fig:odoms}
\end{figure}

==> OldFiles/Introduction.tex <==
\section{Introduction}
In an age in which data leaks frequently make headlines, the importance of privacy has never been clearer. As a result, leaders in the tech sector have turned to differential privacy as a framework for ensuring information security. From one relatively simple definition, researchers have developed an extensive arsenal of algorithms that allows data analysts to privately interact with sensitive datasets. These algorithms aim to accomplish a variety of goals, from privately understanding complex social networks to securely returning counts and order statistics on dataset.

However, in the age of machine learning, the most important private algorithms fall into the realm of utility maximization. Private utility maximization algorithms aim to allow data analysts to flexibly maximize a utility function over a sensitive dataset. These algorithms, such as private stochastic gradient descent, form the backbone of private machine learning, and are thus integral to conducting private data analysis. However, the theoretical guarantees provided by private utility maximization algorithms often don’t meet the needs of modern data analysts. This is because the majority of private utility maximization algorithms focus on meeting strict privacy guarantees, providing utility guarantees in terms of the privacy constraints \cite{chaudhuri2008privacy}, \cite{chaudhuri2011differentially}. Given that machine learning models are often used in safety-critical regimes \cite{phan2017preserving}, analysts may need to meet strict accuracy guarantees. Privacy may still be a desirable aspect of computation, but it is by no means the primary goal.

Only recently have researchers begun investigating techniques that prioritize optimizing utility while treating privacy guarantees as a secondary concern. This is in opposition to the standard approach to privacy, wherein algorithms are designed first and foremost to meet strict privacy requirements, optimizing utility guarantees subject to these privacy constraints.
%\rrcomment{\jwcomment{perhaps resolved now?} Can you be more specific here as to what you are referring to?  I would say that since the beginning of DP research, work has been about ensuring privacy while also showing (empirically or theoretically) the impact to utility.  Do you mean formulating this as an optimization problem is recent?}. 
One of the most promising mechanisms along this front was introduced in \cite{koufogiannis2015gradual}. In this work, the authors constructed a mechanism for gradually releasing a private, high-dimensional parameter. By successively removing Laplace noise in a correlated fashion from an initial vector, the authors are able to ensure that the privacy of releasing arbitrarily many estimates only depends on the privacy level of the least noisy parameters viewed. This is in stark contrast to results about the composition of differentially private algorithms, in which privacy degrades according to the total number of parameters viewed \cite{dwork2010boosting}, \cite{kairouz2015composition}, \cite{murtagh2016complexity}. Recognizing the importance of this gradual release mechanism to utility maximization, authors in \cite{ligett2017accuracy} created a novel means of integrating the above mechanism with the classic AboveThreshold procedure \cite{dwork2014algorithmic} to obtain provable utility and ex-post privacy. The authors then demonstrate the effectiveness of such a mechanism on common statistical problems such as ridge regression and $\ell_2$-regularized logistic regression. However, no work in the literature has attempted to construct a general framework for studying these mechanisms which gradually remove noise from a hidden parameter, which we hereinafter refer to \textit{noise reduction mechanisms}. By studying the properties of noise reduction mechanisms generally, one can directly apply powerful results to new mechanisms as they are developed. Moreover, such a framework can allow for modularity in combining base noise reduction mechanisms with classical procedures such as AboveThreshold which allow for data-dependent, utility maximizing guarantees.  As such, in this work, it is our goal to provide a general framework for studying noise reduction in the context of utility maximization.
\begin{comment}
In this work, \rrcomment{would be nice to have an itemized list of the contributions to make it more clear that the contribution is not just Laplace $\to$ Gaussian.} we extend the noise reduction framework to the realm of the Gaussian mechanism. In particular, by leveraging time-uniform concentration results for Brownian motion, we are able to develop a Gaussian analogue of the Laplace noise reduction technique introduced in [] and leveraged in []. Suitably, we call our mechanism the \textit{Brownian mechanism}. Our mechanism has a variety of desirable properties that make it preferable over the mechanism constructed with Laplace noise. First, since our mechanism leverages Gaussian noise instead of Laplace noise, it is more readily compatible with problems where utility is measured through the $\ell_2$ norm, such as private ridge regression and private principal component analysis. Second, the time-uniform bounds leveraged in our analysis can be fine-tuned for different desired tradeoffs between privacy and utility, providing an extra level of flexibility over the Laplace noise mechanism. Lastly, our mechanism can be modified to settings where the $\ell_2$ sensitivity of the utility function is unknown, but the sensitivity under some matrix norm is known. This allows for increased flexibility over the Laplace-based mechanism, which instead requires knowledge of the $\ell_1$ sensitivity. Ultimately, in order for differential privacy to be truly practical in industrial settings, researchers must construct mechanisms which give data analysts maximal flexibility. Our Brownian mechanism allows analysts to adaptively balance privacy-utility tradeoffs, allowing for greatly increased flexibility in private empirical risk minimization.


\subsection{Our Contributions}

In this work, we present a novel mechanism for gradually releasing a high-dimensional private vector subject to utility maximization constraints. In particular, we construct the \textit{Brownian mechanism}, a novel method of noise reduction which adds correlated Gaussian noise to a private, utility-maximizing parameter through a Brownian motion. In particular, our contributions surrounding the Brownian mechanism are as follows:


\begin{enumerate}
    \item In Section~\ref{sec:bm}, we construct the \textit{Brownian Mechanism}, a novel noise reduction mechanism for gradually revealing a private, high-dimensional vector. This mechanism significantly more flexible than the mechanism presented in \cite{} and \cite{}, as we can fine-tune our control of privacy loss through time-uniform concentration inequalities for Brownian motion. Additionally, our mechanism also merges more naturally with pervasive statistical problems such as private principal component analysis and private ridge regression.
    \item In Section~\ref{sec:aug}, we show how the Brownian mechanism can be used to gradually release a private parameter subject to utility constraints which depend on private data. We present the framework of \textit{Augmented Brownian Mechanisms}, which allows us to combine our Brownian mechanism with private queries to a hidden database while still controlling privacy loss. As an example, we show how to \textit{augment} our Brownian mechanism with the classical AboveThreshold mechanism to obtain high-probability bounds on both utility and privacy loss simultaneously.
    \item Also in Section~\ref{sec:aug}, we present another novel mechanism, \textit{ReducedAboveThreshold (RAT)}. RAT serves as an analogue to AboveThreshold where the noise added to queries is allowed to decrease over time. We show that ReducedAboveThreshold can be used to more naturally augment our Brownian mechanism, and as a result we can obtain tighter utility guarantees without sacrificing much in terms of privacy loss.
\end{enumerate}


In sum, our Brownian mechanism serves as a novel technique for allowing data analysts to adaptively balance privacy-utility tradeoffs. The fine-grained privacy control provided by the Brownian mechanism ultimately allows for greatly increased flexibility in privately solving utility maximization problems.
\end{comment}
\subsection{Our Contributions}

In our work, we provide a general approach for gradually releasing a high-dimensional, private vector subject to utility maximization constraints. We not only introduce a general definition for noise reduction mechanisms, but also introduce what we call the \textit{framework of mechanism augmentation}. In this framework, in addition to witnessing a sequence of noisy parameter iterates generated from a noise reduction mechanism, a data analyst is also shown iterates from some additional, data-dependent stochastic process. If this process, called the \textit{augmenting process}, is chosen strategically, data analysts can obtain both provable privacy and utility guarantees. We show how this framework can be applied by combining it with a novel noise reduction technique, which we call the \textit{Brownian mechanism}. The \textit{Brownian mechanism} works by adding correlated Gaussian noise to a private, utility-maximizing parameter through a Brownian motion. Noise is then iteratively stripped until a suitable stopping condition is met. We also create a new mechanism for data-dependent stopping, which we call \textit{ReducedAboveThreshold}. This mechanism is like AboveThreshold, but differs in that it guarantees higher accuracy as more queries are conducted. In full detail, our contributions are as follows.

\begin{enumerate}
    \item In Section~\ref{sec:bm}, we provide a general definition for noise reduction mechanisms and discuss some of the properties these mechanisms posses. To demonstrate the value in such a definition, we construct the \textit{Brownian Mechanism}, a novel noise reduction mechanism for gradually revealing a private, high-dimensional vector. This mechanism is significantly more flexible than the mechanism presented in \cite{koufogiannis2015gradual} and \cite{ligett2017accuracy}, as we can fine-tune our control of privacy loss through time-uniform concentration inequalities for Brownian motion. 
    \item In Section~\ref{sec:aug}, we present the framework of \textit{mechanism augmentation}, which involves slowly releasing noisy iterates from a noise reduction mechanism alongside iterates from an arbitrary, data-dependent stochastic process. By casting both classical and novel interactive mechanisms as stochastic processes, we are able to obtain provable privacy and utility guarantees for general noise reduction mechanisms. This framework allows for modularity. That is, one can combine arbitrary noise reduction mechanisms with other data-dependent algorithms to obtain simultaneous guarantees of privacy and accuracy-- all without having to consider them jointly.
\end{enumerate}

Overall, through our introductions, we demonstrate that noise reduction is actually a versatile technique which can be leveraged to balance privacy-utility tradeoffs. The fine-grained privacy and accuracy control provided by our techniques ultimately allows for greatly increased flexibility in privately solving utility maximization problems.

==> OldFiles/NR_and_BM.tex <==
\section{Noise Reduction and Useful Processes}

With the basics of privacy now at hand, we can more formally set up the problem of \textit{noise reduction} presented in the introduction. Ultimately, for any input database $x \in \calX$, there is a function $f$ which yields a high-dimensional parameter $f(x) \in \R^d$. This parameter should be interpreted as \textit{utility maximizer} for some optimization problem on the database $x$. That is, for some $u :\calX \times \R^d \rightarrow \R$, we have
$$
f(x) = \arg\min_{\beta \in \R^d}u(x, \beta).
$$

Since the database $x \in \calX$ may contain sensitive or even personally identifying information, an optimization algorithm shouldn't necessarily release the true parameter $f(x)$. Instead, it should release a noisy version.

If our goal were primarily privacy, one valid algorithm algorithm for privately releasing $f(x)$ would be the \textit{Gaussian mechanism}, which releases
$$
\hat{\beta} := f(x) + \xi, \qquad \xi \sim \mathcal{N}(0, \sigma^2 I_d),
$$
for some variance parameter $\sigma^2$. This mechanism guarantees \textit{differential privacy}, but ultimately doesn't allow a data analyst to fine-tune accuracy, which is what is desired.

For a data analyst, it may be more valuable to witness a stream of parameters $\beta_1, \beta_2, \dots, \beta_n, \dots$, where each successive parameter is less private (and thus hopefully more accurate) than the prior. Given such a stream, an analyst should be able to specify some (potentially random) stopping condition $N$ which depends on measured utility and see the output sequence $\beta_1, \dots, \beta_N$. The idea behind noise reduction is that an analyst should not pay an extra price in terms of privacy for the parameters they choose to throw away. More formally, the privacy for viewing the first $n$ noisy parameter estimates $\beta_1, \dots, \beta_n$ should be identical to that of having only witnessed the least noisy (i.e. least private), $\beta_n$. We can formalize this with the following definition of a noise reduction mechanism.

\begin{definition}
\label{def:nrm}
Let $\calR : \calX \times \calT \rightarrow \calY^\ast$ be a randomized algorithm taking in a database $x \in \calX$ and an arbitrary stopping rule $N \in \calT$, producing iterates $\beta_{1:N}(x) := (\beta_1(x), \dots, \beta_N(x)) = (\beta_1(x), \dots, \beta_{N((\beta_n(x))_{n \in \N})})$. For any $x \in \calX$ and any finite set of indices $\{i_1, \dots, i_m\} \subset \N$, let $p^x_{i_1, \dots, i_m}(b_{i_1}, \dots, b_{i_m})$ be the joint density of $(\beta_{i_1}(x), \dots, \beta_{i_m}(x))$.Then, we call $\calR$ a \textit{noise reduction mechanism} if, for every fixed alternative $x' \sim x$ and for every $n \in \N$, we have
$$
\calL_n(x, x') = \log\left(\frac{p^x_{1:n}(\beta_{1:n}(x))}{p^x_{1:n}(\beta_{1:n}(x))}\right) = \log\left(\frac{p^x_n(\beta_n(x))}{p^{x'}_n(\beta_n(x))}\right).
$$
 
Let $(\epsilon_n)_{n \in \N}$ be a sequence of privacy parameters, and $\delta \in (0, 1)$ a probability of failure. We say that $\calR$ is a $((\epsilon_n)_{n \in \N}, \delta)$-\textit{noise reduction mechanism} if, with probability at least $1 - \delta$, we have, simultaneously for all $n \in \N$
$$
\calL_n(x, x') \leq \epsilon_n.
$$
\end{definition}

Definition~\ref{def:nrm} simply tells us the noise reduction mechanisms allow data analysts to view many parameters, all while only paying a privacy cost for the most recent parameter seen. We have the following Lemma, which follows immediately from Definition~\ref{def:nrm}. In words, it tells us that noise reduction mechanisms have tight bounds on privacy loss under stopping conditions that only depend on the viewed parameters.

\begin{lemma}
\label{lem:nrm_stop}
Let $\calR : \calX \times \calT \rightarrow \calY^\ast$ be a noise reduction mechanism, and let $(\calF_n(x))_{n \in \N}$ be the corresponding natural filtration for the iterates of $\calR$ acting on input $x$. That is,
$$
\calF_n(x) := \sigma(\beta_m(x) : m \leq n).
$$
Then, for $N \in \calT$, if $N((\beta_n(x))_{n \in \N})$ is a $(\calF_n(x))_{n \in \N}$ stopping time for all $x \in \calX$, we have, with probability at least $1 - \delta$,
$$
\calL_N(x, x') \leq \epsilon_N
$$
That is, the algorithm $\calR(\cdot, N) : \calX \rightarrow \calY^\ast$ is $(\epsilon_N, \delta)$-ex-post private, per Definition~\ref{def:ex_post}.
\end{lemma}

The astute reader will notice that the high probability privacy loss bound in Lemma~\ref{lem:nrm_stop} actually holds at arbitrary random times $T \in \calT$, not just stopping times. So the question is, why did we restrict ourselves to stopping times in the statement. The answer is that, while the result does hold true at arbitrary times, if the stopping condition depends on information other than the viewed parameters, when we stop we could potentially leak additional information. Ideally, an analyst should be able to leverage additional information about the private dataset to aid in deciding which parameters to select. We address this concern in Section~\ref{sec:aug} below through the framework of \textit{mechanism augmentation}.

The question now is how should a researcher design a noise reduction mechanism? Clearly, adding i.i.d.\ noise to each parameter won't cut it, as this slowly reveals the underlying hidden point $f(x)$, and will correspondingly leak information the underlying dataset $x \in \calX$. More formally, the privacy loss will grow proportional to the number of parameters  The idea is to add \textit{correlated} noise in such a way that (i) all more-noisy iterates can be viewed as a randomized post-processing of the least noisy iterate viewed so far (ii) as we let the number of iterates go towards infinity, we should eventually recover the original parameter. Moreover, ideally the distribution of the iterates, when viewed alone, should match up with the distributions of existing mechanisms (typically either the Laplace or Gaussian mechanism). In the sequel we briefly cover an existing noise reduction mechanism which leverages Laplace noise. Then, we present a more natural form of noise reduction that applies correlated Gaussian noise through a Brownian motion.

\subsection{Laplace Noise Reduction Mechanism}

To be concrete, we first discuss an example of a noise reduction mechanism which has Laplace marginal distributions. This mechanism was never given a catchy name, so we just refer to it as the \textit{Laplace Noise Reduction mechanism} (LNRM) throughout the remainder of this paper. First presented in \cite{koufogiannis2015gradual} and later utilized in \cite{ligett2017accuracy}, LNRM functions by repeatedly adding correlated Laplace noise to some high dimensional parameter $f(x) \in \R$. This process, in turn, generates a sequence of iterates, which are then released in the reverse order of how they were generated. This results in a finite real-valued stochastic process $(\zeta_n)_{n \in [K]}$ where $K$ is the number of iterates. We illustrate the details of how to generate $(\zeta_n)_{n \in \N}$ in Algorithm~\ref{alg:lnr} below.

\begin{algorithm}[h!]
\caption{LaplaceNoiseReduction}\label{alg:lnr}
\begin{algorithmic}
\Require $(\epsilon_n)_{n \in [K]}$ increasing finite sequence of privacy parameters, sensitivity parameter $\Delta \geq 0$.
\State $\zeta_K \gets \Lap\left(\frac{\Delta}{\epsilon_K}\right)$
\For{$n \in K - 1,\dots, 1$}
    \State With probability $\left(\frac{\epsilon_n}{\epsilon_{n + 1}}\right)^2$, $\zeta_n \gets \zeta_{n + 1}$
    \State Otherwise, $\zeta_n \gets \zeta_{n + 1} + \Lap\left(\frac{\Delta}{\epsilon_n}\right)$
\EndFor
\State Return $\zeta_1, \dots, \zeta_K$.
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:lnr} enjoys the following properties, the proof of which can be found in \cite{koufogiannis2015gradual}.

\begin{fact}
Let $(\epsilon_n)_{n \in \N}$ be an increasing finite sequence of privacy parameters and $\Delta$ a sensitivity parameter. Let $(\zeta_n)_{n \in [K]}$ be the iterates produced by Algorithm~\ref{alg:lnr} when run on $(\epsilon_n)_{n \in [K]}$ and $\Delta$. Then,
\begin{enumerate}
    \item $\zeta_n \sim \Lap\left(\frac{\Delta}{\epsilon_n}\right)$, and
    \item $(\zeta_n)_{n \in [K]}$ is a Markov process with respect to the natural filtration $(\calF_n)_{n \in [K]}$.
\end{enumerate}
Furthermore, if $f:  \calX \rightarrow \R$ is a $\Delta$-sensitive function, define the mechanism $\calR : \calX \times \calT \rightarrow \R^\ast$ to satisfy
$$
\calR(x, N) := (f(x) + \zeta_1, \dots, f(x) + \zeta_N).
$$
Then, we have that $\calR$ is a $((\epsilon_n)_{n \in [K]}, 0)$-noise reduction mechanism.
\end{fact}



A $d$-dimensional version of Algorithm~\ref{alg:lnr} has successfully been used to privately release a parameter subject to accuracy constraints in \cite{ligett2017accuracy}. However, the approach in \cite{ligett2017accuracy} suffers in the sense that (i) the control it provides on privacy loss over time is not flexible, (ii) the constructed procedure is somewhat involved, and (iii) the marginal distributions are Laplace, whereas Gaussian marginals are often more practically useful. 

In the following section, using the preliminaries presented about Brownian Motion in Section~\ref{sec:bm}, we will construct a Gaussian analogue of LNRM which is ultimately more flexible. 



==> OldFiles/The_Brownian_Mechanism.tex <==
\section{The Brownian Mechanism}
\label{sec:nrm}



\subsection{Constructing the Brownian Mechanism from Brownian Motion}
\label{sec:bm}
In this section, we define a novel noise reduction technique which we call the \textit{Brownian Mechanism}. The idea behind Brownian mechanisms is simple. We mask a hidden parameter, say $\beta \in \R^d$, by adding on a $d$-dimensional standard Brownian motion. We then examine the process at strategically chosen times to gain privacy guarantees. Later, in Section~\ref{sec:aug}, we will discuss how to obtain utility guarantees as well. The noise added by the Brownian motion makes it difficult for an adversary to determine if $\beta$ was the underlying point being masked, or some other relatively close $\beta' \in \R^d$. Without further adieu, we present the definition of a the Brownian mechanism.


\begin{definition}[\textbf{Brownian Mechanism}]
\label{def:bm}
For a function $f : \calX \rightarrow \R^d$, a decreasing sequence of times $(t_n)_{n \in \N}$, and an input $x \in \calX$, define the sequence of iterates $(\beta_n(x))_{n \in \N}$ by 
$$
\beta_n(x) := f(x) + B_{t_n},
$$
where $(B_t)_{t \geq 0}$ is a $d$-dimensional standard Brownian motion. The \textbf{Brownian Mechanism} associated with a function $f$ and sequence of times $(t_n)_{n \in \N}$ is the function $\calB : \calX \times \calT \rightarrow (\R^d)^\ast$, which, when given a dataset $x \in \calX$ and a stopping condition $N \in \calT$, outputs the vector:
$$
\beta_{1:N}(x) = (\beta_1(x), \beta_2(x), \dots, \beta_N(x)) = (\beta_1(x), \dots, \beta_{N((\beta_n(x))_{n \in \N})}).
$$

\end{definition}

Definition~\ref{def:bm} essentially formalizes the earlier mentioned intuitive description of a Brownian mechanism. Going forward, we often drop the dependence on $x$ as we will be dealing with a fixed database throughout. In English, the Brownian mechanism takes a (hidden) input dataset and a stopping condition. It then releases correlated noisy estimates of the true hidden parameter (that is, $f(x)$), until some stopping condition (viewed as a random time $N$) is satisfied. When $N$ is large, we expect to gain more information about the underlying dataset, and thus we expect privacy loss to be large. On the other hand, when $N$ is small, we expect to have a small privacy loss. 

Before we can study various means for picking stopping conditions $N$, we show that the Brownian mechanism is, in fact, a noise reduction mechanism per Definition~\ref{def:nrm}. To do this, we examine the privacy loss process for the Brownian mechanism. One may expect the privacy loss process to be messy, as the data analyst is viewing multiple noisy estimates of $f(x) \in \R^d$. Thankfully, due to the fact Brownian motion is a Markov process, the privacy loss of viewing multiple parameters takes on a very simple form. 


\begin{lemma}
\label{lem:markov}
Let $\calB$ be the Brownian mechanism associated with a function $f$ and sequence of times $(t_n)_{n \in \N}$. Fix an underlying database $x \in \calX$, and, for any $n \in \N$, let $\beta_{1:n} := \calB(x, n)$ be the output of the Brownian mechanism run on $x$ and the deterministic time $n$. For any $x \in \calX$ and times $s_1 > s_2 > \cdots > s_1$, let $p^{x}_{s_1, \dots, s_m}(x_1, \dots, x_m)$ denote the joint density of Brownian motion started at $f(x)$ at times $s_1, \dots, s_m$. Fixing a neighbor $x' \sim x$, the \textit{privacy loss process} $(\calL_n(x, x'))_{n \in \N}$ satisfies:
$$
\calL_{n}(x, x') := \log\left(\frac{p^{x}_{t_n, \cdots, t_1}(\beta_n, \dots, \beta_1)}{p^{x'}_{t_n, \cdots, t_1}(\beta_n, \dots, \beta_1)}\right) =  \log\left(\frac{p^{x}_{t_n}(\beta_n)}{p^{x'}_{t_n}(\beta_n)}\right).
$$
In other words, the Brownian mechanism is a noise reduction mechanism. Consequently, if $N \in \calT$ satisfying that $N((\beta_n(x))_{n \in \N})$ is a stopping time with respect to the natural filtration for $(\beta_n(x))_{n \in \N}$ , we have the following privacy loss bound at time $N := N((\beta_n(x))_{n \in \N})$:
$$
\calL_N(x, x') = \log\left(\frac{p^x_{t_N}(\beta_N)}{p^{x'}_{t_N}(\beta_N)}\right).
$$
\end{lemma}

Lemma~\ref{lem:markov} tells us that an analyst who views multiple parameter estimates from a Brownian mechanism only pays a price (in terms of privacy loss) for the least private parameter viewed. This is exactly what we wanted out of a noise reduction mechanism with Gaussian marginals! Of course, there are still several holes to fill in. While we have shown that the privacy loss only depends on the least private parameter viewed by the analyst, we can actually say stronger things about the privacy loss process. In particular, we will find a closed form expression for the privacy loss process which can be stated in terms of a Brownian motion. Consequently, we will be able to apply the time-uniform bounds on Brownian motion discussed in Section~\ref{sec:bm_background} to get time-uniform bounds on privacy loss! Thus, we will be able to view the Brownian mechanism as a $((\epsilon_n)_{n \in \N}, \delta)$-noise reduction mechanism for any $\delta \in (0, 1)$ and a variety of sequences $(\epsilon_n)_{n \in \N}$.

\subsection{Characterizing the Privacy Loss of Brownian Mechanisms}

It is a well-known fact in differential privacy that the privacy loss random variable of the Gaussian mechanism is in fact itself normally distributed \cite{bun2016concentrated}
%\rrcomment{I dont think this result is in the text book and the author names for the book in the references looks off, as it says Dwork, Roth, et al. Maybe the correct cite is Bun, Steinke '16 or Dwork, Rothblum '16.}. 
It turns out that this characterization of privacy loss actually carries over to Brownian mechanisms as well. Namely, the privacy loss process of the Brownian mechanism can be decomposed as the sum of a standard Brownian motion and a deterministic drift term. Formally, we have the following Theorem. 

\begin{theorem}[\textbf{Privacy loss of the Brownian Mechanism}]
\label{thm:bm_ploss}
Let $\calB$ be the Brownian mechanism for a function $f : \calX \rightarrow \R^d$ and a sequence of times $(t_n)_{n \in \N}$. Fix an input database $x \in \calX$ and a function $f : \calX \rightarrow \R^d$, and, for any $n \in \N$, let $\beta_{1:n} := \beta_{1:n}(x) = \calB(x, n)$. Then, for any fixed alternative $x' \in \calX$, there exists a 1-dimensional Brownian Motion $(W_t)_{t \geq 0}$ such that the privacy loss process $(\calL_n(x, x'))_{n \in \N}$ for the Brownian mechanism satisfies
$$
\calL_n(x, x') = \frac{||f(x) - f(x')||_2^2}{2t_n} + \frac{||f(x) - f(x')||_2}{t_n}W_{t_n}.
$$
Consequently, if $f$ has $\ell_2$-sensitivity 1, we have the following bound on privacy loss:
$$
\calL_n(x, x') \leq \frac{1}{2t_n} +\frac{1}{t_n}|W_{t_n}|, \qquad \forall n \in \N.
$$

\end{theorem}

The proof of a more general version of Theorem~\ref{thm:bm_ploss} can be found in Appendix~\ref{app:gen_mech}. With Theorem~\ref{thm:bm_ploss} and the various time-uniform bounds on Brownian motion presented in Section~\ref{sec:bm_background}, we can now construct a slew of high-probability bounds on the privacy loss process, $(\calL_n(x, x'))_{n \in \N}$. These confidence sequences can be fine-tuned for a variety of settings, giving our Brownian mechanism added flexibility over the Laplace Noise Reduction Mechanism presented in \cite{koufogiannis2015gradual} and leveraged in \cite{ligett2017accuracy}.

\begin{theorem}[\textbf{Bounds on Privacy Loss}]
\label{thm:up_conf}
Let $\calB$ be the Brownian mechanism associated with a function $f$ and sequence of times $(t_n)_{n \in \N}$. For fixed alternatives $x \sim x' \in \calX$, let $(L_n(x, x'))_{n \in \N}$ be the corresponding privacy loss process associated $\calB$.  Then, for any confidence parameter $\delta \in (0, 1)$ and any following sequences $(\epsilon_n)_{n \in \N}$, $\calB$ is a $((\epsilon_n)_{n \in \N}, \delta)$-noise reduction mechanism:
\begin{enumerate}
    \item For any $\rho > 0$, the sequence $(\epsilon_n)_{n \in \N}$ given by
    $$
    \epsilon_n = \frac{1}{2t_n} + \frac{1}{t_n}\sqrt{(t_n + \rho)\log\left(\frac{t_n + \rho}{\rho\delta^2}\right)}.
    $$
    
    \item For any $a, b > 0$ such that $e^{-2ab} = \delta$, the sequence  $(\epsilon_n)_{n \in \N}$ given by
    $$
    \epsilon_n = \frac{1}{2t_n} + \frac{1}{t_n}(at_n + b).
    $$

    
\end{enumerate}
\end{theorem}

Theorem~\ref{thm:up_conf} gives a means of constructing high-probability time-uniform upper bounds on the privacy loss of the Brownian mechanism. As a consequence, we derive random bounds on the privacy loss for arbitrary stopping times $N$ which only depend on the iterates. However, note that Theorem~\ref{thm:up_conf} does not provide differential privacy guarantees. If we want to obtain the guarantees of differential privacy, we need to put an upper bound on how many iterates a data analyst can see. 

\begin{corollary}
Suppose $N \in \calT$ is a stopping time with respect to the natural filtration generated by the iterates of the Brownian mechanism, and $N' := N \land m$ is a new stopping rule obtained by taking the minimum of the stopping rule $N$ and the deterministic time $m \in \N$. Then, we have the guarantee
$$
\calL_{N'}(x, x') \leq \epsilon_m.
$$
Consequently, $\calB(x, N')$ is $(\epsilon_m, \delta)$-differentially private for any of the sequences $(\epsilon_n)_{n \in \N}$ listed in Theorem~\ref{thm:up_conf}.
\end{corollary}


As with any noise reduction viewed in isolation, there is a downside to the Brownian mechanism as presented so far. In particular, the stopping condition $N$ passed to $\calB$ must depend \textit{only} on the iterates viewed up to any point in time if we want to obtain meaningful privacy guarantees. While this allows a data analyst to determine stopping conditions based on criteria such as accuracy on a held-out dataset, ultimately an analyst may desire something more. In particular, accuracy/utility on the unknown, private dataset $x \in \calX$ may be desired. Technically, for \textit{any} random time $N$ (not just stopping times), we have the high-probability guarantee that
$$
\calL_N(x, x') \leq \epsilon_N.
$$
However, as aforementioned, when $N$ is not a function of the iterates, the time at which we stop can leak information about the underlying dataset (e.g. it could depend on additional, private queries to the database). In this case, we actually need to update the privacy loss process to reflect this additional information. We handle this more intricate situation in Section~\ref{sec:aug} below by introducing the general framework of \textit{mechanism augmentation}. Before we conclude this section, we provide a simple example of a situation where the Brownian mechanism (without augmentation) can still be of practical interest.

\begin{example}
\label{ex:holdout}
Let $x \in \calX$ be some unknown dataset, and $y \in \calX$ some fixed \textit{public} dataset openly available to the data analyst. Let $u :\calX \times \R^d \rightarrow \R$ be some utility function, and set the function $f$ to be the utility maximizer, i.e.
$$
f(x) := \arg\max_{\beta \in \R^d}u(x, \beta).
$$
Here, a data analyst may be comfortable with a iterate $\beta_n$ if it performs sufficiently well on the heldout dataset $y$. The (heuristic) intuition would be that if the parameter performs well on the heldout dataset $y$ and a sufficient amount of noise has been removed from the hidden parameter $f(x)$, then the parameter would also perform well (with respect to utility) on the hidden dataset $x$. 

More formally, we would define the stopping rule $N \in \calT$ as 
$$
N((y_n)_{n \in \N}) := \inf\{n \in \N: u(x, y_n) \geq T\},
$$
where $T$ is some suitably high threshold. It is clear that, for any $x \in \calX$, $N((\beta_n(x))_{n \in \N})$ is a stopping time with respect to the natural filtration for $(\beta_n(x))_{n \in \N}$. Then, running $\calB(x, N)$ would have a high-probability privacy loss bound of $\epsilon_N$ (for some chosen sequence $(\epsilon_n)_{n \in \N}$ on the privacy loss) and a utility of at least $T$ on the set $y$.

In many settings, this approach may perform suitably well. For more formal guarantees, however, Section~\ref{sec:aug} is needed.
\end{example}




==> OldFiles/abstract.tex <==
\begin{abstract}
    Differential privacy is rapidly becoming an industry-wide framework for protecting sensitive user information. However, in the modern, data-driven age, there is a growing detach between how theoreticians and practitioners desire to interact with privacy. Researchers designing private algorithms often approach problems from a \textit{privacy first} perspective, setting strict privacy constraints and optimizing utility functions subject to these constraints. On the other hand, practitioners may often prefer a \textit{utility first} perspective, setting strict utility constraints and taking whatever level privacy they can get subject to said constraints. To address this latter viewpoint on privacy, \cite{ligett2017accuracy} construct a \textit{noise reduction framework} using Laplace noise.  In short, a noise reduction mechanism interactively produces a sequence of increasingly accurate estimates of some utility maximizing parameter such that the privacy of the entire interaction \textit{only} depends on the privacy of the final (least noisy) parameter viewed. 
    % By combining a Laplace noise-based mechanism for the gradual release of sensitive data \cite{koufogiannis2015gradual} with the classical AboveThreshold mechanism \cite{dwork2014algorithmic}, the authors are able to optimize utility while still maintaining privacy for a variety of statistical problems.
    
    In this work, we design  a new \textit{Brownian mechanism}, a noise reduction mechanism which, instead of having Laplace marginals, has Gaussian marginals. This mechanism is not only more intuitive, but also is more readily applicable to problems such as principal component analysis and $\ell_2$-regularized logistic regression. In addition to the Brownian mechanism, we propose the general framework of \textit{mechanism augmentation}. This framework allows for the combination of arbitrary noise reduction mechanisms with additional, data-dependent \textit{augmenting processes} to obtain provable utility and privacy guarantees. Overall, our work yields a flexible framework within which practitioners of privacy can optimize utility while still preserving privacy.
    
    
\end{abstract}

==> OldFiles/even_older_files/Brownian_Motion.tex <==
\section{Background on Brownian Motion}
\subsection{Defining Brownian Motion and Basic Properties}
Brownian motion is perhaps the most famous (or infamous depending on how many homework problems you've done) example of a continuous time stochastic process. First introduced in the context of describing the dispersion of pollen on the surface of water, Brownian Motion has found applications throughout areas of mathematics from queueing theory to quantitative finance. In this work, we will apply Brownian Motion to the study of data privacy, constructing what we call the \textit{Brownian Mechanism}.

Before we can describe our mechanism, we first convey both the definition and basic properties of standard Brownian Motion.

\begin{definition}[\textbf{Standard Brownian Motion}]
\label{def:bm}
A real-valued stochastic process $(B_t)_{t \geq 0}$ is a standard 1-dimensional Brownian motion if it satisfies the following criteria.
\begin{enumerate}
    \item $B_t$ has almost surely continuous sample paths.
    \item $B_0 = 0$ almost surely.
    \item $B_t$ has independent increments, i.e. $B_{t + s} - B_t$ is independent of $B_t$ for any $s, t \geq 0$.
    \item $B_t \sim N(0, t)$.
\end{enumerate}

Likewise, a process $B_t$ in $\mathbb{R}^d$ is a $d$-dimensional standard Brownian motion if $B_t^{(i)}$ is standard 1-dimensional Brownian motion for each $i \in [d]$, and the components of $B_t$ are independent.
\end{definition}

Throughout, for conciseness, we will simply refer to standard Brownian Motion as just Brownian motion. Sometimes, we will consider a Brownian motion started at a point other than the origin. We write such a process as $(B^x_t)_{t \geq 0}$, where $x \in \R^d$ is the intial point. We trivially have the decomposition $B^x_t = x + B_t$ for some standard Brownian Motion, $(B_t)_{t \geq 0}$. 

Brownian Motion enjoys a number of properties which will be useful in the sequel. We simply state these properties without proof, as they can all be found in reference texts such as [] and [].

\begin{fact}[\textbf{Properties of Brownian Motion}]
\lab{fact:bm_prop}
\begin{enumerate}
    \item Brownian motion is a martingale with respect to its natural filtration $(\mathcal{F}_t)_{t \geq 0}$ given by $\calF_t := \sigma\left(B_s: s\leq t\right)$, i.e. for all $0 \leq s \leq t$, $\mathbb{E}\left(B_t|\calF_s\right) = B_s$ almost surely.
    \item If $p \in \mathbb{R}^d$ is a unit vector (under the $\ell_2$ norm), $B_t$ a standard $d$-dimensional Brownian motion, then the process $W_t := \langle p, B_t \rangle$ is a standard 1-dimensional Brownian motion.
    \item For any $\lambda > 0$, the process $(X_t^\lambda)_{t \geq 0}$ given by $X_t := \exp\left(\lambda B_t - \frac{\lambda^2}{2}t\right)$ is a martingale. It is known as \textit{Geometric Brownian motion}.
    \item Brownian motion obeys the \textit{Markov property}. That is, for any function $f$, $\mathbb{E}(f(B_t) | \calF_s) = \mathbb{E}(f(B_t)|B_s)$. This can alternatively be viewed as $\mathbb{E}(f(B_t)|\calF_s) = \mathbb{E}f\left(B^{B_s}_{t - s}\right)$.

\end{enumerate}
\end{fact}
\subsection{Concentration Results for Brownian Motion}
As mentioned in Fact~\ref{fact:bm_prop}, one of the most useful properties of Brownian Motion is that it is a martingale. At a high-level, a martingale is a stochastic process where our best guess for where the process will be at a future time is where the process is now. Martingales are of both practical and theoretical interest due to the fact they support strong, time-uniform concentration inequalities. The following classical result is the backbone of almost all time-uniform concentration results, of which we will state a few later.

\begin{fact}[\textbf{Ville's Inequality}]
\label{fact:ville}
Suppose $(X_t)_{t \geq 0}$ is a non-negative martingale. Let $\delta \in (0, 1)$ be an arbitrary fixed parameter. Then,
$$
\P\left(\exists t \geq 0 : X_t \geq \frac{1}{\delta}\right) \leq \delta.
$$

\end{fact}
Note that a standard Brownian Motion $B_t$ itself is not a non-negative martingale. As a result, we cannot apply Fact~\ref{fact:ville} directly. However, do note that $(X^\lambda_t)_{t \geq 0}$, geometric Brownian motion with parameter $\lambda \in \R$, is in fact a non-negative martingale. As a result, some of the concentration results below will leverage this process instead of Brownian motion directly.

One classic result regarding Brownian motion is what is a known as a line-crossing inequality. 

\begin{fact}[\textbf{Line Crossing Inequality for Brownian Motion}]
\label{fact:line_cross}
Suppose $(B_t)_{t \geq 0}$ is a standard Brownian motion. Let $a, b \in \R_{>0}$ be arbitrary positive real numbers. Then,
$$
\P\left(\exists t \geq 0 : B_t \geq at + b\right) \leq e^{-2ab}.
$$

\end{fact}

For a proof of Fact~\ref{fact:line_cross}, see a standard graduate text in probability theory such as Durrett [].

Another concentration result for Brownian motion, which we call a curve crossing inequality (as opposed to line crossing) comes from applying a technique called \textit{the method of mixtures}. The method of mixtures is a technique for martingale concentration that hinges on a simple observation. Suppose $\{(X_t^\lambda)_{t \geq 0}\}_{\lambda \in \R}$ is a family of non-negative martingales (indexed by $\lambda \in \R$), and suppose $\pi(d\lambda)$ is a probability measure on $\R$. Using Fubini's theorem for conditional expectations, it is straightforward to show that the \textit{mixture process} defined as 
$$
Y_t := \int_{\R}X^\lambda_t\pi(d\lambda)
$$
is in fact a non-negative martingale. One can then apply Fact~\ref{fact:ville} to the process $(Y_t)_{t \geq 0}$ to obtain interesting concentration results.

The above paragraph may sound a bit dense on a first pass, but we can illustrate the usefulness of the technique in the following Fact. 

\begin{fact}[\textbf{Curve Crossing Inequality for Brownian Motion}]
\label{fact:mixture}
Let $(B_t)_{t \geq 0}$ be a standard Brownian Motion, and let $\rho >0$ be a fixed positive real number. Then, for any confidence parameter $\delta \in (0,1)$, we have
$$
\P\left(\exists t \geq 0 : B_t > \sqrt{2(t + \rho)\log\left(\frac{t + \rho}{\delta^2\rho}\right)}\right).
$$

\end{fact}

The proof of Fact~\ref{fact:mixture} is already known, and can be found in papers such as [] and []. Nonetheless, since it illustrates how to apply the method of mixtures, we include the proof in the Appendix.






==> OldFiles/even_older_files/IntroductionOLD.tex <==
\section{Introduction}

In an age in which data leaks frequently make headlines, the importance of privacy has never been clearer. As a result, leaders in the tech sector have turned to differential privacy as a framework for ensuring information security. At an intuitive level, the definition of differential privacy is very simple: if two inputs to a randomized algorithm are similar, then the distributions of outputs should be similar as well. From this simple definition, researchers have constructed an arsenal of tools that analysts can use to understand datasets.

Despite the abundance of research surrounding differential privacy and its applications to data analysis, there are still many restrictions on how practitioners can privately interact with datasets. One of the most glaring drawbacks is the limited flexibility analysts have in balancing tradeoffs between data privacy and model utility in machine learning. The majority of differentially private algorithms focus on providing strict privacy guarantees, only providing utility results in expectation or with high probability. On the other hand, given that machine learning models are often used in safety-critical regimes, analysts may need to prioritize meeting strict accuracy guarantees. Privacy may still be a desirable aspect of computation, but it is by no means the primary goal.

There are naïve approaches for meeting accuracy guarantees while still maintaining privacy. For instance, an analyst may privately train a machine learning model, receive a noisy version of an optimal parameter, and then evaluate the parameter on a held-out set to test accuracy. If the accuracy is lower than some preordained threshold, the analyst may need to run the private algorithm again in hopes of generating a more accurate parameter. Clearly, iteratively doing this ensures that the overall level of privacy quickly degrades, for instance, according to advanced composition. Instead, to enable full flexibility in model training and testing, an analyst should only need to pay a privacy cost for the least noisy (and hence least private) parameter viewed so far. While this cannot be achieved by repeatedly adding independent noise to the outputs of an optimization procedure, it can be achieved by strategically adding correlated noise. 

This framework, which involves iteratively removing correlated noise from an optimal parameter estimate, is referred to as \textit{noise reduction}. The framework of noise reduction was first introduced in [REF], in which the authors investigate the problem of hitting a target accuracy while maximizing the overall level of privacy. 

has been considered in the context of using Laplace noise~\cite{ligett2017accuracy} \cite{koufogiannis2015gradual}, but it is often more desirable to use Gaussian noise instead. This is due to a variety of reasons, such as the fact Gaussian distributions have lighter tails than Laplace distributions, and thus introduce less error into the procedure. Moreover, many procedures such as Principal Component Analysis and $\ell_2$-regularized optimization meld naturally with the addition of Gaussian noise. Applying Laplace noise to these settings, on the other hand, requires messy conversions and approximations.





algorith despite the abundance of research surrounding differential privacy and its applications to data analysis, there are still many restrictions on how practitioners can privately interact with datasets. 

This disconnect has been addressed, to some degree, by considering the problem of \textit{noise reduction}.


Introduce Privacy:

Privacy Restrictive/Example of Privacy vs. utility tradeoffs:

Framework for Maximizing Utility:


Previous Works and Shortcomings:
The noise reduction framework was first considered in [REF]. In this work, the authors develop a Laplace-based noise mechanism for gradually releasing sensitive data. In particular, their mechanism provides the guarantee that if multiple noisy copies of the sensitive data are released, the overall privacy degrades only according to the least private version of the data released. This is contrary to results such as advanced composition [REF], which show a much greater, additive decay in overall privacy. Based on this mechanism, authors in [REF] develop a framework for doing private empirical risk minimization. In particular, they this mechanism along with the sparse vector mechanism to do private ridge and logistic regression. While the Laplace


Our Results:
In this work, we combine recent advances in time-uniform concentration with well-known results in continuous time stochastic processes to develop a Gaussian framework for doing noise reduction.
\begin{enumerate}
    \item We develop a flexible, Brownian motion-based mechanism for Gaussian noise reduction. This complements the original Laplace mechanism presented in REF and utilized in REF. Moreover, it present an increased level of flexibility, as it can be fine tuned for privacy-utility tradeoffs.

    \item We show how our mechanism can be applied to applications which naturally support Gaussian noise, such as private ridge regression and private principal component analysis. 
\end{enumerate}
 

==> OldFiles/even_older_files/Stochastic_Processes.tex <==
\section{Noise Reduction and Useful Processes}

In the previous section, we outlined the basics of differential privacy and ex-post privacy. At the heart of our exploration was the notion of privacy loss, a random variable which \swdelete{served as a proxy for measuring} \swedit{measures} how much information was released by any given output of a randomized algorithm. To satisfy ex-post privacy in a meaningful manner, we want to find mechanisms that give us tight control over the  privacy loss.

Recall that our goal in this work is ultimately to construct an ex-post private algorithm for approximately maximizing a utility function (equivalently, minimizing a loss function). In particular, we will focus on output perturbation algorithms, i.e. those which release multiple noisy estimates of some optimal, utility-maximizing parameter. Using such a mechanism, we can iteratively view noisy parameters, stopping when utility guarantees are met in some sense.  If we were to view multiple parameters, adding independent noise to each, we would expect bounds on privacy loss to quickly degrade. However, if we add correlated noise to the parameters, it is possible to obtain slowly degrading bounds on privacy loss, ultimately providing tighter ex-post privacy guarantees.

In particular, the best we can do is hope that the privacy of releasing $n$ parameter estimates only depends on the privacy of releasing the $n$th estimate. More specifically, if we can show that the sequence of released iterates forms a \textit{Markov} process, then this desired slow degradation of privacy loss will be achieved. We formalize this notion below, formally defining Markov processes and the notion of privacy loss of many parameters only depending on a single one. Then, we introduce Brownian motion, a classical example of a continuous-time Markov process. We will discuss the basics behind Brownian motion in preparation for presenting our Brownian mechanism in the following Section.

\swcomment{while i appreciate the overview above, i think the readers may find it hard to understand these descriptions without much context. I suggest we first describe the high-level problem we want to solve: releasing some vector-valued function $f(x)$ subject to some accuracy criterion while minimizing privacy loss. then briefly mention the key challenges and novel techniques}


\subsection{Markov Processes and their Privacy Loss}

We start by defining the general notion of a Markov process.

\begin{definition}[\textbf{Markov Processes}]
\label{def:markov_process}
Let $(X_n)_{n \in \N}$ be a stochastic process taking values in some measurable space $(E, \Epsilon)$. Let $(\calF_n)_{n \in \N}$ be the natural filtration for $(X_n)_{n \in \N}$, i.e. We say $(X_n)_{n \in \N}$ is a Markov process if, for any $n \in \N$ and any $A \in \Epsilon$,
$$
\P(X_{n + 1} \in A | X_{n}) = \P(X_{n + 1} \in A | \calF_n).
$$

\end{definition}

Intuitively, a process is Markovian (i.e. is a Markov process) if one's best guess for where the process is at time $n + 1$ given the whole history of the process up until time $n$ depends only on where the process was at time $n$. This property is known throughout as the \textit{Markov Property}, and it forms the basis of our privacy loss analysis.

Why are Markov processes important for us? Suppose $(p^x_{i_1, \dots, i_m})_{m \in \N, i_1 \leq i_2 \leq \cdots \leq i_m \in \N}$ \rrcomment{Can we use notation with fewer subscripts here, perhaps something like  $(p^x_{i_1, \dots, i_m}: m \in \N, i_j \in \N \text{ for } j \in [m] ,i_1 \leq i_2 \leq \cdots \leq i_m )$ } is a family of joint densities for the process $(M_n(x))_{n \in \N}$ at times $i_1, \dots, i_m$ with $M_1(x) = f(x) \in \R^d$ almost surely (we suppress the dependence on $x$ going forward). Suppose we viewed iterates $M_{i_1}, \dots, M_{i_m}$, and were questioning the starting point of the Markov process. That is, whether it was started at $f(x)$ or $f(x')$, for neighbors $x \sim x' \in \calX$. Given our discussion in the previous section, the \textit{privacy loss} might be a reasonable quantity of interest to examine. In particular, for $x \sim x'$, if $\calL_{I}(x, x')$ denotes the privacy loss of viewing the process at the times in $I \subset \N$, we have
\swcomment{indices are quite confusing here. is $i_1$ different from 1?}\rrcomment{I concur.}
$$
\calL_I(x, x') := \log\left(\frac{p_I^x(M_I(x))}{p_I^{x'}(M_I(x))}\right) = \log\left(\frac{p_{i_1}^x(M_{i_1}(x))}{p_{i_1}^{x'}(M_{i_1}(x))}\right).
$$

That is, the privacy loss random variable only depends on the earliest time at which we examined the Markov process! Thus, as we will see below, if we can reframe popular differentially private algorithms such as the Laplace and Gaussian mechanism in the framework of Markov processes, we can view many noisy estimates for an optimal parameter and only pay a privacy cost for the least noisy one. This will ultimately allow us to obtain improved utility over traditional differentially private methods.



\subsection{Brownian Motion}

Brownian motion is perhaps the most famous (or infamous depending on how many homework problems you've done)\swcomment{make sure you delete this...} example of a continuous time stochastic process. First introduced in the context of describing the dispersion of pollen on the surface of water\rrcomment{cite, maybe?}, Brownian Motion has found applications throughout areas of mathematics from queueing theory to quantitative finance. In this work, we will apply Brownian Motion to the study of data privacy, constructing what we call the \textit{Brownian Mechanism}.

Before we can describe our mechanism, we first convey both the definition and basic properties of standard Brownian Motion.

\begin{definition}[\textbf{Standard Brownian Motion}]
\label{def:bm}
A real-valued stochastic process $(B_t)_{t \geq 0}$ is a standard 1-dimensional Brownian motion if it satisfies the following criteria.
\begin{enumerate}
    \item $B_t$ has almost surely continuous sample paths.
    \item $B_0 = 0$ almost surely.
    \item $B_t$ has independent increments, i.e. $B_{t + s} - B_t$ is independent of $B_t$ for any $s, t \geq 0$.
    \item $B_t \sim N(0, t)$.
\end{enumerate}

Likewise, a process $B_t$ in $\mathbb{R}^d$ is a $d$-dimensional standard Brownian motion if $B_t^{(i)}$ is standard 1-dimensional Brownian motion for each $i \in [d]$, and the components of $B_t$ are independent.
\end{definition}

Throughout, for conciseness, we will simply refer to standard Brownian Motion as just Brownian motion. Sometimes, we will consider a Brownian motion started at a point other than the origin. We write such a process as $(B^x_t)_{t \geq 0}$, where $x \in \R^d$ is the intial point. We trivially have the decomposition $B^x_t = x + B_t$ for some standard Brownian Motion, $(B_t)_{t \geq 0}$. 

Brownian Motion enjoys a number of properties which will be useful in the sequel. We simply state these properties without proof, as they can all be found in reference texts such as [] and [].

\begin{fact}
\label{fact:bm_prop}
\textbf{Properties of Brownian Motion}
\begin{enumerate}
    \item Brownian motion is a martingale with respect to its natural filtration $(\mathcal{F}_t)_{t \geq 0}$ given by $\calF_t := \sigma\left(B_s: s\leq t\right)$, i.e. for all $0 \leq s \leq t$, $\mathbb{E}\left(B_t|\calF_s\right) = B_s$ almost surely.
    \item If $p \in \mathbb{R}^d$ is a unit vector (under the $\ell_2$ norm), $B_t$ a standard $d$-dimensional Brownian motion, then the process $W_t := \langle p, B_t \rangle$ is a standard 1-dimensional Brownian motion.
    \item For any $\lambda > 0$, the process $(X_t^\lambda)_{t \geq 0}$ \rrcomment{a bit of overloaded notation with what you defined above $B_t^x = B_t + x$.} given by $X_t := \exp\left(\lambda B_t - \frac{\lambda^2}{2}t\right)$ is a non-negative martingale. It is known as \textit{Geometric Brownian motion}.
    \item Brownian motion obeys the \textit{Markov property}. That is, for any measurable set $A \subset \R^d$, $\P(B_t \in A \mid \calF_s) = \P(B_t \in A\mid B_s)$. \rrcomment{Perhaps should be $P(B_t \in A\mid \calF_s)$} 

\end{enumerate}
\end{fact}

As mentioned in Fact~\ref{fact:bm_prop}, one of the most useful properties of Brownian Motion is that it is a martingale. At a high-level, a martingale is a stochastic process where our best guess for where the process will be at a future time is where the process is now. Martingales are of both practical and theoretical interest due to the fact they support strong, time-uniform concentration inequalities. The following classical result is the backbone of almost all time-uniform concentration results, of which we will state a few later.

\begin{fact}[\textbf{Ville's Inequality}]
\label{fact:ville}
Suppose $(X_t)_{t \geq 0}$ is a non-negative martingale. Let $\delta \in (0, 1)$ be an arbitrary fixed parameter. Then,
$$
\P\left(\exists t \geq 0 : X_t \geq \frac{1}{\delta}\right) \leq \delta.
$$

\end{fact}
Note that a standard Brownian Motion $B_t$ itself is not a non-negative martingale. As a result, we cannot apply Fact~\ref{fact:ville} directly. However, do note that $(X^\lambda_t)_{t \geq 0}$, geometric Brownian motion with parameter $\lambda \in \R$, is in fact a non-negative martingale. As a result, some of the concentration results below will leverage this process instead of Brownian motion directly.

One classic result regarding Brownian motion is what is a known as a line-crossing inequality. 

\begin{fact}[\textbf{Line Crossing Inequality for Brownian Motion}]
\label{fact:line_cross}
Suppose $(B_t)_{t \geq 0}$ is a standard Brownian motion. Let $a, b \in \R_{>0}$ be arbitrary positive real numbers. Then,
$$
\P\left(\exists t \geq 0 : B_t \geq at + b\right) \leq e^{-2ab}.
$$

\end{fact}

For a proof of Fact~\ref{fact:line_cross}, see a standard graduate text in probability theory such as Durrett [].

Another concentration result for Brownian motion, which we call a curve crossing inequality (as opposed to line crossing) comes from applying a technique called \textit{the method of mixtures}. The method of mixtures is a technique for martingale concentration that hinges on a simple observation. Suppose $\{(X_t^\lambda)_{t \geq 0}\}_{\lambda \in \R}$ is a family of non-negative martingales (indexed by $\lambda \in \R$), and suppose $\pi(d\lambda)$ is a probability measure on $\R$. Using Fubini's theorem for conditional expectations, it is straightforward to show that the \textit{mixture process} defined as 
$$
Y_t := \int_{\R}X^\lambda_t\pi(d\lambda)
$$
is in fact a non-negative martingale. One can then apply Fact~\ref{fact:ville} to the process $(Y_t)_{t \geq 0}$ to obtain interesting concentration results.

The above paragraph may sound a bit dense on a first pass, but we can illustrate the usefulness of the technique in the following Fact. 

\begin{fact}[\textbf{Curve Crossing Inequality for Brownian Motion}]
\label{fact:mixture}
Let $(B_t)_{t \geq 0}$ be a standard Brownian Motion, and let $\rho >0$ be a fixed positive real number. Then, for any confidence parameter $\delta \in (0,1)$, we have
$$
\P\left(\exists t \geq 0 : B_t > \sqrt{2(t + \rho)\log\left(\frac{t + \rho}{\delta^2\rho}\right)}\right).
$$

\end{fact}

The proof of Fact~\ref{fact:mixture} is already known, and can be found in papers such as [] and []. Nonetheless, since it illustrates how to apply the method of mixtures, we include the proof in the Appendix.

\begin{comment}

Suppose $\beta \in \R^d$ is a utility maximizer for some problem, and that $(\beta_n)_{n \in \N{$


\begin{definition}[\textbf{Noise Reduction Mechanism}]
Suppose $\calB : \calX \times \N \rightarrow E$ is a randomized mechanism which releases $\cal$

\end{definition}


\begin{proposition}
Suppose $\calB$ is a noise reduction mechanism with corresponding privacy bounds $(\epsilon_n)_{n \in \N}$, and suppose $(p_{1, \dots, n})_{n \in \N}$ is a family of densities for $\calB(x, n) = (\beta_1(x), \dots, \beta_n(x))$. For any fixed $n \in \N$, fixed alternative $x' \sim x$, we can see that the privacy loss for $\calB(x, n)$ is given by 
$$
\calL_n(x, x') := \log\left(\frac{p^{x}_{1:n}(\beta_{1:n})}{p^{x'}_{1:n}(\beta_{1:n})}\right) = \log\left(\frac{p^x_n(\beta_n)}{p^{x'}_n(\beta_n)}\right).
$$
That is, the privacy loss of a noise reduction mechanism only depends on the 
\end{proposition}
\end{comment}

==> OldFiles/generalization_and_proof.tex <==
\section{The Generalized Brownian Mechanism and Privacy Loss}
\label{app:gen_mech}

In Section~\ref{sec:bm}, we constructed the Brownian Mechanism and characterized its privacy loss process. In our work, we always made the assumption that the function $f : \calX \rightarrow \R^d$ associated with the Brownian mechanism had $\ell_2$ sensitivity at most 1. In this section, we present a simple variant of the Brownian mechanism which can be applied to functions $f$ which have sensitivity bounded by 1 under \textit{any} matrix norm $||\cdot||_A$.

Before stating the generalized algorithm, we briefly cover the basics of generalized inner products on $\R^d$ and their induced norms. Recall that a matrix $A$ is called \textit{positive definite} if $A$ is symmetric and has strictly positive eigenvalues. Associated with any positive definite matrix $A$ there is a natural inner product $\langle \cdot, \cdot\rangle_A$ which acts on arbitrary vectors $x, y \in \R^d$ as follows:
$$
\langle x, y \rangle_A = x^TAy.
$$
Such an inner product can be written in terms of the standard inner product on $\R^d$ in a variety ways. For instance, we clearly have $\langle x, y \rangle_A = \langle Ax, y \rangle = \langle x, Ay \rangle = \langle A^{1/2}x, A^{1/2}y\rangle$ where $A^{1/2}$ is a matrix square root of $A$. These various identities will prove useful in the analysis below. Given said matrix inner product $\langle \cdot, \cdot \rangle_A$, the associated norm $||\cdot ||_A$ on $\R^d$ is given by
$$
||x||_A = \sqrt{\langle x, x \rangle_A} = \sqrt{x^TA x}
$$
where $x \in \R^d$ is an arbitrary vector. 

Using this notation, we say that a function $f : \calX \rightarrow \R^d$ has $\ell_A$ sensitivity at most $\Delta$ if 
$$
||f(x) - f(x')||_A \leq \Delta \qquad \forall x \sim x' \in \calX.
$$
Observe that the set of vectors which have $\ell_A$ norm at most 1 is precisely the image of the unit ball $\calB_1(0) := \{y \in \R^d : ||y||_2 \leq 1\}$ under the mapping $A^{-1/2}$, i.e.
$$
\{y \in \R^d : ||y||_A \leq 1\} = A^{-1/2}\calB_1(0) = \{A^{-1/2}y \in \R^d : ||y||_2 \leq 1\}. 
$$

This indicates how we should develop a generalized Brownian mechanism for general matrix norms. In particular, instead of adding on a standard Brownian motion $(B_t)_{t \geq 0}$ to a hidden high-dimensional parameter $f(x) \in \R^d$, we should instead add on $(A^{-1/2}B_t)_{t \geq 0}$. This yields the following generalization of Definition~\ref{def:bm}.

\begin{definition}[Generalized Brownian Mechanism]
\label{def:gbm}
For a function $f : \calX \rightarrow \R^d$, a decreasing sequence of times $(t_n)_{n \in \N}$, and an input $x \in \calX$, define the sequence of iterates $(\beta^A_n(x))_{n \in \N}$ by 
$$
\beta_n(x) := f(x) + A^{-1/2}B_{t_n},
$$
where $(B_t)_{t \geq 0}$ is a $d$-dimensional standard Brownian motion. The \textbf{Generalized Brownian Mechanism} associated with a function $f$, sequence of times $(t_n)_{n \in \N}$, and positive-definite matrix $A$ is the function $\calB^A : \calX \times \calT \rightarrow (\R^d)^\ast$, which, when given a dataset $x \in \calX$ and a stopping condition $N \in \calT$, outputs the vector:
$$
\beta^A_{1:N}(x) = (\beta^A_1(x), \beta^A_2(x), \dots, \beta^A_N(x)) = (\beta_1^A(x), \dots, \beta^A_{N((\beta^A_n(x))_{n \in \N})}).
$$


\end{definition}

Given such a mechanism, it is clear that, for any $n \in \N$, any input dataset $x \in \calX$, and any fixed alternative $x' \in \calX$, as in the case of the regular Brownian mechanism, we have the privacy loss decomposition.
$$
\calL_n(x, x') = \log\left(\frac{q^{x}_{t_n, \cdots, t_1}(\beta^A_n, \dots, \beta^A_1)}{q^{x'}_{t_n, \cdots, t_1}(\beta^A_n, \dots, \beta^A_1)}\right) =  \log\left(\frac{q^{x}_{t_n}(\beta^A_n)}{q^{x'}_{t_n}(\beta^A_n)}\right),
$$
where $q^x_{t_n, \dots, t_1}(y_n, \dots, y_1)$ is the joint density of $(\beta^A_1(x), \dots, \beta^A_n(x)) = (f(x) + A^{-1/2}B_{t_1}, \dots, f(x) + A^{-1/2}B_{t_n})$. The second equality follows from the fact that the shifted process $(A^{-1/2}B_{t})_{t \geq 0}$ is also a Markov process. Consequently, the generalized Brownian mechanism is still a noise reduction mechanism. In the following Theorem, we see we get precisely the same bound on the privacy loss process associated with the generalized Brownian mechanism as we do with the Brownian mechanism.

\begin{theorem}[\textbf{Privacy Loss Process for Brownian Motion}]
\label{thm:gen_priv_loss}


Let $\calB_A$ be a generalized Brownian mechanism associated with function $f : \calX \rightarrow \R^d$, sequence of times $(t_n)_{n \in \N}$, and positive definite matrix $A$. Moreover, assume $f$ has $\ell_A$-sensitivity at most 1. Let $x, x' \in \calX$ be arbitrary input datasets, and $(\calL_n(x, x'))_{n \in \N}$ the corresponding privacy loss process. Then, for any $n \in \N$, we have
$$
\calL_n(x, x') = \frac{1}{2t_n}||f(x) - f(x')||_A^2 - \frac{||f(x) - f(x')||_A}{t_n}W_{t_n},
$$
where $(W_t)_{t \geq 0}$ is some standard one-dimensional Brownian motion. Consequently, if $x$ and $x'$ are neighbors, we have
$$
\calL_n(f(x), f(x')) \leq \frac{1}{t_n}|W_{t_n}| + \frac{1}{2t_n}.
$$
\end{theorem}
\begin{proof}
The second statement is trivial and follows from our assumption of bounded $\ell_A$ sensitivity.

Without loss of generality, and for the sake of simplicity, we can assume $f(x) = 0$. Observe that, for $y \in \R^d$, the random vector $f(x') + A^{-1/2}B_t$ is a multivariate Gaussian distributed according to $\calN(f(x'), A^{-1})$ with Lebesgue density
$$
q_{t_n}^{x'}(y) \propto \exp\left(-\frac{1}{2t}||y  - f(x')||^2_A\right).
$$

Consequently, the privacy loss can be written as 
\begin{align*}
\calL_n(x, x') &= \log\left(\frac{q^x_{t_n}( A^{-1/2}B_{t_n})}{q_{t_n}^{x'}(A^{-1/2}B_{t_n})}\right) \\
&= \frac{1}{2t_n}\left( - ||A^{-1/2}B_{t_n}||_A^2 + ||A^{1/2}B_{t_n} - f(x')||_A^2\right) \\
&= -\frac{1}{t_n}\langle A^{-1/2}B_{t_n}, f(x') \rangle_A + \frac{1}{2t_n}||f(x')||_A^2 \\
&= -\frac{||A^{1/2}f(x')||_2}{t_n}\left\langle A^{-1/2}B_{t_n}, A^{-1/2}\frac{A^{1/2}f(x')}{||A^{1/2}f(x')||_2}\right\rangle_A + \frac{1}{2t_n}||f(x')||_A^2 \\
&= -\frac{||f(x')||_A}{t_n}\left\langle B_{t_n}, \frac{A^{1/2}f(x')}{||A^{1/2}f(x')||_2}\right\rangle + \frac{1}{2t_n}||f(x')||_A^2 \\
&= -\frac{||f(x')||_A}{t_n}W_{t_n} + \frac{1}{2t_n}||f(x')||_A^2,
\end{align*}
which proves the desired result.
\end{proof}

Note that, if we take $A = I_d$, the $d$-dimensional identity matrix, Theorem~\ref{thm:gen_priv_loss} yields Theorem~\ref{thm:bm_ploss} as a special case. Like any noise reduction mechanism, the generalized Brownian mechanism can be augmented to obtain provable accuracy guarantees, as outlined in Section~\ref{sec:aug}. This generalized mechanism allows for a refined outlook on function sensitivity, as $\ell_2$-sensitivity may be overly pessimistic in some situations.

==> OldFiles/generalized_above_threshold.tex <==
\section{Reduced Above Threshold}
\label{app:rat}


In this Appendix, we introduce a generalization of the classic AboveThreshold procedure called ReducedAboveThreshold (or RAT, for short). Recall that AboveThreshold was a differentially private algorithm with the following guarantee: with high-probability, the algorithm yields the first index of a query that is ''close" to being over a desired threshold (where the measure of closeness is inversely proportional to the privacy parameter $\epsilon$). In Section~\ref{}, we generalized the results of \cite{ligett2017accuracy} to show that AboveThreshold can actually be used to augment any noise reduction mechanism (such as our Brownian mechanism, for instance).

However, we noted that AboveThreshold was a bit of a mismatch for the noise reduction framework. Take the example of utility maximization: in each round, a noise reduction mechanism yields successively more accurate estimates of the utility-maximizing parameter. To obtain this increased accuracy, the mechanism ultimately pays the price of decreased privacy over time. AboveThreshold, as noted above, \textit{does not} give an improved utility guarantee as time progresses. This is because the variance of the Laplace noise added in each round is the same. An ideal mechanism should have the flexibility to match the privacy level of the noise reduction mechanism at any point in time, ultimately providing stronger utility guarantees as we view increasingly accurate parameter estimates.

This is precisely the goal of ReducedAboveThreshold. By decreasing the variance of the Laplace noise added in each iteration to the query, we can ultimately provide stronger utility guarantees as we view successively more parameter estimates. The only subtlety is that, as noted in Algorithm~\ref{alg:at}, Laplace noise is only added once to the threshold at the beginning of time in AboveThreshold. As seen in \cite{dwork2014algorithmic}, this single addition of noise is essential for allowing the proof of privacy to go through. We can circumvent this seeming roadblock by leveraging noise reduction, however. In particular, as will be seen shortly, if we \textit{reduce} the level of Laplace noise on the threshold over time using Algorithm~\ref{alg:lnr}, we can actually maintain privacy loss guarantees. We formalize this now in Algorithm~\ref{alg:rat}.

\begin{algorithm}[!h]
\caption{ReducedAboveThreshold}\label{alg:rat}
\begin{algorithmic}
\Require $(\epsilon_n)_{n \in [K]}$ increasing sequence of privacy parameters, $(T_n)_{n \in [K]}$ sequence of thresholds, input database $x \in \calX$, adaptively chosen sequence of $\Delta$-sensitive functions $(f_n)_{n \in [K]}$.
\State Let $(\zeta_n)_{n \in [K]}$ be iterates of Algorithm~\ref{alg:lnr} with privacy parameters $(\epsilon_n/2\Delta)_{n \in [K]}$.
\For{$n \in [K]$}
    \State $\xi_n \sim Lap\left(\frac{4\Delta}{\epsilon_n}\right)$
    \If{$f_n(x) + \xi_n \geq T_n + \zeta_n$}
        \State Print $1$
        \State HALT
    \Else
        \State Print $0$
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

First, we observe that Algorithm~\ref{alg:rat} is a strict generalization of the classic AboveThreshold mechanism. As such, we expect it to maintain somewhat similar theoretical guarantees. The key difference is that the privacy loss will now be proportional to the level of noise added on the final iterate (that is, the iteration printing $1$). That is, if $N$ denotes the (random) round on which the algorithm halts, our privacy loss will be bounded by $\epsilon_N$. Correspondingly, the (random) utility guarantee will be inversely proportional to the privacy parameter on the final iteration, i.e. inversely proportional to $\epsilon_N$.This is desirable in a noise-reduction setting, as we want to obtain improvable utility guarantees as we sacrifice privacy.

\begin{theorem}[\textbf{Guarantees of ReducedAboveThreshold}]
\label{thm:rat}
Suppose $(\epsilon_n)_{n \in [K]}$ is a finite, increasing sequences of privacy parameters, $(f_n)_{n \in [K]}$ is a sequence of $\Delta$-sensitive functions, $(T_n)_{n \in [K]}$ a $\R$-valued sequence of thresholds, and $x \in \calX$ an input database. Let $N$ denote the random number of iterations Algorithm~\ref{alg:rat} runs for. For any neighboring dataset $x' \sim x \in \calX$, let $\calL^{RAT}(x, x')$ denote the privacy loss of Algorithm~\ref{alg:rat}. Then, we have the following random bound on privacy loss:
$$
\calL^{RAT}(x, x') \leq \epsilon_N.
$$

Moreover, define the sequence of utility parameters $(\eta_n)_{n \in [K]}$ by
$$
\eta_n := \frac{4\Delta}{\epsilon_n}\left(\log\left(\frac{2}{\gamma}\right) - \log(p_n)\right),
$$
where $\sum_{n \in [K]}p_n = 1$. Then, with probability at least $1 - \gamma$, we have 
$$
f_N(x) \geq T_N - \eta_N,
$$
where $N$ is the random time outlined above.
\end{theorem}

Note that, in the case $(\epsilon_n)_{n \in [K]}$ is taken to be a constant sequence, Theorem~\ref{thm:rat} exactly recovers the traditional guarantees of AboveThreshold, justifying that RAT is a strict generalization of AboveThreshold. We prove the above theorem in two parts. First we prove the utility guarantee, which ultimately boils down to a simple union bound argument. Then, we prove the privacy guarantee. The proof here requires leveraging the unique structure of the Laplace Noise Reduction mechanism-- in particular the fact that (a) its marginals follow a Laplace distribution and (b) that the process itself is Markovian. We start with the proof of accuracy:

\begin{proof}[\textbf{Accuracy of RAT}]
The accuracy guarantee follows by applying two simple union bounds. Observe we have the probability bound
$$
\P\left(\bigcup_{n \in \N}\left\{|\xi_n| \geq \eta_n\right\}\right) \leq \sum_{n \in \N}\P(|\xi_n| \geq \eta_n) = \sum_{n \in \N}\exp\left(-\frac{\epsilon_n\eta_n}{4\Delta}\right) = \frac{\gamma}{2}\sum_{n \in \N}p_n = \frac{\gamma}{2}.
$$

Likewise, we have
$$
\P\left(\bigcup_{n \in \N}\left\{|\zeta_n| \geq \eta_n\right\}\right) \leq \sum_{n \in \N}\P(|\zeta_n| \geq \eta_n) \leq \sum_{n \in \N}\exp\left(-\frac{\epsilon_n\eta_n}{2\Delta}\right) \leq \frac{\gamma}{2}\sum_{n \in \N}p_n = \frac{\gamma}{2}.
$$
Consequently, with probability at least $1 - \gamma$, for all $n \in \N$, we simultaneously have $|\xi_n| \leq \frac{\eta_n}{2}$ and $|\zeta_n| \leq \frac{\eta_n}{2}$. In particular, when the algorithm halts, this directly yields
$$
f_N(x) \geq T_N - \eta_N.
$$
\end{proof}

Now, we proceed to the proof of privacy of Algorithm~\ref{alg:rat}, which is ultimately a bit more involved.

\begin{proof}
Without loss of generality, we can assume $T_1 = T_2 = \cdots = T_n = T$ for some single threshold $T$, as we can always set $f'_n(x) := f_n(x) + T - T_n$. Let $(\alpha_n)_{n \in [K]}$ denote the random sequence of $\{0, 1\}$ outputs of Algorithm~\ref{alg:rat} run on the parameters stated in Theorem~\ref{thm:rat}. If $\P_x(\alpha_{1:n} \in \cdot)$ denotes the probability distribution of the first $n$ outputs, define the random variables.
$$
L_n(x, x') := \log\left(\frac{\P_x\left(\alpha_{1:n} = 0^{n - 1}1\right)}{\P_{x'}\left(\alpha_{1:n} = 0^{n - 1}1\right)}\right) \leq \epsilon_n
$$

If $N := \inf\{n \in \N: \alpha_n = 1\}$ is the time at which RAT halts, then we have we have the following characterization of the privacy loss of RAT
$$
\calL^{RAT}(x, x') = L_N(x, x').
$$
Thus, it suffices to show that $L_n(x, x') \leq \epsilon_n$, for all $n \in [K]$. To achieve this goal, we essentially rework to the proof of correctness for AboveThreshold found in \cite{}. However, this is not quite straightforward, as we need need to handle the fact that the threshold is randomly changing over time.

First, observe that we can write the desired probability as
$$
\P_x\left(\alpha_{1:n} = 0^{n - 1}1\right) = \int_{\R^n}g_T(\tau_1, \dots, \tau_n)\left(\prod_{i = 1}^{n - 1}\P(f_i(x) + \xi_i < \tau_i)\right)\P(f_n(x) + \xi_n \geq \tau_n)d\vec{\tau}
$$

where $g_T$ represents the density for the joint distribution of $(T + \zeta_1, \dots, T + \zeta_n)$, where $(\zeta_n)_{n \in \N}$ is the process obtained from the Laplace Noise Reduction framework. We now need three inequalities. The first two are commonplace and are used in \cite{}, so we do note provide a proof. The third of which is a product of our novel RAT mechanism, and hence we provide a proof. The inequalities are as follows.
\begin{enumerate}
    \item For $i < n$ and fixed $\tau_i$, $\P(f_i(x) + \xi_i < \tau_i) \leq \P(f_i(x') + \xi_i < \tau_i + \Delta)$,
    \item for $i = n$ and fixed $\tau_n$, $\P(f_n(x) + \xi_n \geq \tau_n) \leq e^{\epsilon_n'}$, and
    \item for any $\tau_{1:n} \in \R^n$, $g_T(\tau_1, \dots, \tau_n) \leq g_T(\tau_1 + \Delta, \dots, \tau_n + \Delta)$.
\end{enumerate}

We now prove the third inequality. In particular, we have
\begin{align*}
    \frac{g_T(\tau_1, \dots, \tau_n)}{g_{T - \Delta}(\tau_1, \dots, \tau_n)} &= \frac{g_T(\tau_n)g_T(\tau_1, \dots, \tau_{n - 1}|T + \zeta_n = \tau_n)}{g_{T - \Delta}(\tau_n)g_{T - \Delta}(\tau_1, \dots, \tau_{n - 1}|T + \zeta_n - \Delta = \tau_n)} \\
    &= \frac{g_{T}(\tau_n)}{g_{T - \Delta}(\tau_n)} \leq e^{\epsilon_n}
\end{align*}
where the first equality follows from applying Bayes rule to the joint densities of the noisy thresholds, and the second equality follows from the fact that the process $(\zeta_n)_{n \in \N}$ is Markovian, per Lemma~\ref{lem:lnr_guar}. The final inequality follows again from Lemma~\ref{lem:lnr_guar}, which tells us that the marginal distributions of $\zeta_n$ are $Lap\left(\frac{4\Delta}{\epsilon_n}\right)$. Now, observe that by a simple shift of parameters we have
$$
g_{T - \Delta}(\tau_1, \dots, \tau_n) = g_T(\tau_1 + \Delta, \dots, \tau_n + \Delta).
$$
Plugging this in, we have
\begin{align*}
   \P_{x}\left(\alpha_{1:n} = 0^{n - 1}1\right) &= \int_{\R^n}g_T(\tau_1, \dots, \tau_n)\left(\prod_{i = 1}^{n - 1}\P(f_i(x) + \xi_i < \tau_i)\right)\P(f_n(x) + \xi_n \geq \tau_n)d\vec{\tau} \\
   &\leq e^{\epsilon_n}\int_{\R^n}g_{T - \Delta}(\tau_1, \dots, \tau_n)\left(\prod_{i = 1}^{n - 1}\P(f_i(x) + \xi_i < \tau_i)\right)\P(f_n(x) + \xi_n \geq \tau_n)d\vec{\tau} \\
    &\leq e^{\epsilon_n + \epsilon_n'}\int_{\R^n}g_{T - \Delta}(\tau_1, \dots, \tau_n)\left(\prod_{i = 1}^{n - 1}\P(f_i(x') + \xi_i < \tau_i + \Delta)\right)\P(f_n(x) + \xi_n \geq \tau_n + \Delta)d\vec{\tau} \\
    &= e^{\epsilon_n + \epsilon_n'}\int_{\R^n}g_{T}(\tau_1 + \Delta, \dots, \tau_n + \Delta)\left(\prod_{i = 1}^{n - 1}\P(f_i(x') + \xi_i < \tau_i + \Delta)\right)\P(f_n(x) + \xi_n \geq \tau_n + \Delta)d\vec{\tau} \\
    &= \P_{x'}\left(\alpha_{1:n} = 0^{n - 1}1\right).
\end{align*}
Rearranging furnishes the desired result.
\end{proof}




==> OldFiles/laplace_motion.tex <==
\section{Laplace Motion}

In their work, \cite{koufogiannis2015gradual} construct a discrete time Markov process having Laplace marginal distributions. 

\begin{definition}[Discrete time Laplace Motion]
Given a increasing sequence of strictly positive times $(t_n)_{n \geq 1}$ fixed in advance, first set $t_0 := 0$, and then define the random variables $(\zeta_n)_{n \geq 1}$ by
$$
\zeta_n := \begin{cases}
0 & \text{with probability } \frac{t_{n-1}^2}{t_n^2} \\
\textrm{Lap}(t_n) & \text{with probability } 1 - \frac{t_{n - 1}^2}{t_n^2}.
\end{cases}
$$
Then, the process $(Z_n)_{n \in \N_0}$ given by $Z_0 = 0$ and
$$
Z_n := 
% \begin{cases}
% 0 & \text{if } n = 0 \\
% \textrm{Lap}(t_1) & \text{if } n = 1 \\
Z_{n - 1} + \zeta_n , \text{ for } n \geq 1,
% & \text{otherwise}.
% \end{cases}
$$
is called a \textit{discrete Laplace motion} associated with $(t_n)_{n \geq 1}$.

\end{definition}

The following can be easily checked.

\begin{lemma}
Suppose $(Z_n)_{n \in \N}$ is a discrete Laplace motion associated with times $(t_n)_{n \geq 1}$. Then, we have:
\begin{enumerate}
    \item $Z_n \sim \textrm{Lap}(t_n)$.
    \item $(Z_n)_{n \in \N}$ is a Markov process.
    \item $(Z_n)_{n \in \N}$ is a martingale.
\end{enumerate}
\end{lemma}

In this work, we provide a natural extension of the discrete time Laplace motion to continuous time, constructing a process which we just entitle \textit{Laplace motion}. 

\begin{definition}[Laplace Motion] Let $\epsilon > 0$ be arbitrary. Let $(N(t))_{t \geq \epsilon}$ be an inhomogeneous Poisson process with intensity function $\lambda(t) := \frac{2}{t}$. Define the increasing sequence of random times $(T_n)_{n \in \N}$ by $T_n := \inf\{t \geq \epsilon : N(t) \geq  n\}$ and $T_0 := \epsilon$, i.e. $T_n$ is the random time associated with the $n$th jump of $(N(t))_{t \geq \epsilon}$. Then, the \textit{Laplace motion} started at $\epsilon > 0$ is the continuous time jump process given by
$$
Z(t) := \textrm{Lap}(\epsilon) + \sum_{n \leq N(t)}\textrm{Lap}(T_n).
$$

\end{definition}

By construction, $Z(t)$ is a Markov process with independent increments. However, it is not clear that $Z(t) \sim \mathrm{Lap}(t)$. We now prove this.

\begin{theorem}
Let $(Z(t))_{t \geq 0}$ by a Laplace motion started at $\epsilon > 0$. Then, for any $t \geq \epsilon$, we have
$$
Z(t) \sim \mathrm{Lap}(t).
$$


\end{theorem}
\begin{proof}
Recall that if $X \sim \mathrm{Lap}(s)$, then $X$ has characteristic function $\varphi_s$ given by
$$
\varphi_s(\lambda) = \frac{1}{1 + \lambda^2 s^2}.
$$
Let $\phi$ denote the characteristic function of $Z(t) - Z(\epsilon)$. Since $Z(\epsilon)$ and $Z(t) - Z(\epsilon)$ are independent, to show $Z(t) \sim \mathrm{Lap}(t)$, it suffices to show that
$$
\phi(\lambda) = \frac{\varphi_t(\lambda)}{\varphi_\epsilon(\lambda)} = \frac{1 + \lambda^2 \epsilon^2}{1 + \lambda^2 t^2}.
$$

Now, observe that the inhomogenous Poisson process $(N(t))_{t \geq \epsilon}$ can be written as $(\widetilde{N}(e^{t/2}))_{t \geq \log(\epsilon^2)}$ where $\widetilde{N}$ is a homogeneous Poisson process with rate $\lambda = 1$ on $[\log(\epsilon^2), \infty)$. In terms of the process $\widetilde{N}$, we can consider the process $(\widetilde{Z}(t))_{t \geq \log(\epsilon^2)}$ given by
$$
\widetilde{Z}(t) = \mathrm{Lap}(\epsilon) + \sum_{n  \leq \widetilde{N}(t)}\mathrm{Lap}\left(e^{\widetilde{T}_n/2}\right),
$$
where $\widetilde{T}_n := \inf\{t \geq \log(\epsilon^2) : \widetilde{N}(t) \geq n\}$. It is easy to see that $\widetilde{Z}(\log(t^2)) - \widetilde{Z}(\log(\epsilon^2)) =_d Z(t) - Z(\epsilon)$.

Leveraging this identity, it follows that we have
\begin{align*}
    \phi(\lambda) &= \E\left[e^{i \lambda (Z(t) - Z(\epsilon))}\right] = \E\left[e^{i \lambda (\widetilde{Z}(\log(t^2)) - \widetilde{Z}(\log(\epsilon^2)))}\right] \\
    &= \sum_{n = 0}^\infty \frac{\epsilon^2}{t^2}\frac{\left[\log(t^2/\epsilon^2)\right]^n}{n!}\int_{\log(\epsilon^2) \leq u_1 < u_2 < \cdots < u_n \leq \log(t^2)}f^{(n)}(u_1, \dots, u_n)\prod_{i = 1}^n\E\left[e^{i\lambda \mathrm{Lap}(e^{u_i/2})}\right]d\mathbf{u} \\
    &= \frac{\epsilon^2}{t^2}\sum_{n = 0}^\infty \int_{\log(\epsilon^2) \leq u_1 < u_2 < \cdots < u_n \leq \log(t^2)}\prod_{i = 1}^n\frac{1}{1 + \lambda^2e^{u_i}}d\mathbf{u} \\
    &=: \square.
\end{align*}

In the above, $f^{(n)}(u_1, \dots, u_n) := \frac{n!}{[\log(t^2/\epsilon^2)]^n}$ is the distribution of the order statistics $(U_{(1)}, \dots, U_{(n)})$ of $n$ i.i.d. random variables that are uniform on $[\log(\epsilon^2), \log(t^2)]$. Essentially, what we have done is \textit{first} conditioned of the number of Poisson arrivals that occur in the interval $[\log(\epsilon^2), \log(t^2)]$. Then, on the event $\{N(t) = n\}$, we condition again on the location of the $n$ arrivals, which we know to be uniformly distributed across the time interval. Once the arrival locations are known, we can compute the conditional characteristic function, which is the the product of characteristic functions as illustrated in the integral above.  

Now, we show inductively that
$$
\int_{\log(\epsilon^2) \leq u_1 < u_2 < \cdots < u_n \leq \log(t^2)}\prod_{i = 1}^n\frac{1}{1 + \lambda^2e^{u_i}}d\mathbf{u} = \frac{1}{n!}\left[\log\left(\frac{t^2}{\epsilon^2}\frac{1 + \lambda^2 \epsilon^2}{1 + \lambda^2 t^2}\right)\right]^n.
$$

The base case of $n = 1$ is trivially true. Now, we have that
\begin{align*}
&\int_{\log(\epsilon^2) \leq u_1 < u_2 < \cdots < u_n \leq \log(t^2)}\prod_{i = 1}^n\frac{1}{1 + \lambda^2e^{u_i}}d\mathbf{u} \\
&= \int_{u_1 = \log(\epsilon^2)}^{\log(t^2)}\frac{1}{1 + \lambda^2e^{u_1}}\int_{u_1 < u_2 < \dots < u_n}\prod_{i = 2}^n\frac{1}{1 + \lambda^2 e^{u_i}}d\mathbf{u}_{-1}du_1 \\
&= \frac{1}{(n - 1)!}\int_{u = \log(\epsilon^2)}^{\log(t^2)}\frac{1}{1 + \lambda^2e^u}\left[\log\left(\frac{t^2}{e^u}\frac{1 +\lambda^2 e^u}{1 + \lambda^2 t^2}\right)\right]^{n - 1}du \\
&= \frac{1}{n!}\int_{\log(\epsilon^2)}^{\log(t^2)}\frac{d}{du}\left[\log\left(\frac{t^2}{e^u}\frac{1 + \lambda^2 e^u}{1 + \lambda^2 t^2}\right)\right]^n du \\
&= \frac{1}{n!}\left[\log\left(\frac{t^2}{\epsilon^2}\frac{1 + \lambda^2 \epsilon^2}{1 + \lambda^2 t^2}\right)\right]^n.
\end{align*}
Leveraging this identity, we have that
\begin{align*}
    \square &= \frac{\epsilon^2}{t^2}\sum_{n = 0}^\infty \frac{1}{n!}\left[\log\left(\frac{t^2}{\epsilon^2}\frac{1 + \lambda^2 \epsilon^2}{1 + \lambda^2 t^2}\right)\right]^n \\
    &= \frac{\epsilon^2}{t^2}\exp\left(\log\left(\frac{t^2}{\epsilon^2}\frac{1 + \lambda^2 \epsilon^2}{1 + \lambda^2 t^2}\right)\right) \\
    &= \frac{1 + \lambda^2\epsilon^2}{1 + \lambda^2 t^2}.
\end{align*}
This proves the desired result.
\end{proof}


==> OldFiles/measure_theory_background.tex <==
\section{Measure-Theoretic Background}
In this section, we provide the necessary measure-theoretic background to be fully formal throughout the rest of this work. For a more in-depth background on the measure-theoretic underpinnings of this work, we recommend the reader refer to a standard graduate text in probability theory such as Durrett~\cite{durrett2019probability}, for instance.

To start, the most basic measure-theoretic notion we will need is that of a \textit{probability space}.

\begin{definition}
\label{def:prob_space}
A \textit{probability space} is a triple $(\Omega, \calF, \P)$ where 
\begin{enumerate}
    \item $\Omega$ is a set,
    \item $\calF$ is a $\sigma$-algebra, i.e. a subset of the power set $2^\Omega$ that is closed under countable unions, countable intersections, and complements, and
    \item $\P : \calF \rightarrow [0, 1]$ is a probability measure.
\end{enumerate}

A \textit{measurable space} is just a tuple $(\calY, \calG)$ of a set $\calY$ and $\sigma$-algebra $\calG$ lacking an associated probability measure.
\end{definition}
Heuristically, $\Omega$ be be viewed as an abstract sample space containing the ''random seeds" for the random variables we will consider from this point forward. Likewise, $\calF$ can be viewed as the set of all possible events that can occur. A probability measure, then, just assign probabilities to events in $\calF$ in accordance with the properties of a measure. We ultimately need probability spaces and measurable spaces to formalize the notion of \textit{random variables} and their associated laws.

\begin{definition}
Let $(\Omega, \calF, \P)$ be a probability space and $(\calY, \calG)$ a measurable space. Then, a function $X : \Omega \rightarrow \calY$ is called a \textit{random variable} if it is measurable, i.e. $X^{-1}(G) \in \calF$ for all $G \in \calG$.

Every random variable has associated with it a law $\mu_X : \calG \rightarrow [0, 1]$ assigning probabilities to the events in $\calG$ by $\mu_X(G) := \P(X \in G) := \P(X^{-1}(G))$.


\end{definition}

Random variables can just be seen as taking in a random seed in $\Omega$ and producing some random outcome in the output measurable space $(\calY, \calG)$. The law of a random variable just gives the probability of witnessing events in the outcome space.

With the aforementioned formalization of probability spaces and random variables, we begin formalizing how algorithms should be viewed throughout this work. Typically, algorithms are viewed as a randomized mappings $A : \calX \rightarrow \calY$, where $\calX$ is the space of all input datasets, and $(\calY, \calG)$ is some measurable space. However, for the sake of formalism, for any neighboring datasets $x \sim x'$, we can view the $A(x)$ and $A(x')$ as random variables both defined on a common probability space $(\Omega, \calF, \P)$, both with respective laws $\mu_x, \mu_{x'}$ defined on the measurable space $(\calY, \calG)$. Sometimes, we will need to consider an adaptively chosen sequence of algorithms $(A_n)_{n \in I}$ where the indexing set satisfies either $I = [K]$ for some finite $K \in \N$ or $I = \N$. In this case, for any neighbors $x \sim x' \in \calX$, we view $A_n(x)$ and $A_n(x')$ as random variables on a probability space $(\Omega, \calF, \P)$ simultaneously for all $n \in I$.

Often times, we will need to formalize the notion of accumulating information over time. We do this through the notion of a filtration, which we will define shortly. Before we do this, we need to define the notion of a $\sigma$-algebra generated by a collection of random variables. Given $\calA \subset \calF$, the \textit{$\sigma$-algebra generated by $\calA$}, denoted as $\sigma(\calA)$, is the smallest $\sigma$-algebra containing $\calA$. If $\{X_i\}_{i \in I}$ is a collection of random variable indexed by some set $I$, the \textit{$\sigma$-algebra generated by $\{X_i\}_{i \in I}$}, denoted by $\sigma(X_i : i \in I)$, is just $\sigma(\calA)$ for $\calA := \left\{\bigcup_{i \in I}X_i^{-1}(G_i) : G_i \in \calG, \forall i \in I\right\}$. Now, we can formal define filtrations.

\begin{definition}
Given a $\sigma$-algebra $\calF$, an sequence of $\sigma$-algebras $(\calF_n)_{n \in \N}$ is called a \textit{filtration of $\calF$} if
\begin{enumerate}
\item $\calF_n \subset \calF_{n + 1}$, for all $n \in \N$, and
\item $\calF_n \subset \calF$.
\end{enumerate}

If $(X_n)_{n \in \N}$ is a sequence of random variables taking values in the measurable space $(\calY, \calG)$, the corresponding \textit{natural filtration of $\calF$ associated with $(X_n)_{n \in \N}$} is the filtration $(\calF_n)_{n \in \N}$ given by $\calF_n := \sigma(X_m : m \leq n)$.

\end{definition}



==> ack.tex <==
\section{Acknowledgements}

AR acknowledges support from NSF DMS 1916320 and an ARL IoBT CRA grant. Research reported in this paper was sponsored in part by the DEVCOM Army Research Laboratory under Cooperative Agreement W911NF-17-2-0196 (ARL IoBT CRA). The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation herein.

ZSW and JW were supported in part by the NSF CNS2120667, a CyLab 2021 grant, a Google Faculty Research Award, and a Mozilla Research Grant.

JW acknowledges support from NSF GRFP grants DGE1745016 and DGE2140739.

==> appendices/bm_proofs.tex <==
\section{Proofs From Section~\ref{sec:bm}}
\label{app:bm}

\begin{figure}
\centering
    \subfloat[Variance of Noise vs. Privacy Loss]{
        \includegraphics[width=0.4\textwidth]{figs/var_vs_ploss.png}
        \label{fig:bound:var_pl}
    }
    \subfloat[Privacy Loss vs. Variance of Noise]{
        \includegraphics[width=0.4\textwidth]{figs/ploss_vs_var.png}
        \label{fig:bound:pl_var}
    }
    
    \caption{
    A comparison of the linear and mixture boundaries, both optimized for tightness at $\epsilon = 0.3$ with $\delta = 10^{-6}$. The first plot directly plots the corresponding bounds as in Theorem~\ref{thm:priv_bound}. The second plot inverts the boundaries, showing the variance necessary to meet a target privacy level. 
    %In both plots, the linear bound demonstrates improved tightness at the privacy level optimized for. On the other hand, the mixture boundary demonstrates greater \textit{overall} tightness.
    }
    \label{fig:bound}
\end{figure}

Here, we prove the results from Section~\ref{sec:bm}. We start by showing that $\BM$ is in fact a noise-reduction mechanism, per the condition in Definition~\ref{def:nr}.



\begin{proof}[\textbf{Proof of Lemma~\ref{lem:bm_nr}}]

For any initial value $\mu \in \R^d$ and any $n \geq 1$, let $p^\mu_{1:n}$ denote the joint density of $B_{T_n}, \dots, B_{T_1}$ where $(B_t)_{t \geq 0}$ is a Brownian motion started at $\mu$ and $T_n := T_n(x)$ is a time function. We have the decomposition
\[
p_{1:n}^\mu\left(B_{T_n}, \dots, B_{T_1}\right) \propto \exp\left( - \frac{(B_{T_1} - \mu)^2}{2T_1}\right)\prod_{m = 2}^n \exp\left(\frac{-(B_{T_m} - \mu - \frac{T_m}{T_{m - 1}}(B_{T_{m -1}} - \mu))^2}{2(T_{m - 1} - T_m)}\cdot \frac{T_{m -1}}{T_m}\right).
\]

This decomposition follows as $B_{T_1} \sim \calN(\mu, T_1)$, and, given $B_{T_1}, \dots, B_{T_{m - 1}}$, we have that $B_{T_m} \sim \calN\left(\mu + \frac{T_m}{T_{m - 1}}(B_{T_{m - 1}} - \mu), \frac{(T_{m - 1} - T_m)T_m}{T_{m - 1}}\right)$, as $B_{T_m}$ is conditionally distributed as a Brownian bridge. 
Now, a straightforward calculation yields the equivalence
\begin{align*}
    p^\mu_{1 : n}(B_{T_n}, \dots, B_{T_1}) &\propto \exp\left( - \frac{(B_{T_1} - \mu)^2}{2T_1}\right)\prod_{m = 2}^n \exp\left(\frac{-(B_{T_m} - \mu - \frac{T_n}{T_{m - 1}}(B_{T_{m -1}} - \mu))^2}{2(T_{m - 1} - T_m)}\cdot \frac{T_{m -1}}{T_m}\right) \\
    &= \exp\left(\frac{-(B_{T_n} - \mu)^2}{2T_n}\right)\prod_{m = 2}^n \exp\left(\frac{-(B_{T_{m - 1}} - B_{T_m})^2}{2(T_{m - 1} - T_m)}\right).
\end{align*}
Hence, for any two mean vectors $\mu, \mu' \in \R^d$, we can decompose the ratio of densities as 
\[
\frac{p^\mu(B_{T_n}, \dots, B_{T_1})}{p^{\mu'}(B_{T_n}, \dots, B_{T_1})} = \frac{\exp\left(\frac{-(B_{T_n} - \mu)^2}{2T_n}\right)}{\exp\left(\frac{-(B_{T_n} - \mu')^2}{2T_n}\right)},
\]
which is just the ratio between the density of a $\calN(\mu, T_n)$ random variable evaluated at $B_{T_n}$ and the density of a $\calN(\mu', T_n)$ random variable evaluated at $B_{T_n}$, proving precisely the desired result.
\end{proof}


\begin{comment}
\begin{proof}[\textbf{Proof of Lemma~\ref{lem:bm_nr}}]
Let $x \in \calX$ be a fixed input dataset and $x'$ a neighboring dataset. For any increasing sequence of times $t_1 < t_2 < \dots < t_n$ and point $y \in \R^d$, let $p^y_{t_1, \dots, t_n}$ denote the joint density of $(y + B_{t_1}, \dots, y + B_{t_n})$. Since $p^{y}$ is just the joint density for a Brownian motion started at $y$, applying Bayes rule and the Markov property, it follows that, for any $\beta_1, \dots, \beta_n \in \R^d$,
\begin{equation}
\label{eq:bm_bayes}
p^{y}_{t_1, \dots, t_n}(\beta_1, \dots, \beta_n) = p^y_{t_1}(\beta_1)p^{\beta_1}_{t_2 -t_1, \dots, t_n -t_1}(\beta_2, \dots, \beta_n).
\end{equation}
The strong Markov property \citep{durrett2019probability} will yield that the above is true even when the selected times are random. Note that $\calL_{1:n}^{\BM}(x, x')$, the privacy loss between $\BM_{1:n}(x)$ and $\BM_{1:n}(x')$, is given by
\[
\calL^{\BM}_{1:n}(x, x') = \log\left(\frac{p^{f(x)}_{T_n(x), \dots, T_1(x)}(\BM_n(x), \dots, \BM_1(x))}{p^{f(x')}_{T_n(x), \dots, T_1(x)}(\BM_n(x), \dots, \BM_1(x))}\right).
\]

Likewise, $\calL_n^{\BM}(x, x')$, the privacy loss between $\BM_n(x)$ and $\BM_n(x')$, is given by
\[
\calL^{\BM}_n(x, x') = \log\left(\frac{p^{f(x)}_{T_n(x)}(\BM_n(x))}{p^{f(x')}_{T_n(x)}(\BM_n(x))}\right).
\]
Applying Equation~\eqref{eq:bm_bayes}, we have
\begin{align*}
\calL^{\BM}_{1:n}(x, x') &= \log\left(\frac{p^{f(x)}_{T_n(x), \dots, T_1(x)}(\BM_n(x), \dots, \BM_1(x))}{p^{f(x')}_{T_n(x), \dots, T_1(x)}(\BM_n(x), \dots, \BM_1(x))}\right) \\
&= \log\left(\frac{p^{f(x)}_{T_n(x)}(\BM_n(x))}{p^{f(x')}_{T_n(x)}(\BM_n(x))}\right) + \log\left(\frac{p^{\BM_n(x)}_{T_{n - 1}(x) - T_n(x), \dots, T_1(x) - T_n(x)}(\BM_{n - 1}(x), \dots, \BM_1(x))}{p^{\BM_n(x)}_{T_{n - 1}(x) - T_n(x), \dots, T_1(x) - T_n(x)}(\BM_{n - 1}(x), \dots, \BM_1(x))}\right) \\
&= \log\left(\frac{p^{f(x)}_{T_n(x)}(\BM_n(x))}{p^{f(x')}_{T_n(x)}(\BM_n(x))}\right) = \calL^{\BM}_n(x, x'),
\end{align*}
proving the desired result.

\end{proof}
\end{comment}
We now prove Theorem~\ref{thm:bm_ploss}, which gives a closed form characterization of the Brownian mechanism. In what follows, we use the same notation for the density of Brownian motion as in the above proof.

\begin{proof}[\textbf{Proof of Theorem~\ref{thm:bm_ploss}}]
The second statement of the theorem is trivial and follows from our assumption of bounded $\ell_2$ sensitivity. Hence, we only prove the first statement below.

Without loss of generality, and for the sake of simplicity, we can consider the function $g(y) := f(y) - f(x)$, as then $g(x) = 0$. Observe that, for $y \in \calX$, the vector $g(y) + B_t$ has Lebesgue density
\[
p_{t}^{g(y)}(\beta) \propto \exp\left(-\frac{1}{2t}||\beta  - g(y)||^2_2\right).
\]

Consequently, the privacy loss can be written as 
\begin{align*}
\calL_n^{\BM}(x, x') &= \log\left(\frac{p^{0}_{T_n(x)}(B_{T_n(x)})}{p_{T_n(x)}^{g(x')}(B_{T_n(x)})}\right) = \frac{1}{2T_n(x)}\left( - ||B_{T_n(x)}||_2^2 + ||B_{T_n(x)} - g(x')||_2^2\right) \\
&= -\frac{1}{T_n(x)}\langle B_{T_n(x)}, g(x') \rangle + \frac{1}{2T_n(x)}||g(x')||_2^2 \\
&= -\frac{||g(x')||_2}{T_n(x)}\left\langle B_{T_n(x)}, \frac{g(x')}{||g(x')||_2}\right\rangle + \frac{1}{2T_n(x)}||g(x')||_2^2 \\
&= -\frac{||g(x')||_2}{T_n(x)}\left\langle B_{T_n(x)}, \frac{g(x')}{||g(x')||_2}\right\rangle + \frac{1}{2T_n(x)}||g(x')||_2^2 \\
&= -\frac{||g(x')||_2}{T_n(x)}W_{T_n(x)} + \frac{1}{2T_n(x)}||g(x')||_2^2.
\end{align*}
Note that the last inequality follows from the fact that if $(B_t)_{t \geq 0}$ is a d-dimensional Brownian motion and $z \in \R^d$ is a unit vector under the $\ell_2$ norm, then the process $W_t := \langle z, B_t \rangle$ is a standard Brownian motion. Noting that $g(x') = f(x') - f(x)$ and that $(-W_t)_{t \geq 0}$ is also a Brownian motion furnishes the result.
\end{proof}

We now use the characterization of privacy loss in Theorem~\ref{thm:bm_ploss} alongside the time-uniform concentration results for continuous time martingales found in Appendix~\ref{app:martingale} to construct two general families of privacy boundaries. We now prove Theorem~\ref{thm:priv_bound}.

\begin{proof}[\textbf{Proof of Theorem~\ref{thm:priv_bound}}]

Recall from Theorem~\ref{thm:bm_ploss} that we have the following bound
\[
\calL_n^{\BM}(x, x') \leq \frac{\Delta^2}{2T_n(x)} + \frac{\Delta}{T_n(x)}W_{T_n(x)}^+,
\]
where $A^+ :=\max(A, 0)$. First, by leveraging Lemma~\ref{lem:mixture}, we see that, with probability at least $1 - \delta$, for all $n \in \N$, we have
\[
\calL_n^{\BM}(x, x') \leq \frac{\Delta^2}{2T_n(x)} + \frac{\Delta}{T_n(x)}\sqrt{2(T_n(x) + \rho)\log\left(\frac{1}{\delta}\sqrt{\frac{T_n(x) + \rho}{\rho}}\right)} = \psi_\rho^M(T_n(x)),
\]
proving that $\psi_\rho^M$ is a valid $\delta$-privacy boundary. Likewise, by Lemma~\ref{lem:line_cross}, we have that
\[
\calL_n^{\BM}(x, x') \leq \frac{\Delta^2}{2T_n(x)} + \frac{\Delta}{T_n(x)}(a T_n(x) + b) = \frac{\Delta}{T_n(x)}\left(\frac{\Delta}{2} + b\right) + \Delta a = \psi^L_{a, b}(T_n(x)),
\]
showing $\psi_{a, b}^L$ is a valid $\delta$-privacy boundary.

\end{proof}

==> bm.tex <==
\section{The Brownian Mechanism: a Gaussian Noise Reduction Mechanism}
\label{sec:bm}

% In this section, we introduce the Brownian mechanism, an approach for gradually releasing a private parameter with Gaussian noise. 
The Brownian mechanism works by simulating a Brownian motion starting at some multivariate parameter; this parameter should be thought of as the risk-minimizing output if there were no privacy constraints. The data analyst first observes the random walk at some large time.
%corresponding to a large amount of noise added to the initial parameter. 
Then, if so desired, the analyst ``rewinds'' time to an earlier point on the Brownian path, reducing noise to obtain a more accurate estimate. Due to the Markovian nature of Brownian motion, the analyst will only pay a privacy cost proportional to variance of the random walk at the earliest inspected time. In what follows, when we refer to a sequence $(T_n)_{n \geq 1}$ of \textit{time functions}, we mean a sequence of functions $T_n : (\R^d)^{n - 1} \rightarrow \R_{\geq 0}$ such that, for all $n$ and $\beta_{1:n} \in (\R^d)^{n}$,
\begin{equation}\label{eq:time-functions}
T_{n + 1}(\beta_{1:n}) \leq  T_n(\beta_{1:n-1}).
\end{equation}

\begin{definition}
\label{def:bm}
Let $f : \calX \rightarrow \R^d$ be a function and $(T_n)_{n \geq 1}$ a sequence of time functions. Let $(B_t)_{t \geq 0}$ be a standard $d$-dimensional Brownian motion. 
%For $x \in \calX$, let $(f(x) + B_t)_{t \geq 0}$ be a $d$-dimensional Brownian motion started at $f(x)$ and let $(T_n(x))_{n \geq 1}$ be a decreasing sequence of (random) times such that $T_n(x)$ only depends on $x \in \calX$ through $f(x) + B_{T_1}, \dots, f(x) + B_{T_{n - 1}}$, i.e. $T_n(x)$ is $\sigma\left( f(x) + B_{T_m} : m < n\right)$-measurable. We define the the Brownian mechanism associated with $f$ and $(T_n)_{n \geq 1}$ as 
The Brownian mechanism associated with $f$ and $(T_n)_{n \geq 1}$ is the algorithm $\BM : \calX \rightarrow (\R^d)^\infty$ given by
\[
\BM(x) := \left(f(x) + B_{T_n(x)}\right)_{n \geq 1},
\]
where we set $T_n(x) := T_n\left(f(x) + B_{T_1(x)}, \dots, f(x) + B_{T_{n - 1}(x)}\right)$ with $T_1(x)$ being constant.

\end{definition}

We have chosen $T_n(x)$ as indexing notation to denote dependence on $x$, even if this is only through observed parameters. In the context of ERM, one can think of $f$ as computing a risk minimizing parameter associated with a private dataset $x \in \calX$. The data analyst uses $T_n$ along with the first $n - 1$ iterates to determine how far to rewind time to obtain the $n$th iterate. %This added adaptivity is not provided by $\LNR$ as presented by \citet{koufogiannis2015gradual}, as $\LNR$ requires fixing the sequence of privacy parameters, $(\epsilon_n)_{n \in [K]}$ in advance. As mentioned in Section~\ref{sec:back}, we extend $\LNR$ to be adaptive in Appendix~\ref{app:nr}. 
Due to the Markovian nature of Brownian motion, we get the following lemma. We include a proof in Appendix~\ref{app:bm} for completeness.

\begin{lemma}
\label{lem:bm_nr}
Let $x \sim x'$ be neighbors. For any $n \geq 1$, let $\calL^{\BM}_{1:n}(x, x')$ denote the privacy loss between $\BM_{1:n}(x)$ and $\BM_{1:n}(x')$ and $\calL^{\BM}_{n}(x, x')$ the privacy loss between $\BM_n(x)$ and $\BM_n(x')$. Then, 
\[
\calL^{\BM}_{1:n}(x, x') = \calL^{\BM}_n(x, x').
\]

\end{lemma}

Lemma~\ref{lem:bm_nr} just tells us that the Brownian mechanism is a noise reduction mechanism, i.e.\ that the privacy lost by viewing the first $n$ iterates is exactly the privacy lost by viewing the $n$th iterate in isolation. 
Thus, we can identify $\calL_{1:n}^{\BM}(x, x')$ with $\calL_n^{\BM}(x, x')$ going forward.


The Brownian mechanism, as defined above, produces an infinite sequence of parameters. In practice, a data analyst will only view finitely many iterates, stopping when some utility condition has been met or a minimum privacy level is reached. We introduce \textit{stopping functions} to model how a data analyst adaptively interacts with noise reduction mechanisms.

\begin{definition}[\textbf{Stopping Function}]
\label{def:stop}
Let $M : \calX \rightarrow \calY^\infty$ be a noise reduction mechanism. For $x \in \calX$, let $(\calF_n(x))_{n \in \N}$ be the filtration given by $\calF_n(x) := \sigma(M_i(x) :i \leq n)$.\footnote{The notation $\sigma(X)$ denotes the $\sigma$-algebra generated by $X$. $N$ is said to be a stopping time with respect to $(X_n)$ if $\{N \leq n\} \in \sigma(X_m :m \leq n)$ for all $n \in \N$. This definition can be extended to allow for $N$ to depend on independent, external randomization, but we omit this for simplicity.} A function $N : \calY^\infty \rightarrow \N$ is called a stopping function if for any $x \in \calX$, $N(x) := N(M(x))$ is a stopping time with respect to $(\calF_n(x))_{n \geq 1}$.
%ADD BACK TO FOOTNOTE This definition can be extended to allow for $N$ to depend on independent, external randomization, but we omit this for simplicity.
\end{definition}
A stopping function $N$ is a rule used to decide when to stop viewing parameters that \textit{only} depends on the observed iterates of the noise reduction mechanism. $N$ could heuristically be ``stop at the first time a parameter achieves an accuracy of 95\% on a held-out dataset.'' If a data analyst uses a stopping function alongside $\BM$, per Definition~\ref{def:nr}, the privacy loss accrued upon stopping is $\calL^{\BM}_{N(x)}(x, x')$.
Recall from Figure~\ref{fig:BM-cartoon} and equation~\eqref{eq:time-functions} that the later iterations of BM correspond to smaller noise variances, meaning that $T_n$ is a decreasing sequence in the number of iterations $n$. Further, the filtration $\calF$ defined above is quite different from the usual filtrations considered for Brownian motions. 
In some cases, an analyst may want the stopping function to depend on the underlying private dataset through more than just the released parameters, e.g. they may want their rule to be ``stop at the first time a parameter achieves an accuracy of 95\% on the private dataset.'' In this case, additional privacy may be lost due to observing $N(x)$. We detail how to handle this more subtle case in Section~\ref{sec:rat}.
%RE ADD INDENT

The following theorem characterizes the privacy loss of the Brownian mechanism.
\begin{theorem}
\label{thm:bm_ploss}
Let $\BM$ be the Brownian mechanism associated with $(T_n)_{n \geq 1}$ and a function $f$. For neighbors $x \sim x'$,  the privacy loss between $\BM_{1:n}(x)$ and $\BM_{1:n}(x')$ is given by
\[
\calL_{1:n}^{\BM}(x, x') = \calL_{n}^{\BM}(x, x') = \frac{||f(x) - f(x')||_2^2}{2T_n(x)} + \frac{||f(x) - f(x')||_2}{T_n(x)} W_{T_n(x)},
\]
where $(W_t)_{t \geq 0}$ is a standard, univariate Brownian motion. Suppose $f$ has $\ell_2$-sensitivity at most $\Delta_2$. Then, letting $a^+ := \max(0, a)$, we have
\[
\calL_n^{\BM}(x, x')  \leq \frac{\Delta_2^2}{2T_n(x)} + \frac{\Delta_2}{T_n(x)}W_{T_n(x)}^+.
\]

\end{theorem}

Theorem~\ref{thm:bm_ploss} also holds when a deterministic time $n$ is replaced by  $N(x)$, where $N$ is a stopping function. 
The above theorem can be viewed as a process-level equivalent of the well-known fact that the privacy loss of the Gaussian mechanism has an uncentered Gaussian distribution~\citep{balle2018improving}. We prove the Theorem~\ref{thm:bm_ploss} in Appendix~\ref{app:bm}. Given the clean characterization of privacy loss above, we now show how to construct high-probability, time-uniform privacy loss bounds. We define \textit{privacy boundaries}, which map the variance of $\BM$ to high-probability bounds on privacy loss.

\begin{definition}
\label{def:priv_bound}
A function $\psi : \R_{\geq 0} \rightarrow \R_{\geq 0}$ is a \textit{$\delta$-privacy boundary} for the Brownian mechanism associated with time functions $(T_n)_{n \geq 1}$ if for any neighboring datasets $x \sim x'$, we have
\[
\P\left(\exists n \geq 1 : \calL_n^{\BM}(x, x') > \psi(T_n(x))\right) \leq \delta.
\]
\end{definition}

 Since the privacy loss of $\BM$ is a deterministic function of a Brownian motion, we can apply results from martingale theory to construct general families of privacy boundaries.

\begin{theorem}
\label{thm:priv_bound}
Assume the same setup as in Theorem~\ref{thm:bm_ploss}. Let $\delta > 0$ and $f$ be a function with $\ell_2$-sensitivity $\Delta_2$. The following classes of functions form $\delta$-privacy boundaries.
\begin{enumerate}
\item{\textbf{(Mixture boundary)}} For any $\rho > 0$, $\psi^{M}_\rho$ given by
\[
\psi^{M}_\rho(t) := \frac{\Delta^2_2}{2t} + \frac{\Delta_2}{t}\sqrt{2(t + \rho)\log\left(\frac{1}{\delta}\sqrt{\frac{t + \rho}{\rho}}\right)}.
\]
\item{\textbf{(Linear boundary)}} For any $a, b > 0$ such that $2ab = \log(1/\delta)$, $\psi^{L}_{a, b}$ given by
\[
\psi^{L}_{a, b}(t) := \frac{\Delta_2}{t}\left(\frac{\Delta_2}{2} + b\right) + \Delta_2 a.
\]
\end{enumerate}

\end{theorem}

We prove Theorem~\ref{thm:priv_bound} in Appendix~\ref{app:bm}. In the same appendix, we plot the boundaries in Figure~\ref{fig:bound}. 
%It is clear that no boundary uniformly dominates another, indicating a fundamental tradeoff between optimizing the tightness at a fixed time and providing an overall tight bound on privacy loss.
\begin{comment}
\begin{figure}
\centering
    \subfloat[Variance of Noise vs. Privacy Loss]{
        \includegraphics[width=0.4\textwidth]{figs/var_vs_ploss.png}
        \label{fig:bound:var_pl}
    }
    \subfloat[Privacy Loss vs. Variance of Noise]{
        \includegraphics[width=0.4\textwidth]{figs/ploss_vs_var.png}
        \label{fig:bound:pl_var}
    }
    
    \caption{
    A comparison of the linear and mixture boundaries, both optimized for tightness at $\epsilon = 0.5$. The first plot directly plots the corresponding bounds as in Theorem~\ref{thm:priv_bound}. The second plot inverts the boundaries, showing the variance necessary to meet a target privacy level. 
    %In both plots, the linear bound demonstrates improved tightness at the privacy level optimized for. On the other hand, the mixture boundary demonstrates greater \textit{overall} tightness.
    }
    \label{fig:bound}
\end{figure}
\end{comment}

Privacy boundaries serve a dual purpose for the Brownian mechanism. First, since time-uniform concentration bounds are valid at arbitrary data-dependent times, that need not be stopping times with respect to the standard forward Brownian Motion filtration \citep{howard2021unif}, privacy boundaries provide ex-post privacy guarantees.  Second, in many settings, it may be more natural for a data analyst to adaptively specify target privacy levels instead of noise levels. 
This is, for instance, the case in our experiments in Section~\ref{sec:exp}. 
By inverting privacy boundaries, data analysts can compute the proper amount of noise to remove at each step to meet target privacy levels.
%RE ADD indent here

We make the above precise in Corollary~\ref{cor:ex_post}. In what follows, when we refer to a sequence $(\Epsilon_n)_{n \geq 1}$ of \textit{privacy functions}, we mean a sequence of functions $\Epsilon_n : (\R^d)^{n - 1} \rightarrow \R_{\geq 0}$ such that, for all $n$ and $\beta_{1:n} \in (\R^d)^{n}$, $\Epsilon_{n + 1}(\beta_{1:n}) \geq \Epsilon_n(\beta_{1:n-1})$. 

\begin{corollary}
\label{cor:ex_post}
Let $N$ be a stopping function, as in Definition~\ref{def:stop}. If $\psi$ is a $\delta$-privacy boundary for $\BM$, we have
\[
\sup_{x \sim x'}\P\left(\calL^{\BM}_{N(x)}(x, x') \geq \psi\left(T_{N(x)}(x)\right)\right) \leq \delta,
\]
i.e.\ the algorithm $\BM_{1:N(\cdot)}(\cdot)$ is $\left(\psi(T_{N(\cdot)}(\cdot)), \delta\right)$-ex post private, where $(\cdot)$ denotes a positional argument for an input $x \in \calX$. 
Further, let $(\Epsilon_n)_{n \geq 1}$ be a sequence of privacy functions, and define
\[
T_n(\beta_{1:n - 1}) := \inf\left\{t \geq 0 : \psi(t) \geq \Epsilon_n(\beta_{1:n - 1})\right\}.
\]
Then $\BM_{1:N(\cdot)}(\cdot)$ is $(\Epsilon_{N(\cdot)}(\cdot), \delta)$-ex post private, where $\Epsilon_n(x)$ is defined analogously to $T_n(x)$.
\end{corollary}

Again, $N$ should be thought of as a stopping rule based on parameter accuracy. $\Epsilon_n$ should be thought of as a rule for choosing the $n$th privacy parameter given $\BM_{1:n-1}(x)$. 
%\jwedit{The second part of Corollary~\ref{cor:ex_post} thus specifies how a data analyst can adaptively select target privacy levels when using the Brownian mechanism.}
%We restrict Corollary~\ref{cor:ex_post} to stopping functions because, as mentioned above, if  $N(x)$ depends on $x \in \calX$ through more than the observed iterates and external randomization, the time at which the analyst stops can leak information about the data. We show how to bound this leakage in Section~\ref{sec:rat}.




\begin{comment}
As a final point, we note that in many settings, such as those in Section~\ref{sec:exp}, it is desirable for a data analyst to be able to specify a sequence of functions determining privacy levels $(\epsilon_n)_{n \geq 1}$ instead of a sequence of functions $(T_n)_{n \geq 1}$ determining times. The data analyst can readily use a $\delta$-privacy boundary $\psi$ accompanying $\BM$ to map target privacy levels to times. In detail, the analyst can just define the (random) times $T_n(x) := \inf\left\{t \geq 0 : \psi(t) \geq \epsilon_n(x)\right\}$. It is straightforward to see that, in this setting, $\sup_{x \sim x'}\P(\exists n \geq 1 : \calL_{n}^{\BM}(x, x') \geq \epsilon_n(x)) \leq \delta$. In particular, this yields that for any stopping function $N$, the algorithm $\BM_{1:N(\cdot)}(\cdot)$ is $(\epsilon_{N(\cdot)}, \delta)$-ex post private.
\end{comment}

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} {\bf We construct the Brownian mechanism is Section~\ref{sec:bm}, show how to query utility on private datasets in a manner that provides adaptive privacy guarantees in Section~\ref{sec:rat}, and conduct experiments showing the Brownian mechanism outperforms Laplace noise reduction in Section~\ref{sec:exp}}.
  \item Did you describe the limitations of your work?
    \answerYes{} {\bf In the Conclusion (Section~\ref{sec:conc}) we discuss how traditional composition results for differential privacy do not directly apply to mechanisms with ex-post privacy guarantees. We leave it as future work to address composition in this setting. Additionally, in the same section, we mention noise reduction is only applicable to output perturbation methods. We leave it as future work to generalize to other modes of private computation, such as objective perturbation.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{} {\bf There are no negative societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} {\bf All theoretical results have a full set of assumptions stated.}
        \item Did you include complete proofs of all theoretical results? 
    \answerYes{} {\bf The proofs of all non-trivial results are fully contained in the appendices. Appendix~\ref{app:bm} contains the proofs for Section~\ref{sec:bm}, Appendix~\ref{app:rat} contains the proofs for Section~\ref{sec:rat}, and Appendix~\ref{app:nr} contains proofs for Section~\ref{sec:lnr}.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} {\bf The code is commented and contained in the supplement.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} {\bf These details are included in the paper and code.}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} {\bf We included 95\% confidence intervals on the relevant experiments. See the graphs in Section~\ref{sec:exp}}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{} {\bf Experiments were lightweight and run on a laptop.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} {\bf The datasets are properly attributed in the Bibliography.}
  \item Did you mention the license of the assets?
    \answerNA{} {\bf The datasets leveraged in this work are public, and hence do not require licensing.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{} {\bf we only use well-known, broadly used, publicly available datasets, without offensive content or personal information.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the text of instructions given to participants and screenshots?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> lnr.tex <==
\section{An Adaptive, Continuous-Time Extension of Laplace Noise Reduction}
\label{sec:lnr}

Here, we generalize the original noise reduction mechanism of \citet{ligett2017accuracy}, which will be used as a subroutine in Algorithm~\ref{alg:rat} in the following section. We first describe the original Laplace-based Markov process of \citet{koufogiannis2015gradual}. Fix any positive integer $K$ and any finite, increasing sequence of times $(t_n)_{n \in [K]}$. Let $(\zeta_n)_{n = 0}^K$ be the $d$-dimensional process given by $\zeta_0 = 0$ and
\begin{equation}
\label{eq:orig_lap_proc}
\zeta_n = \begin{cases}
\zeta_{n - 1} &\text{ with probability } \left(\frac{t_{n - 1}}{t_n}\right)^2 \\
\zeta_{n - 1} + \Lap(t_n) &\text{ otherwise.}
\end{cases}
\end{equation}

\citet{koufogiannis2015gradual} show that $\zeta_n \sim \Lap(t_n)$ and that $(\zeta_n)_{n = 0}^K$ is Markovian. \citet{ligett2017accuracy} use the above process to construct a noise reduction mechanism. Namely, they define the the \textit{Laplace Noise Reduction} mechanism associated with $f : \calX \rightarrow \R^d$ and $(t_n)_{n \in [K]}$ to be the algorithm $\LNR : \calX \rightarrow (\R^d)^K$ given by $\LNR(x) := (f(x) + \zeta_{K}, \dots, f(x) + \zeta_1)$. If $t_n := \Delta_1/\epsilon_n$, then releasing $n$th component $\LNR_n(x)$ in isolation is equivalent to running the classical Laplace mechanism with privacy level $\epsilon_n$. 

We now extend the process $(\zeta_n)_{n \in [K]}$ to a continuous time process with the same finite-dimensional distributions. Let $\eta > 0$ be arbitrary, and let $(P_t)_{t \geq \eta}$ be an inhomogeneous Poisson process with intensity function $\lambda(t) := \frac{2}{t}$. For $n \geq 1$, let $\calT_n := \inf\{t \geq \eta : P_t \geq  n\}$ be the $n$th jump of $(P_t)_{t \geq \eta}$ and set $\calT_0 := \eta$. Noting that $P_t$ must be a nonnegative integer, define the process $(Z_t)_{t \geq \eta}$ by
\begin{equation}
\label{eq:lap_proc}
Z_t :=  \sum_{n = 0}^{P_t}\Lap(\calT_n).
\end{equation}
It is immediate that $(Z_t)_{t \geq \eta}$ is Markovian. We show in Appendix~\ref{app:nr} that $Z_t \sim \Lap(t)$. With $(Z_t)_{t \geq \eta}$, one can make $\LNR$ fully adaptive, meaning that the times $(t_n)_{n \in [K]}$ at which it is invoked need not be prespecified, and can depend on the underlying input database $x$ by using time functions. 
%\jwedit{As aforementioned, this adaptivity is needed for our construction of Algorithm~\ref{alg:rat}.}
\begin{definition}
\label{def:lnr}
Let $f : \calX \rightarrow \R^d$ be a function and $(T_n)_{n \geq 1}$ a sequence of time functions. Let $(Z_t)_{t \geq \eta}$ be the process defined in Equation~\eqref{eq:lap_proc}. The \textit{Laplace noise reduction} mechanism associated with $f$ and $(T_n)_{n \geq 1}$ is the algorithm $\LNR : \calX \rightarrow (\R_{>0} \times \R^d)^\infty$ given by
\[
\LNR(x) := \left( T_n(x), f(x) + Z_{T_n(x)}\right)_{n \geq 1},
\]
where again $T_n(x) := T_n(f(x) + Z_{T_1(x)}, \dots, f(x) + Z_{T_{n - 1}(x)})$.
\end{definition}

If the analyst would prefer instead to specify privacy functions $(\Epsilon_n)_{n \geq 1}$, they can do so by leveraging the corresponding time functions $T_n(x) := \Delta_1/\Epsilon_n(x)$, where $\Epsilon_n(x)$ is defined analogously to $T_n(x)$. We leverage $\LNR$ in our experiments in Section~\ref{sec:exp} and the process $(Z_t)_{t \geq 0}$ as a subroutine in constructing $\RAT$. $\LNR$ admits the following trivial ex-post privacy guarantee.

\begin{prop}
\label{prop:lnr}
Let $\LNR$ be associated with $(T_n)_{n \geq 1}$ and a function $f$ with $\ell_1$-sensitivity $\Delta_1$. If $N$ is stopping function, the algorithm $\LNR_{1:N(\cdot)}(\cdot)$ is $(\Delta_1/T_{N(\cdot)}(\cdot), 0)$-ex post private.
\end{prop}


% \section{Skellam Noise Reduction}\label{sec:Skellam}

\paragraph{Skellam Noise Reduction.} Last, we briefly discuss how to generate a noise reduction mechanism for Skellam noise~\citep{agarwal2021skellam}. Recall that a random variable $X$ has a Skellam distribution with parameters $\lambda_1$ and $\lambda_2$ if $X =_d Y_1 - Y_2$, where $Y_1 \sim \mathrm{Poisson}(\lambda_1)$ and $Y_2 \sim \mathrm{Poisson}(\lambda_2)$ are independent Laplace random variables. For succinctness, we write $X \sim \textrm{Skell}(\lambda_1, \lambda_2)$.

Let $(P_1(t))_{t \geq 0}$ and $(P_2(t))_{t \geq 0}$ be two independent, homogeneous Poisson process with rates $\lambda_1$ and $\lambda_2$ respectively. Observe that the continuous time process $(X_t)_{t \geq 0}$ given by $X_t := P_1(t) - P_2(t)$ is clearly Markovian, has independent increments, and has $X_t \sim \mathrm{Skell}(t\lambda_1, t\lambda_2)$. Thus, $(X_t)_{t \geq 0}$ can be used to define a Skellam noise reduction mechanism by releasing $(T_n(x), f(x) + X_{T_n(x)})_{n \geq 1}$ for some sequence of time functions $(T_n)_{n \geq 1}$.


==> tex_graveyard.tex <==

\rrcomment{Please review the following:}
We now consider more general time functions $T_n(x)$ yet keeping $n$ to be fixed.  We will denote $z_{-i} \in \R^{d-1}$ to denote a vector $z \in \R^d$ with coordinate $i$ removed and $z = (z_{-i}, z_i)$.  Without loss of generality, we assume that $T_n(t, (z_{-d}, z_d))$ is strictly increasing in $z_d$ for every $n>1$, and $t \in (0, b), z_{-d} \in \R^{d-1}$, where $T_1 = b$ is constant.  For $n>2$ we have that $\BM_{1:n}(x)$ produces a vector of length $n\cdot (d+1)$.  Under the assumption that $T_n(t, (z_{-d}, z_d) )$ is strictly increasing in its last coordinate, the distribution of $\BM_{1:n}(x)$ can instead be understood with the following mechanism $\tilde{M}_{1:n}(x)$, which produces a vector of length $dn +1$,
\[
\tilde{M}_{1:n}(x) = \left( \left(T_{n}(x), f(x) + B_{T_n(x)} \right), \left( T_{n-1}(x), (f(x) + B_{T_{n-1}(x)})_{-d} \right), \cdots, \left(T_1(x), (f(x) + B_{T_{1}(x)})_{-d} \right) \right).
\]
Note that for all $i \in [n-1]$, we have that $f(x) + B_{T_i(x)}$ is a measurable function of 
\[
\left( (T_{i}(x),  (f(x) + B_{T_{i}(x)})_{-d}), 
 (T_{i+1}(x),  (f(x) + B_{T_{i+1}(x)})_{-d})\right),
 \] so that $\BM_{1:n}(x)$ is a measurable function of $\tilde{M}_{1:n}(x)$.  We then consider the density of $\tilde{M}_{1:n}(x)$ with respect to the Lebesgue measure on the space 
\[
S_{1:n} = (0, b) \times \R^d \times \{(0,b) \times \R^{d-1} \}^{n-1}
\]
and we compare the privacy loss of $\BM_{1:n}(x)$ with the privacy loss of $\BM_{n}(x) = (T_n(x), f(x) + B_{T_n(x)})$.  The density of $\BM_n(x)$ is computed with respect to the Lebesgue measure on $(0,b) \times \R^d$.

We will write $\tilde{z}_i = (z_i)_{-d}$ for $i \in [n-1]$. We start by computing the density $p_{1:n}^x(t_n, z_{n}, t_{n-1}, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_{2}, \tilde{z}_1)$ of $\tilde{M}_{1:n}(x) $ on the space $S_{1:n}$, so that $0<t_n< \cdots < t_2 < b$ and $z_n \in \R^d$ and $\tilde{z}_i \in \R^{d-1}$ for $i \in [n-1]$.  We will write $a \leq b$ for $a, b \in \R^d$ to mean coordinate-wise inequality $a_i \leq b_i$ for $i \in [d]$.  We then have,
\begin{align*}
& F^x_{1:n}(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1) \\
& \qquad = \Pr\left[ T_i(x) \leq t_i, i \in \{2, \cdots, n \}, f(x) + B_{T_n(x)} \leq z_n, \ (f(x) + B_{T_i(x)})_{-d} \leq \tilde{z}_i \text{ for } i \in [n-1] \right] \\
& \implies p_{1:n}^x(t_n, z_n, \cdots, t_2, z_2, z_1)  = \frac{\partial^{dn}}{\partial t_n \partial z_n \partial t_{n-1} \partial \tilde{z}_{n-1} \cdots \partial t_{2} \partial \tilde{z}_2 \partial \tilde{z}_1 } F_{1:n}^x(t_n, z_n, t_{n-1}, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1). 
\end{align*}
Note that for $y \in \R^k$ we use $\partial^k / \partial y$ to denote the gradient with respect $y$.  To make dependencies more explicit and to simplify notation, we will write $\tilde{T}_2(z_1) = T_2(b, z_1)$ and for $n>2$, we have
\[
\tilde{T}_{n}(z_1, \cdots, z_{n-1}) = T_n( \tilde{T}_{n-1}(z_1, \cdots, z_{n-2}), z_{n-1}).
\]
By assumption $T_n(t, z )$ is strictly increasing in $z_d$, we know that $\tilde{T}_{n}(z_1, \cdots, z_{n-1})$ is strictly increasing in $z_{n-1,d}$ for all fixed $z_1, \cdots,z_{n-2}, (z_{n-1})_{-d}$ with $n \geq 2$.  We denote $\tilde{T}^{-1}_n(z_1, \cdots, z_{n-2}, \tilde{z}_{n-1}, t_n) \in \R$ as the inverse of this function of $z_{n-1,d}$ for fixed $z_1, \cdots, z_{n-2}, \tilde{z}_{n-1}$.  Hence 
\begin{align*}
    & F^x_{1:n}(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1)  = \frac{1}{\sqrt[d]{2\pi b}} \int_{\tilde{w}_1 \leq \tilde{z}_1} \int_{-\infty}^{\tilde T_{2}^{-1}(\tilde{w}_1, t_2)} \exp\left(- \frac{|| w_1 -f(x)||_2^2}{2b} \right)\\
    &\cdot  \frac{1}{\sqrt[d]{2\pi \tilde{T}_2(w_1) (b - \tilde{T}_2(w_1))/b}} \int_{\tilde{w}_2 \leq \tilde{z}_2}\\
    & \qquad \qquad \cdot \int_{-\infty}^{\tilde T_{3}^{-1}(w_1, \tilde{w}_2, t_2 )} \exp\left(- \frac{||w_2 -f(x) - \tilde T_{2}(w_1) (w_1 - f(x)) / b ||_2^2}{2\tilde T_{2}(w_1) (b-\tilde T_{2}(w_1))/b } \right)  \\
    & \vdots \\
    & \cdot \frac{1}{\sqrt[d]{2\pi \tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \left(\tilde{T}_{n-2}(w_1, \cdots, w_{n-3}) 
 - \tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \right) / \tilde{T}_{n-2} (w_1, \cdots, w_{n-3}) }} \\
    & \cdot \int_{\tilde{w}_{n-1} \leq \tilde{z}_{n-1}} \int_{-\infty}^{\tilde T_{n}^{-1}(w_1, \cdots, w_{n-2}, \tilde{w}_{n-1}, t_n )} \exp\left(- \frac{|| w_{n-1} - f(x) - \left( \frac{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})}{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3})} \right) (w_{n-2} - f(x))||_2^2}{2\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \left( \frac{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3}) - \tilde{T}_{n-1}(w_1, \cdots, w_{n-2})}{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3})} \right)} \right) \\
    & \cdot \frac{1}{\sqrt[d]{2\pi \tilde{T}_{n}(w_1, \cdots, w_{n-1}) \left(\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) 
 - \tilde{T}_{n}(w_1, \cdots, w_{n-1}) \right) / \tilde{T}_{n-1} (w_1, \cdots, w_{n-2}) }} \\
    & \cdot \int_{w_n \leq z_n} \exp\left( -\frac{ || w_n - f(x) - \left( \frac{\tilde{T}_{n}(w_1, \cdots, w_{n-1})}{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})} \right) (w_{n-1} - f(x)) ||_2^2}{2\tilde{T}_{n}(w_1, \cdots, w_{n-1}) \left( \frac{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) - \tilde{T}_{n}(w_1, \cdots, w_{n-1})}{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})} \right)} \right)dw_n dw_{n-1} \cdots dw_{1}
\end{align*}
We then take gradient with respect to $z_n$ to get the most inner integral simplifying to the following
\[
 \exp\left( -\frac{ || z_n - f(x) - \left( \frac{\tilde{T}_{n}(w_1, \cdots, w_{n-1})}{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})} \right) (w_{n-1} - f(x)) ||_2^2}{2\tilde{T}_{n}(w_1, \cdots, w_{n-1}) \left( \frac{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) - \tilde{T}_{n}(w_1, \cdots, w_{n-1})}{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})} \right)} \right).
\]
Next, we differentiate with respect to $t_n$ to get, 
\begin{align*}
& \frac{\partial^{d+1}}{\partial t_n \partial z_n} F^x_{1:n}(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1) = \frac{1}{\sqrt[d]{2\pi b}} \int_{\tilde{w}_1 \leq \tilde{z}_1} \int_{-\infty}^{\tilde T_{2}^{-1}(\tilde{w}_1, t_2)} \exp\left(- \frac{|| w_1 -f(x)||_2^2}{2b} \right)\\
    &\cdot  \frac{1}{\sqrt[d]{2\pi \tilde{T}_2(w_1) (b - \tilde{T}_2(w_1))/b}} \int_{\tilde{w}_2 \leq \tilde{z}_2}\\
    & \qquad \qquad \cdot \int_{-\infty}^{\tilde T_{3}^{-1}(w_1, \tilde{w}_2, t_2 )} \exp\left(- \frac{||w_2 -f(x) - \tilde T_{2}(w_1) (w_1 - f(x)) / b ||_2^2}{2\tilde T_{2}(w_1) (b-\tilde T_{2}(w_1))/b } \right)  \\
    & \vdots \\
    & \cdot \frac{1}{\sqrt[d]{2\pi \tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \left(\tilde{T}_{n-2}(w_1, \cdots, w_{n-3}) 
 - \tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \right) / \tilde{T}_{n-2} (w_1, \cdots, w_{n-3}) }} \\
    & \cdot \int_{\tilde{w}_{n-1} \leq \tilde{z}_{n-1}} \exp\left(- \frac{|| (\tilde{w}_{n-1}, \tilde T_{n}^{-1}(w_1, \cdots, w_{n-2}, \tilde{w}_{n-1}, t_n )) - f(x) - \left( \frac{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})}{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3})} \right) (w_{n-2} - f(x))||_2^2}{2\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \left( \frac{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3}) - \tilde{T}_{n-1}(w_1, \cdots, w_{n-2})}{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3})} \right)} \right)  \\
    & \qquad \cdot  \frac{\partial}{\partial t_n} \tilde T_{n}^{-1}(w_1, \cdots, w_{n-2}, \tilde{w}_{n-1}, t_n )  \\
    & \cdot \frac{1}{\sqrt[d]{2\pi \tilde{T}_{n}(w_1, \cdots, w_{n-1}) \left(\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) 
 - \tilde{T}_{n}(w_1, \cdots, w_{n-1}) \right) / \tilde{T}_{n-1} (w_1, \cdots, w_{n-2}) }} \\
    & \cdot \exp\left( -\frac{ || z_n - f(x) - \left( \frac{\tilde{T}_{n}(w_1, \cdots, w_{n-1})}{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})} \right) (w_{n-1} - f(x)) ||_2^2}{2\tilde{T}_{n}(w_1, \cdots, w_{n-1}) \left( \frac{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) - \tilde{T}_{n}(w_1, \cdots, w_{n-1})}{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})} \right)} \right)d\tilde{w}_{n-1} \cdots dw_{1} 
\end{align*}
Taking the gradient with respect to $\tilde{z}_{n-1}$ then gives us
\begin{align*}
& \frac{\partial^{2d}}{\partial \tilde{z}_{n-1}\partial t_n \partial z_n} F^x_{1:n}(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1) = \frac{1}{\sqrt[d]{2\pi b}} \int_{\tilde{w}_1 \leq \tilde{z}_1} \int_{-\infty}^{\tilde T_{2}^{-1}(\tilde{w}_1, t_2)} \exp\left(- \frac{|| w_1 -f(x)||_2^2}{2b} \right)\\
    &\cdot  \frac{1}{\sqrt[d]{2\pi \tilde{T}_2(w_1) (b - \tilde{T}_2(w_1))/b}} \int_{\tilde{w}_2 \leq \tilde{z}_2}\\
    & \qquad \qquad \cdot \int_{-\infty}^{\tilde T_{3}^{-1}(w_1, \tilde{w}_2, t_2 )} \exp\left(- \frac{||w_2 -f(x) - \tilde T_{2}(w_1) (w_1 - f(x)) / b ||_2^2}{2\tilde T_{2}(w_1) (b-\tilde T_{2}(w_1))/b } \right)  \\
    & \vdots \\
    & \cdot \frac{1}{\sqrt[d]{2\pi \tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \left(\tilde{T}_{n-2}(w_1, \cdots, w_{n-3}) 
 - \tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \right) / \tilde{T}_{n-2} (w_1, \cdots, w_{n-3}) }} \\
    & \cdot  \exp\left(- \frac{|| (\tilde{z}_{n-1}, \tilde T_{n}^{-1}(w_1, \cdots, w_{n-2}, \tilde{z}_{n-1}, t_n )) - f(x) - \left( \frac{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})}{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3})} \right) (w_{n-2} - f(x))||_2^2}{2\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \left( \frac{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3}) - \tilde{T}_{n-1}(w_1, \cdots, w_{n-2})}{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3})} \right)} \right) \\
    & \cdot \frac{1}{\sqrt[d]{2\pi t_n \left(\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) 
 - t_n \right) / \tilde{T}_{n-1} (w_1, \cdots, w_{n-2}) }} \cdot \frac{\partial}{\partial t_n} \tilde T_{n}^{-1}(w_1, \cdots, w_{n-2}, \tilde{z}_{n-1}, t_n ) \\
    & \cdot \exp\left( -\frac{ || z_n - f(x) - \left( \frac{t_n}{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})} \right) ( (\tilde{z}_{n-1}, \tilde{T}_n^{-1}(w_1, \cdots, w_{n-2}, \tilde{z}_{n-1}, t_n) ) - f(x)) ||_2^2}{2t_n \left( \frac{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) -t_n}{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})} \right)} \right) d{w}_{n-2} \cdots dw_{1}
\end{align*}
We then continue in the same manner and write $T^{-1}_i(t_{i-1}, \tilde{z}_{i-1}, t_i)$ to be the inverse of $T_i(t_{i-1}, \tilde{z}_{i-1}, z_{i-1}[d])$ in the last coordinate to get
\begin{align*}
    & p^x_{1:n}(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1)  = \frac{1}{\sqrt[d]{2\pi b}}  \exp\left(- \frac{|| (\tilde{z}_1, T_{2}^{-1}(\tilde{z}_1, t_2)) -f(x)||_2^2}{2b} \right) \frac{\partial}{\partial t_2} T_{2}^{-1}(\tilde{z}_{1}, t_2 ) \\
    &\cdot  \frac{1}{\sqrt[d]{2\pi t_2 (b - t_2)/b}}\cdot \exp\left(- \frac{|| (\tilde{z}_2,  T_{3}^{-1}(t_2, \tilde{z}_2, t_3 )) -f(x) - t_2 ( (\tilde{z}_{1},  T_{2}^{-1}(\tilde{z}_{1}, t_2 )) - f(x)) / b ||_2^2}{2t_2 (b-t_2)/b } \right)  \\
    & \vdots \\
    & \cdot \frac{1}{\sqrt[d]{2\pi t_{n-1} \left(t_{n-2} 
 - t_{n-1} \right) / t_{n-2} }} \\
    & \cdot  \exp\left(- \frac{|| (\tilde{z}_{n-1}, T_{n}^{-1}(t_{n-1}, \tilde{z}_{n-1}, t_n )) - f(x) - \left( \frac{t_{n-1}}{t_{n-2}} \right) ( (\tilde{z}_{n-2}, T^{-1}_{n-1}(t_{n-2}, \tilde{z}_{n-2}, t_{n-1} )) - f(x))||_2^2}{2t_{n-1} \left( \frac{t_{n-2} - t_{n-1}}{t_{n-2}} \right)} \right) \\
    & \cdot \frac{1}{\sqrt[d]{2\pi t_n \left(t_{n-1} 
 - t_n \right) / t_{n-1} }} \cdot \frac{\partial}{\partial t_n} T_{n}^{-1}(t_{n-1}, \tilde{z}_{n-1}, t_n ) \\
    & \cdot \exp\left( -\frac{ || z_n - f(x) - \left( \frac{t_n}{t_{n-1}} \right) ( (\tilde{z}_{n-1}, T_n^{-1}(t_{n-1}, \tilde{z}_{n-1}, t_n) ) - f(x)) ||_2^2}{2t_n \left( \frac{ t_{n-1} -t_n}{t_{n-1}} \right)} \right) 
\end{align*}
We now rearrange some terms to get
\begin{align*}
    & p^x_{1:n}(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1)  \\
    & \qquad = (2\pi)^{-nd/2}  \left( t_n(t_{n-1} - t_{n}) \cdots (b - t_2)\right)^{-d/2} \cdot \prod_{i=2}^n \frac{\partial}{\partial t_i} T_{i}^{-1}(t_{i-1}, \tilde{z}_{i-1}, t_i ) \\
    & \qquad \cdot  \exp\left\{ - \frac{1}{2} \left[  \frac{|| (\tilde{z}_1, T_{2}^{-1}(\tilde{z}_1, t_2)) -f(x)||_2^2}{b}  + \frac{|| (\tilde{z}_2,  T_{3}^{-1}(t_2, \tilde{z}_2, t_3 )) -f(x) - t_2 ( (\tilde{z}_{1},  T_{2}^{-1}(\tilde{z}_{1}, t_2 )) - f(x)) / b ||_2^2}{t_2 (b-t_2)/b } \right. \right.  \\
    & \qquad \qquad  + \cdots + \\
    & \qquad \qquad  + \frac{|| (\tilde{z}_{n-1}, T_{n}^{-1}(t_{n-1}, \tilde{z}_{n-1}, t_n )) - f(x) - \left( \frac{t_{n-1}}{t_{n-2}} \right) ( (\tilde{z}_{n-2}, T^{-1}_{n-1}(t_{n-2}, \tilde{z}_{n-2}, t_{n-1} )) - f(x))||_2^2}{t_{n-1} \left( \frac{t_{n-2} - t_{n-1}}{t_{n-2}} \right)} \\
    & \qquad \qquad \left. \left. + \frac{ || z_n - f(x) - \left( \frac{t_n}{t_{n-1}} \right) ( (\tilde{z}_{n-1}, \tilde{T}_n^{-1}(t_{n-1}, \tilde{z}_{n-1}, t_n) ) - f(x)) ||_2^2}{t_n \left( \frac{ t_{n-1} -t_n}{t_{n-1}} \right)}  \right] \right\} \\
    & \qquad = (2\pi)^{-nd/2}  \left( t_n(t_{n-1} - t_{n}) \cdots (b - t_2)\right)^{-d/2} \cdot \prod_{i=2}^d \frac{\partial}{\partial t_i} T_{i}^{-1}(t_{i-1}, \tilde{z}_{i-1}, t_i ) \\
    & \qquad \cdot  \exp\left\{ - \frac{1}{2} \left[  \frac{|| z_n -f(x)||_2^2}{t_n}  + \frac{|| (\tilde{z}_{n-1},  T_{n}^{-1}(t_{n-1}, \tilde{z}_{n-1}, t_n )) - z_n ||_2^2}{t_{n-1} - t_n } \right. \right.  \\
    &  \qquad \qquad +\frac{|| (\tilde{z}_1, T_2^{-1}(\tilde{z}_1, t_2) ) - ( \tilde{z}_2, T_3^{-1} (t_2, \tilde{z}_2, t_3) ||_2^2}{b-t_2}\\
    & \qquad \qquad \left. \left.  + \sum_{j=3}^{n-1} \frac{ || (\tilde{z}_{j-1}, T_j^{-1}(t_{j-1}, \tilde{z}_{j-1}, t_j) ) - (\tilde{z}_{j}, T_{j+1}^{-1}(t_{j}, \tilde{z}_{j}, t_{j+1}) ) ||_2^2}{t_{j-1} - t_j}  \right] \right\}
\end{align*}
We then integrate over $t_{n-1}, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1$ in order to get the density $p^x(t_n, z_n; n)$
\begin{align*}
& p^x(t_n, z_n; n) = \int_{t_n < t_{n-1} < \cdots < t_2<b} \int_{(\R^{d-1})^{n-1}} p^x_{1:n}(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1) d\tilde{z}_{n-1} \cdots d \tilde{z}_{1} dt_{n-1}\cdots dt_2 \\
& = \exp\left\{ - \frac{1}{2} \left[  \frac{|| z_n -f(x)||_2^2}{t_n} \right] \right\} \\
& \qquad \cdot \int_{t_n < t_{n-1} < \cdots < t_2<b} \int_{(\R^{d-1})^{n-1}}  (2\pi)^{-nd/2}  \left( t_n(t_{n-1} - t_{n}) \cdots (b - t_2)\right)^{-d/2} \cdot \prod_{i=2}^n \frac{\partial}{\partial t_i} T_{i}^{-1}(t_{i-1}, \tilde{z}_{i-1}, t_i ) \\
    & \qquad \cdot  \exp\left\{ - \frac{1}{2} \left[ \frac{|| (\tilde{z}_{n-1},  T_{n}^{-1}(t_{n-1}, \tilde{z}_{n-1}, t_n )) - z_n ||_2^2}{t_{n-1} - t_n } +\frac{|| (\tilde{z}_1, T_2^{-1}(\tilde{z}_1, t_2) ) - ( \tilde{z}_2, T_3^{-1} (t_2, \tilde{z}_2, t_3) ||_2^2}{b-t_2} \right. \right.  \\
    & \qquad \qquad \left. \left.  + \sum_{j=3}^{n-1} \frac{ || (\tilde{z}_{j-1}, T_j^{-1}(t_{j-1}, \tilde{z}_{j-1}, t_j) ) - (\tilde{z}_{j}, T_{j+1}^{-1}(t_{j}, \tilde{z}_{j}, t_{j+1}) ) ||_2^2}{t_{j-1} - t_j}  \right] \right\}d\tilde{z}_{n-1} \cdots d \tilde{z}_{1} dt_{n-1}\cdots dt_2
\end{align*}
Putting this all together, we get the following relation for neighbors $x, x'$
\begin{align}
    \frac{p^x_{1:n}(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1)}{p^{x'}_{1:n}(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1)} & =  \exp\left\{ - \frac{1}{2} \left[  \frac{|| z_n -f(x)||_2^2}{t_n}  - \frac{|| z_n -f(x')||_2^2}{t_n} \right] \right\} \nonumber \\
    & = \frac{ p^x(t_n, z_n; n) }{ p^{x'}(t_n, z_n; n) } \label{eq:pl_relation}
\end{align}

We now consider a random stopping time $N(x) \gets n$. In this case, we consider the augmented mechanism
\[
\tilde{M}^*(x) = (N(x), \tilde{M}_{1:N(x)}(x) ) \in S^* = \cup_{n=1}^\infty \left\{ \left\{ n\right\} \times S_{1:n} \right\}
\]
We then consider the same Lebesgue measure for the dimensions in $S_{1:n}$ equip a counting meansure on $\N$, which gives a $\sigma$-finite measure on $S^*$.  All densities and privacy loss random variables will be with respect to this measure.  We will then compare the privacy loss of $M^*(x)$ with the privacy loss of the mechanism $M^*_{\text{last}}(x) = (N(x), \tilde{M}^*_{N(x)}(x))$.  The density of $M^*_{\text{last}}(x)$ is computed with respect to the product of the counting measure of $\N$ and the Lebesgue measure on $(0,b) \times \R$.  We then have
\begin{align*}
    & Q^x(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1; n) \\
    & = \Pr\left[N(x) = n,  T_i(x) \leq t_i, i \in \{2, \cdots, n \}, f(x) + B_{T_n(x)} \leq z_n, \ (f(x) + B_{T_i(x)})_{-d} \leq \tilde{z}_i \text{ for } i \in [n-1] \right]
\end{align*}
We will write the stopping time $N(z_1, z_2, \cdots, z_{i-1})$ to depend on the previous outcomes prior to round $i>1$.  We then have 
\begin{align*}
    & Q^x(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1; n) \\
    & = \frac{1}{\sqrt[d]{2\pi b}} \int_{\tilde{w}_1 \leq \tilde{z}_1} \int_{-\infty}^{\tilde T_{2}^{-1}(\tilde{w}_1, t_2)} \exp\left(- \frac{|| w_1 -f(x)||_2^2}{2b} \right) \mathbbm{1}\{N(w_1) > 1 \} \\
    &\cdot  \frac{1}{\sqrt[d]{2\pi \tilde{T}_2(w_1) (b - \tilde{T}_2(w_1))/b}} \int_{\tilde{w}_2 \leq \tilde{z}_2}\\
    & \qquad \qquad \cdot \int_{-\infty}^{\tilde T_{3}^{-1}(w_1, \tilde{w}_2, t_2 )} \exp\left(- \frac{||w_2 -f(x) - \tilde T_{2}(w_1) (w_1 - f(x)) / b ||_2^2}{2\tilde T_{2}(w_1) (b-\tilde T_{2}(w_1))/b } \right) \mathbbm{1}\{N(w_1, w_2) > 2 \} \\
    & \vdots \\
    & \cdot \frac{1}{\sqrt[d]{2\pi \tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \left(\tilde{T}_{n-2}(w_1, \cdots, w_{n-3}) 
 - \tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \right) / \tilde{T}_{n-2} (w_1, \cdots, w_{n-3}) }} \\
    & \cdot \int_{\tilde{w}_{n-1} \leq \tilde{z}_{n-1}} \int_{-\infty}^{\tilde T_{n}^{-1}(w_1, \cdots, w_{n-2}, \tilde{w}_{n-1}, t_n )} \mathbbm{1}\{N(w_1, \cdots, w_{n-1}) > n-1 \} \\
    & \qquad \cdot \exp\left(- \frac{|| w_{n-1} - f(x) - \left( \frac{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})}{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3})} \right) (w_{n-2} - f(x))||_2^2}{2\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) \left( \frac{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3}) - \tilde{T}_{n-1}(w_1, \cdots, w_{n-2})}{\tilde{T}_{n-2}(w_1, \cdots, w_{n-3})} \right)} \right) \\
    & \cdot \frac{1}{\sqrt[d]{2\pi \tilde{T}_{n}(w_1, \cdots, w_{n-1}) \left(\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) 
 - \tilde{T}_{n}(w_1, \cdots, w_{n-1}) \right) / \tilde{T}_{n-1} (w_1, \cdots, w_{n-2}) }} \\
    & \cdot \int_{w_n \leq z_n} \mathbbm{1}\{N(w_1,\cdots, w_n) > n \}\\
    & \qquad \cdot  \exp\left( -\frac{ || w_n - f(x) - \left( \frac{\tilde{T}_{n}(w_1, \cdots, w_{n-1})}{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})} \right) (w_{n-1} - f(x)) ||_2^2}{2\tilde{T}_{n}(w_1, \cdots, w_{n-1}) \left( \frac{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2}) - \tilde{T}_{n}(w_1, \cdots, w_{n-1})}{\tilde{T}_{n-1}(w_1, \cdots, w_{n-2})} \right)} \right)dw_n dw_{n-1} \cdots dw_{1}
\end{align*}
We then perform the same differentiation and rearrangement of terms as before to get the following
\begin{align*}
    & p^x_{1:n}(t_n, z_n, t_n, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1; n)  \\
    & \qquad = (2\pi)^{-nd/2}  \left( t_n(t_{n-1} - t_{n}) \cdots (b - t_2)\right)^{-d/2} \\
    & \cdot \prod_{i=2}^n \left( \frac{\partial}{\partial t_i} T_{i}^{-1}(t_{i-1}, \tilde{z}_{i-1}, t_i ) \mathbbm{1}\left\{ N((\tilde{z}_1, T_{2}^{-1}(\tilde{z}_1,t_2) ), \cdots (\tilde{z}_{i-1}, T_{i}^{-1}(t_{i-1}, \tilde{z}_{i-1},t_i) ) > i-1 \right\} \right) \\
    & \qquad \cdot \mathbbm{1} \left\{ N((\tilde{z}_1, T_{2}^{-1}(\tilde{z}_1,t_2) ), \cdots (\tilde{z}_{n-1}, T_{n}^{-1}(t_{n-1}, \tilde{z}_{n-1},t_{n}), z_n) = n \right\} \\
    & \qquad \cdot \exp\left\{ - \frac{1}{2} \left[  \frac{|| z_n -f(x)||_2^2}{t_n}  + \frac{|| (\tilde{z}_{n-1},  T_{n}^{-1}(t_{n-1}, \tilde{z}_{n-1}, t_n )) - z_n ||_2^2}{t_{n-1} - t_n } \right. \right.  \\
    &  \qquad \qquad +\frac{|| (\tilde{z}_1, T_2^{-1}(\tilde{z}_1, t_2) ) - ( \tilde{z}_2, T_3^{-1} (t_2, \tilde{z}_2, t_3) ||_2^2}{b-t_2}\\
    & \qquad \qquad \left. \left.  + \sum_{j=3}^{n-1} \frac{ || (\tilde{z}_{j-1}, T_j^{-1}(t_{j-1}, \tilde{z}_{j-1}, t_j) ) - (\tilde{z}_{j}, T_{j+1}^{-1}(t_{j}, \tilde{z}_{j}, t_{j+1}) ) ||_2^2}{t_{j-1} - t_j}  \right] \right\}
\end{align*}
As before, we can integrate over $t_{n-1}, \tilde{z}_{n-1}, \cdots, t_2, \tilde{z}_2, \tilde{z}_1$ to get the density $p^x(t_n, z_n;n)$ for $\tilde{M}^*_{\text{last} }(x)$, to get the same relation as in \eqref{eq:pl_relation}, but now for random stopping times.


\begin{proof}[\textbf{Proof of Lemma~\ref{lem:bm_nr}}]

For any initial value $\mu \in \R^d$ and any $n \geq 1$, let $p^\mu_{1:n}$ denote the joint density of $B_{T_n}, \dots, B_{T_1}$ where $(B_t)_{t \geq 0}$ is a Brownian motion started at $\mu$ and consider first constant time functions $t_n := T_n(x)$ and fixed $n$. We have the decomposition
\[
p_{1:n}^\mu\left(B_{t_n}, \dots, B_{t_1}\right) \propto \exp\left( - \frac{(B_{t_1} - \mu)^2}{2t_1}\right)\prod_{m = 2}^n \exp\left(\frac{-(B_{t_m} - \mu - \frac{t_m}{t_{m - 1}}(B_{t_{m -1}} - \mu))^2}{2(t_{m - 1} - t_m)}\cdot \frac{t_{m -1}}{t_m}\right).
\]

This decomposition follows as $B_{t_1} \sim \calN(\mu, t_1)$, and, given $B_{t_1}, \dots, B_{t_{m - 1}}$, we have that $B_{t_m} \sim \calN\left(\mu + \frac{t_m}{t_{m - 1}}(B_{t_{m - 1}} - \mu), \frac{(t_{m - 1} - t_m)t_m}{t_{m - 1}}\right)$, as $B_{t_m}$ is conditionally distributed as a Brownian bridge. 
Now, a straightforward calculation yields the equivalence
\begin{align*}
    p^\mu_{1 : n}(B_{t_n}, \dots, B_{t_1}) &\propto \exp\left( - \frac{(B_{t_1} - \mu)^2}{2t_1}\right)\prod_{m = 2}^n \exp\left(\frac{-(B_{t_m} - \mu - \frac{t_n}{t_{m - 1}}(B_{t_{m -1}} - \mu))^2}{2(t_{m - 1} - t_m)}\cdot \frac{t_{m -1}}{t_m}\right) \\
    &= \exp\left(\frac{-(B_{t_n} - \mu)^2}{2t_n}\right)\prod_{m = 2}^n \exp\left(\frac{-(B_{t_{m - 1}} - B_{t_m})^2}{2(t_{m - 1} - t_m)}\right).
\end{align*}
Hence, for any two mean vectors $\mu, \mu' \in \R^d$, we can decompose the ratio of densities as 
\[
\frac{p^\mu(B_{t_n}, \dots, B_{t_1})}{p^{\mu'}(B_{t_n}, \dots, B_{t_1})} = \frac{\exp\left(\frac{-(B_{t_n} - \mu)^2}{2t_n}\right)}{\exp\left(\frac{-(B_{t_n} - \mu')^2}{2t_n}\right)},
\]
which is just the ratio between the density of a $\calN(\mu, t_n)$ random variable evaluated at $B_{t_n}$ and the density of a $\calN(\mu', t_n)$ random variable evaluated at $B_{t_n}$, proving precisely the desired result.
\end{proof}
\jwcomment{Throwing stuff in here:}


\textbf{$N$ is finite, but unbounded.} Now, suppose that for all sequences $(y_m)_{m \geq 1}$, all we know is that $N\left((y_m)_{m \geq 1}\right) < \infty$. Let $\delta > 0$. Then, for any $\omega \in \R^d$, there is some (deterministic) $n_\delta^\omega \in \N$ such that $\P\left(N\left(\left(B_{T_n^\omega}^\omega\right)_{n \geq 1}\right) \leq n_\omega^\delta\right) \geq  1 - \delta$. 

Fix $\mu, \nu \in \R^d,$ and let $n^\delta := n_\nu^\delta \lor n_\mu^\delta$. Let us define the event $E^\delta$ as 
\[
E^\delta := \left\{N\left(\left(B_{T_n^\omega}^\omega\right)_{n \geq 1}\right) \leq n^\delta\right\},
\]
which by assumption occurs with probability at least $1 - \delta$. On this is event, we can apply the result from the earlier case where $N$ is bounded by constant (in this case, the constant is $n^\delta$). Note we are not conditioning in our argument, but only examining the ratio of densities for sample paths lying in $E^\delta$. We thus have
\[
\frac{p^\nu_{1:N}\left(B_{T_1^\nu}^\nu, \dots, B_{T_{N^\nu}^\nu}^\nu\right)}{p^\mu_{1:N}\left(B_{T_1^\nu}^\nu, \dots, B_{T_{N^\nu}^\nu}^\nu\right)} = \frac{\exp\left(-\frac{\left\|B_{T_{N^\nu}^\nu}^\nu - \nu\right\|^2}{2T_{N^\nu}^\nu}\right)}{\exp\left(-\frac{\left\|B_{T_{N^\nu}^\nu}^\nu - \mu\right\|^2}{2T_{N^\nu}^\nu}\right)}
\]
    

with probability at least $1 - \delta$. However, since $\delta \in (0, 1)$ was arbitrary, the result occurs with probability 1.



\rrcomment{Integrating notes from Gena}

We want to show that the Laplace noise reduction is indeed a noise reduction mechanism.  We have a Markov process $(X(t), t \geq 0)$ with $X(0) = 0$ and for each $t > 0$, $X(t)$ has the Laplace distribution with parameter $t$.  The process has independent increments, so that for $0 \leq t_1 < t_2 < \cdots < t_k$ the following increments are independent, and hence the process is Markovian:
\[
X(t_0), X(t_1) - X(t_0), \cdots, X(t_k) - X(t_{k-1}.
\]

Recall that the Laplace noise reduction will add noise to a statistic $f: \calX \to \R^d$ where the noise will follow from the above Markov process.  We now consider time function $(T_n: n \geq 1)$ where $T_1 =b>0$ is a constant for $n \geq 2$, we have $T_n: (0,b] \times \R^d$ such that $T_n(t,z) < t$ for all $(t, z) \in (0,b) \times \R^d$.  We assume that $T_n(t,z)$ is strictly increasing in each coordinate of $z$ as well as $t$ for each $n$.  

\begin{lemma}
Let LNR be associated with $(T_n)_{n \geq 1}$ and a function $f: \calX \to \R^d$ with $\ell_1$-sensitivity $\Delta_1$.  If $N$ is a stopping function and we write $\calL_{1:N(x))}$ as the privacy loss of LNR then we have 
\[
\calL_{1:N(x))} = \calL_{N(x)}
\]
Furthermore, we have
\[
\calL_{N(x)} = |X(T_{N(x)}(x))| / T_{N(x)}(x) - |X(T_{N(x)}(x)) - \Delta_1|/T_{N(x)}(x)
\]
\end{lemma}


The Laplace noise reduction $\LNR_{1:n}(x)$ can then be written as 
\[
\LNR_{1:n}(x) = \left( (T_n(x), f(x) + X(T_{n}(x))), (T_{n-1}(x), f(x) + X(T_{n-1}(x))), \cdots, (T_1(x), f(x) + X(T_{1}(x))) \right)
\]

Note that it suffices to consider the modified mechanism $\tilde{M}_{1:n}$ where \rrcomment{This will probably need to be modified to account for multivariate $z \in \R^d$.}
\[
\tilde{M}_{1:n}(x) = \left( (T_n(x), f(x) + X(T_{n}(x))), f(x) + X(T_{n-1}(x)), \cdots, f(x) + X(T_{1}(x)) \right)
\]

Recall that $\LNR(x)$ will be constant between two endpoints.  We will write set $\calA_k$ as the following collection of intervals with $k \geq 1$
\[
\calA_n = \bigcup_{k \geq 1 } \left\{ \varprod_{j=1}^d \left\{ [a_i^{(j)}, b_i^{(j)}]: 1 \leq a_1^{(j)} < b_1^{(j)} < a_2^{(j)} < b_2^{(j)} < \cdots < a_k^{(j)} < b_k^{(j)} \leq n,  i \in [k] \right\} \right\}
\]
We then define the collection of all sequences $(z_1, \cdots, z_n) \in \R^{d \times n}$ such that $z_{\ell, j}$ is constant for all $a_{i}^{(j)} \leq j \leq b_{i}^{(j)}$. so we can consider the state space $S$ of $\tilde{M}_{1:n}$ in the following form 
\[
S = \bigcup_{\calA} (S_{\calA_n} \times (0,b))
\]
where we denote $\calA$ 


\begin{proof}
\textbf{Step 1: reduction to the case $a = b = 0$:}
First, we note that it suffices to prove the result when $A = a$ is a constant. If we prove the result in this case, we note we have by the tower rule for conditional expectations that, for any event $E$,
\[
\P(Y^{(\tau)} \in E) = \E\left[\P\left(Y^{(\tau)} \in E \mid A \right)\right] = \E\left[\P\left(Z \in E\right)\right] = \P\left(Z \in E \right),
\]

where $(Z_t)_{0 \leq t \leq 1}$ is a Brownian bridge with $Z_0 = Z_1 = 0$. Next, note it suffices to prove the result in the case $a = b = 0.$ Let $(X_t)_{0 \leq t \leq 1}$ be a Brownian bridge satisfying $X_0 = a$ and $X_1 = b$. Define another process $(X_t')_{t \geq 0}$ on the same probability space by $X_t' := X_t - (1 - t)a - tb$. By the first part of Lemma~\ref{lem:bb_prop}, $(X_t')_{t \geq 0}$ is a Brownian bridge on $[0, 1]$ with initial point $X_0' = 0$ and $X_1' = 0$. Clearly, the natural filtration $(\calG_t)_{0 \leq t \leq 1}$ for $(X_t)_{0 \leq t \leq 1}$ is also the natural filtration for $(X_t')_{0 \leq t \leq 1}$. Further, a simple calculation yields that for any fixed $0 \leq s \leq t \leq 1$, $X_t^{(s)'} = X_t^{(s)}$. Thus it also follows that $Y_t^{(\tau)'} = Y_t^{(\tau)}$ for all $(\calG_t)$ stopping times $\tau$ and all $0 \leq t \leq 1$.

\textbf{Step 2: considering when $\tau = T$ is deterministic:}
Thus, going forward we consider the case where $(X_t)_{0 \leq t \leq 1}$ is a Brownian bridge with $X_0 = X_1 = 0$. Clearly it suffices to consider $(X_t)_{0 \leq t \leq 1}$ to be one-dimensional in what follows, as in the multivariate case the coordinates of $X$ are independent one-dimensional Brownian bridges. We first consider the case where $\tau = T$ is a constant time. In this case, the process $(Z_t)_{0 \leq t \leq 1}$ given by
\[
Z_t := \begin{cases} X_t \qquad \text{for } 0 \leq t < T, \\
X_{t - T}^{(T)} \qquad \text{for } T \leq t \leq 1   
\end{cases}
\]
is clearly a Gaussian process on $[0, 1]$ that is continuous on $[0, T)$ and $[T, 1]$. To show the result, we must show (1) for any $s \in [0, T), t \in [T, 1]$, $k(s, t) := \Cov(Z_s, Z_t) = 0$ (this implies $X^{(T)}$, and hence $Y^{(T)}$ is independent of $\calG_T$), (2) $\mu(t) := \E Z_t = 0$ for all $t \in [T, 1]$, and (3) $k(s, t) := \Cov(Z_s, Z_t)= (s - T)\land (t - T) - \frac{(s - T)(t - T)}{1 - T}$ for all $s, t \in [T, 1]$ (these final two points show the law of $X^{(T)}$ is that of a Brownian bridge since we already have sample path continuity).

We now check each of these properties. In what follows, recall that $X_t = B_t - tB_1$ for some (now one-dimensional) Brownian motion $(B_t)_{0 \leq t \leq 1}$, and remember that $\Cov(B_s, B_t) = s\land t$. 
\begin{enumerate}
    \item For $s \in [0, T)$ and $t \in [0, 1 - T]$, we have (assuming for now that $\E[X_t^{(T)}] = 0,$ which we confirm in a later point)
    \begin{align*}
    \Cov(X_s, X_t^{(T)}) &= \E\left[X_s\left(X_{t + T} - \frac{1 - T - t}{1 - T}X_T\right)\right] \\
    &= \E\left[(B_s - s B_1)\left(B_{t + T} - (t + T)B_1 - \frac{1 - T - t}{1 - T}B_{T} + \frac{1 - T - t}{1 - T}TB_1\right)\right].
    \end{align*}
    We now can compute
    \begin{align*}
    &\E\left[B_s\left(B_{t + T} - (t + T)B_1 - \frac{1 - T - t}{1 - T}B_{T} + \frac{1 - T - t}{1 - T}TB_1\right)\right] \\
    &\qquad = s\left(1 - (t + T) - \frac{1 - T - t}{1 - T} + \frac{1 - T - t}{1 - T}T\right) \\
    &\qquad = \frac{s}{1 - T}\left( (1 - T) - (1 - T)(t + T) - (1 - T - t) + (1 - T - t)T\right) \\
    &\qquad = 0.
    \end{align*}
    Likewise, we have
    \begin{align*}
    &\E\left[s B_1\left(B_{t + T} - (t + T)B_1 - \frac{1 - T - t}{1 - T}B_{T} + \frac{1 - T - t}{1 - T}TB_1\right)\right] \\
    &\qquad = s\left( (t + T) - (t + T) - \frac{1 - T - t}{1 - T}T + \frac{1 - T - t}{1 - T}T\right) \\
    &\qquad = 0.
    \end{align*}
    This computation confirms the first point.
    
    \item For any $t \in [0, 1 - T]$, we have
    \begin{align*}
        \E\left[X_t^{(T)}\right] &= \E\left[B_{t + T} - (t + T)B_1 - \frac{1 - T - t}{1 - T}B_{T} + \frac{1 - T - t}{1 - T}TB_1\right] = 0,
    \end{align*}
    proving the second point.
    \item Lastly, using property 3 of Lemma~\ref{lem:bb_prop}, for $s, t \in [0, 1 - T]$ s.t.\ $s < t$, we have
    \begin{align*}
    \Cov\left(X_s^{(T)}, X_t^{(T)}\right) &= \E\left[\left(X_{s + T} - \frac{1 - T - s}{1 - T}X_T\right)\left(X_{t + T} - \frac{1 - T - t}{1 - T}X_T\right)\right] \\
    &= \left\{(s + T) - (s + T)(t + T)\right\} - \frac{1 - T - t}{1 - T}\left\{T - (s + T)T\right\} \\
    &\qquad - \frac{1 - T - s}{1 - T}\left\{T - (t + T)T\right\} + \frac{(1 - T - t)(1 - T - s)}{(1 - T)^2}\left\{T - T^2\right\} \\
    &= \frac{1}{1 - T}\Big[(s + T)(1 - T - t)(1 - T) - T(1 - T - s)(1 - T - t)\Big]\\
    &= \frac{(1 - T - t)s}{(1 - T)} = s - \frac{st}{1 - T}.
    \end{align*}
\end{enumerate}

Since we have shown that, for any $T \in [0, 1],$ $Y^{(T)}$ is independent of $\calG_T$, we have that, for any $E \in \calG_t$ and any bounded, any fixed times $0 \leq t_1 < t_2 < \cdots < t_p \leq 1$, and continuous function $F : \R^{dp} \rightarrow \R_{\geq 0},$

\[
\E\mathbbm{1}_E F(Y_{t_1}^{(T)}, \dots, F_{t_p}^{(T)}) = \P(A) \E F(X_{t_1}, \dots, X_{t_p}),
\]
which is a fact we will use in the sequel.

\textbf{Step 3: generalizing to general stopping times:}

We now emulate a standard proof of the strong Markov property for Brownian motion to extend to the case where $\tau$ is a $(\calG_t)_{0 \leq t \leq 1}$ stopping time (in particular, the proof of Theorem 2.20 in \citet{le2016brownian}).

It suffices to show that, for any $A \in \calG_\tau$, $0 \leq t_1 < t_2 < \cdots < t_p \leq 1$, and $F : \R^{dp} \rightarrow \R_{\geq 0}$ continuous and bounded that
\[
\E\mathbbm{1}_AF(Y_{t_1}^{(\tau)}, \dots, Y_{t_p}^{(\tau)}) = \P(A)\E F(X_{t_1}, \dots, X_{t_p}).
\]

As noted in \citet{le2016brownian}, this not only proves the independence of $(Y_t^{(\tau)})$ and $\calG_\tau$, but also demonstrates by taking $A = \Omega$ (where $(\Omega, \calF, \P)$ is the underlying probability space) that $(Y_t^{(\tau)})$ and $(X_t)$ have the same finite-dimensional distributions, and hence $(Y_t^{(\tau)})$ is a standard $d$-dimensional Brownian bridge since sample paths are continuous.

For $n$ a positive integer and $T \in \R$, define $T\vert_n := \min\{ k2^{-n} : k \in \Z,\; k2^{-n} \geq T\}$, i.e.\ $T\vert_n$ is the smallest real of the form $k2^{-n}$ that is greater than or equal to $T$. A straightforward expansion of $Y_t^{(\tau\vert_n)}$ yields that, for any $t \in [0, 1]$, we have $Y_t^{(\tau\vert_n)} \xrightarrow[n \rightarrow \infty]{} Y_t^{(\tau)},$ and thus bounded convergence yields
\begin{align*}
\E\mathbbm{1}_A F(Y_{t_1}^{(\tau)}, \dots, Y_{t_p}^{(\tau)}) &= \lim_{n \rightarrow \infty}\E \mathbbm{1}_A F(Y_{t_1}^{(\tau\vert_n)}, \dots, Y_{t_p}^{(\tau\vert_n)}) \\
&= \lim_{n \rightarrow \infty}\sum_{k = 0}^{2^n}\E\mathbbm{1}_A\mathbbm{1}_{E_n^k}F(Y_{t_1}^{(\tau\vert_n)}, \dots, Y_{t_p}^{(\tau\vert_n)}) \\
&= \lim_{n \rightarrow \infty}\sum_{k = 1}^{2^n}\E\mathbbm{1}_A\mathbbm{1}_{E_n^k} F(Y_{t_1}^{(k2^{-n})}, \dots, Y_{t_p}^{(k2^{-n})}) \\
&= \lim_{n \rightarrow \infty}\sum_{k = 1}^{2^n}\P(A \cap E_n^k) \E F(Y_{t_1}^{(k2^{-n})}, \dots, Y_{t_p}^{(k2^{-n})})\\
&= \P(A)\E F(X_{t_1}, \dots, X_{t_p}),
\end{align*}
where $(X_t)_{0 \leq t \leq 1}$ is a standard $d$-dimensional Brownian bridge, proving the desired result. In the above, $E_n^k := \{(k - 1)2^{-n} < \tau \leq k2^{-n}\}$, and we use the identity $\mathbbm{1}_{E_n^k}F(Y_{t_1}^{(\tau\vert_n)}, \dots, Y_{t_p}^{(\tau\vert_n)}) = \mathbbm{1}_{E_n^k} F(Y_{t_1}^{(k2^{-n})}, \dots, Y_{t_p}^{(k2^{-n})})$. The second to last inequality follows from applying the result where $t$ is a deterministic time, noting that the event $A \cap E_n^k$ is $\calG_{k2^{-n}}$-measurable.

Thus, we have shown the desired result.
\end{proof}

